The Politics of Fear and the Experience of Bangladeshi Religious Minority Communities Using Social Media Platforms

Despite significant research on online harm, polarization, public deliberation, and justice, CSCW still lacks a comprehensive understanding of the experiences of religious minorities, particularly in relation to fear, as prominently evident in our study. Gaining faith-sensitive insights into the expression, participation, and inter-religious interactions on social media can contribute to CSCW's literature on online safety and interfaith communication. In pursuit of this goal, we conducted a six-month-long, interview-based study with the Hindu, Buddhist, and Indigenous communities in Bangladesh. Our study draws on an extensive body of research encompassing the spiral of silence, the cultural politics of fear, and communication accommodation to examine how social media use by religious minorities is influenced by fear, which is associated with social conformity, misinformation, stigma, stereotypes, and South Asian postcolonial memory. Moreover, we engage with scholarly perspectives from religious studies, justice, and South Asian violence and offer important critical insights and design lessons for the CSCW literature on public deliberation, justice, and interfaith communication.

==> sections/background.tex <==
\section{Literature Review}
%\rifat{Will rewrite this section to improve the narrative, add more citations, and situate this paper better aligning with the discussion}

Bryan’s Suggestions for Organizing the Literature Review

NOTE: This is a very high level suggest outline that I just put together now based on the writing here. I normally would have much more detail fleshing out each section and how it builds the argument we are making, and I often take some time to make sure it is all well laid out before I put in all the details. But I think it’s important for you all—Rifat and Dipto—to make a first pass at this based on these suggestions. If for any reason you do not agree with this, I would love to hear that and more of why!

Section 1: What is the Public Sphere?

Start by defining what we mean by the public sphere. You can draw on public sphere scholars here, such as Habermas and those who are critical of Habermas. See my papers in the comments for a guide on which literature to reference here. But the general gist is that it is a public space wherein people can engage in deliberative practices, include discourse and information exchange, to influence public opinions and policies

Section 2: Negative Experiences in the Offline-Online Public Sphere: An Intersectional Perspective

Shift from a focus on what is the public sphere to the online public sphere

Say how today, social media platforms serve as a digitally-mediated public sphere that work in tandem with the physical world public sphere

In this paper, we focus not on politics systems—as in how digital media shape conversations about political institutions and elites—but the politics, or bias, that shape how people experience and interact online (think of the Langdon Winner form of politics here). You can frame a question related to how people's participation in the public sphere is shaped by their identities?

Define what you mean by identity

Then build on that foundational definition and shift to intersectionality 

Describe the various studies on harm and marginalized identities as you have done

Describe how polarization fits into this conversatoin (though perhaps that can go into the nexct section on religious minorities to help explain the politics of fear). For example, perhaps the idea is that these negative experiences are leading to a polarized intersectional public sphere where people are congregating with like-minded others, or people who share their same identities. 

After you describe the broader literature, then segue into the main focus of this paper—religious minorities

Section 3: The Politics of Fear and Group Co-Existence: The Case of Religious Minorities

To frame the exploration of religious minoirity experiences in the public sphere, we draw on the concept of fear; use the definition of fear you have used

Then highlight how in this work we highlight different ways in which fear can manifest in public spheres 

Start by describing the spiral of silence, highlighting what that concept is, and how it relates to fear

Then, focus on the politics of fear (though, could it be argued that the spiral of silence is a subcategory of the spiral of silence?)

Then highlight all of the work, or lack thereof, focused on religious minorities and how our work is filling a critical and important gap

On Design Justice lenses; I think those need to be removed entirely from the lit review and perhaps introduced in the Discussion. You could of course integrate them into the lit review, but they should be clearly tied to the argument. Given that those lenses aren’t integral to the primary argument and narrative of the Results, I see them as more of a discussion point.

Addendum: I do want to make something clear in this proposed revision. I am simply taking the ideas and concepts that are already presented, but asking for those ideas to be clearly defined and articulated, and importantly, putting them into conversation with one another that frames the narrative of the paper. 

We draw from three lines of scholarship to inform and frame our work: the experience of online harms and support to cope with and mitigate harms for minority communities; public opinion, online polarization, and the marginalization of minority communities; and fear and group coexistence. In the Findings section, we draw from the theories of the spiral of silence, politics of emotion, and communication accommodation to frame and discuss our findings from the study.

\subsection{Online Harms, Support, and Justice for Minority Communities on Social Media}

CSCW has extensively documented the various forms of harassment, harm, and violence that minority communities face online. Scholars in this field have shed light on the challenges minority communities encounter when expressing their identity on social media platforms. One notable study by Cho explores the experiences of US queer youth of color on social media, specifically within the queer Tumblr community~\cite{cho2018default}. The research highlights the concept of ``default publicness,'' an inherent design orientation that prioritizes state-validated identities, often favoring majoritarian views~\cite{cho2018default}. As a result, minority queer youth of color often lose control over their social media activity and face severe negative consequences as their posts are unexpectedly shared with unintended audiences~\cite{cho2018default}. Building on these findings, Devito et al. investigate the misalignment between platform values and the values held by minority LGBTQ+ communities, revealing the negative experiences and harms that arise from this disconnect~\cite{devito2021values}. The CSCW community has further expanded on the struggles faced by minority communities on social media platforms. For instance, Scheuerman et al. conduct interviews to examine the risks and harms experienced by transgender individuals in the US~\cite{scheuerman2018safe}. Their research uncovers how the same platforms that offer opportunities for connection and safe spaces can also be harmful and abusive towards transgender individuals~\cite{scheuerman2018safe}. Anti-trans social media users are shown to target and harass transgender populations, making their online experiences stigmatizing~\cite{scheuerman2018safe}. In similar vein, DeVito et al. employ cognitive mapping exercises and interviews to illustrate how LGBTQ+ communities navigate stigma while performing their identities and seeking social support on social media platforms~\cite{devito2018too}. These studies reveal that minority communities have to take an extra burden to strategically utilize social media ecosystems in mitigating harassment and maintaining a sense of safety. CSCW research has similarly documented harms and unsafe experiences among racial minority groups~\cite{ogbonnaya2020critical, smith2020s, cunningham2023grounds, adamu2023no}. To et al. utilize narrative episode interviews and semi-structured interviews to explore support-seeking practices among racially marginalized populations~\cite{to2020they}. Their findings illustrate the emotional and physical discomfort, embarrassment, and lack of belongingness experienced by individuals due to direct and indirect racially discriminating activities~\cite{to2020they}. Additionally, CSCW literature highlights how minority communities often form counterpublics in response to harms; however, their activism is met with further harassment and harm. For instance, Salehi et al. investigate how visible Muslim American public figures utilize social media platforms to challenge dominant narratives demonizing Muslims and construct counter narratives~\cite{salehi2023sustained}. The demonstrate, the same platform affordances designed to empower users are weaponized against minority social media users, resulting in sustained harassment and abuse of these communities~\cite{salehi2023sustained}. These studies, alongside others in the CSCW and HCI~\cite{buss2022transgender, southerton2021restricted, pym2021still, paceley2022sometimes, simpson2021you}, provide a broad and nuanced understanding of the marginalization, harassment, bias, and other negative experiences encountered by minority communities on social media and other online spaces.

In addition to the existing inequalities faced by minority communities, the intersectionality of multiple minority identities further exacerbates the harms experienced by these communities. Scheuerman et al., for instance, shed light on the intensified abuse and marginalization faced by minority transgender populations, who are also women of color or sex workers~\cite{scheuerman2018safe}. Further exploring the intersectionality of identities, Feuston et al. examine trans individuals with eating disorders and find that the trans minority community within the eating disorder community is more vulnerable to online harm due to the continuous need to validate their identity~\cite{feuston2022you}. The authors argue that dominant norms and standards around eating disorders, often perpetuated by cisgender individuals, create challenges for trans communities who challenge these norms~\cite{feuston2022you}. Similarly, Andalibi et al. focus on LGBTQ individuals and other gender or sexual minorities who have experienced pregnancy loss or have partners who have experienced it~\cite{andalibi2022lgbtq}. Through an intersectional analysis of online experiences during pregnancy loss, the authors demonstrate how the combination of LGBTQ identity and pregnancy loss intensifies discrimination and exclusion on social media platforms~\cite{andalibi2022lgbtq}. Haimson et al. examine non-normative users of social networking sites (SNS) who undergo identity changes and find that the politics of categorization, such as gender, on SNS interfaces can contribute to stress for minority communities within socio-technical systems~\cite{haimson2015disclosure}. Collectively, studies on intersectional minority communities confirm that individuals with intersecting minority identities along axes of race, gender, sexuality, and more, encounter a range of compounding harmful experiences, including harassment, marginalization, bias, and violence. However, the CSCW literature currently lacks comprehensive insights (with a few exceptions) into the experiences of religious minority communities on social media.

To cope with the negative experience and navigating other online safety related issues, the minority communities often find the social media platform policies misaligned and sometimes hostile to them. For example, minority communities are often forced to conform to the universal platform politics and marginalized further~\cite{shahid2023decolonizing, feuston2020conformity}. Drawing on a two years long digital ethnography, Feuston et al. shows how an already marginalized group, people with eating disorders, are pressured to conform to the dominant groups in the content moderation policies~\cite{feuston2020conformity}. The authors show how the eating disorder community loses personal contents and community support due to a moderation that is more aligned with the dominant online user groups. This, in turn, loads the community with an added task of restoring their lost contents. In a similar vein, Haimson et al. study the frequency of content removals for the political conservatives, transgender, and black people through moderation is higher than other communities~\cite{haimson2021disproportionate}. The authors further show that trasnpeoples’ contents are often removed with the allegation of being adult, insulting for the dominant groups, and violent, even though these contents follow the community guidelines. Shahid and Vashistha find how content moderation policies are often oblivious of the context and culture of the global south population~\cite{shahid2023decolonizing}. The risks and vulnerability of the minority communities can also be exacerbated by the increasing move from text-based interactive platforms to video-based interactive platforms. For example, while platforms such as Facebook and Twitter are mostly friends and/or follower based that can emphasize in-group interaction, the video sharing platform such as TikTok cross-partisan dialogues, with the contents being created with aggressive goals to be viral~\cite{medina2020dancing}. The contents are created with humor and sarcasm with the goal of making them viral and run into the risk of ridiculing and bullying minority communities in the form of entertainment, which may not be filtered in the existing moderation technologies. Supporting minority communities through computational tools is also challenging for a number of reasons. The challenges primarily stem from the communities’ willingness to participate in designing and using computational tools that may make them vulnerable to increased exposure and scrutiny for the broader community. Saha et al., for example, note complexities of quantifying the data of the minority communities, that might limit the participation of the community in anticipation that their data are being quantified and silence their participation altogether~\cite{saha2019language}. Cui et al. conduct an interview-based study with the sexual minority women in China in using dating apps and find that the SMWs use the dating app for careful identity disclosure and development~\cite{cui2022so}. The authors discussed how SMW communities are often afraid of unexpected disclosure of their identity, which, in turn, might threaten their online safety by non-LGBTQ communities. These findings suggest that social media policies are barely adaptive to non-dominant identities, norms, and their ways of being.

One nascent body of literature is focusing on restorative justice to mitigate harm for the minority communities~\cite{xiao2023addressing, xiao2022sensemaking, chatlani2023teen, rabaan2023survivor}. The proponent of this literature are arguing for turning the attention from platforms to the vulnerable and affected communities and supporting them~\cite{salehi2023sustained, xiao2023addressing}. Social media companies often address online harm following a justice model primarily centered on ``isolation and punishment’’~\cite{myers2018censored, vaccaro2020end}. While social media platforms offer users the ability to customize posts, report, delete, block content, and contest moderation decisions, these features effectively place the burden on users while holding the power in their hands. These affordances support the platform's governance, moderation, and regulation within the framework of isolation and punishment. Consequently, ethical and political aspects of societies, local modes of justice, and the essence of life of users are disregarded as social media platforms’ policies to tackle online harms are often isolated from local histories, communal practices, and culture~\cite{shahid2023decolonizing}. In contrast, CSCW advocates for prioritizing the victims of online harms and restoring communal bonds and relationships~\cite{xiao2023addressing}. Alongside modern values of freedom, equality, accountability, and deliberation, concepts like healing, apology, social harmony, and other human virtues~\cite{xiao2023addressing} are receiving attention in addressing online harms through restorative justice. While these directions offer hope for supporting the victims, we argue that the literature needs an extension to contextualize restorative justice—as we have discussed in this paper—to better account for the social-psychological and political aspects of fear in South Asia. These aspects in South Asia are often laden with colonial trauma and religious sensitivity, particularly for religious minority communities.


%overlooks the social psychology and politics of fear as has been shown in our study, which intersect with colonial trauma and religious sensitivity for religious minority communities.

The primary reason why we argue for an extension of the literature about religious minority communities, along with the justice frameworks to support them in South Asia, stems from the differences among minority communities in terms of their identities, values, ethics, and contexts. In this paper, we specifically emphasize how faith based politics shape the social media use experiences of religious minority groups, which often serve as an extension, albeit an amplified one, of their social lives. Our analysis centers around fear as a key aspect of the minority experience on social media. This emphasis on fear is informed by a robust body of literature demonstrating how ``religious nationalism,'' which is more prevalent in South Asian regions compared to the Global North and reinforces discrimination and fear against religious minority communities~\cite{bhatia2021religious, bhatia2022hindu, mohan2015locating}. As opposed to modern and secular presumption that social networking sites (SNS) inspire depoliticized and rational societies, SNS platforms in South Asia contribute to the constitution of religious subjects online and amplify existing social segregation along religious identity lines~\cite{bhatia2021religious}. Contrary to the utopian notion of ``self-abstraction'' in public spheres, including social media platforms~\cite{cody2015populist}, far-right religious nationalists in South Asia employ social media to perpetuate social fear, discrimination, and stereotypes against minority castes and religions~\cite{vaghela2021birds, bhatia2021religious, mohan2015locating}. Some individuals may adopt different personas online compared to offline interactions. For instance, they may refrain from engaging in harmful activities offline, but as part of ``digital collectives,'' the same individuals exhibit discriminatory behavior towards religious others through trolling, cyber-bullying, and other online means in South Asian online sphere~\cite{bhatia2021religious}. The politics of fear are often supported and normalized by political parties that benefit from such narratives~\cite{bhatia2022hindu}. The far-right majoritarian religio-political forces enforce various normative systems of ``online'' punishment, including mob violence against religious minorities, further intensifying the fear of engagement with social media and discursive activities among minority communities in South Asia~\cite{bhatia2022hindu}. Altogether, religious minority groups are depicted as both perpetrators and victims of online violence~\cite{kirmani2008competing, bhatia2022revolution}. This is in this context we emphasize that the existing CSCW insights about minority communities are inadequate for understanding the experiences of religious minority communities. To address this gap, our research aims to comprehensively explore the experiences of religious minority communities particularly emphasizing fear-related aspect of their experience using theoretical lenses drawn from anthropology and cultural studies. 

%The literature within the field of CSCW extensively documents various minority communities, but with an imbalanced focus on the Global North, neglecting the experiences of minorities in the global South. The minority communities in South Asia differ


%Through this approach, we aim to contribute to the existing CSCW literature on online deliberation, participation, and online safety by providing a nuanced understanding of the experiences of religious minorities within the context of South Asia.


%social media works both as a stressful and supportive platform for the users~\cite{haimson2015disclosure}. The authors find that






%To protect the communities, the authors proposes refraining harm as a disturbance in interpersonal relationship as opposed to crimes against the State or the social media platforms






%For example, Salehi et al. conduct and interview-based study and document how Muslim Americans regularly face harassment and abuse in their activism against the dominant voices who demonize Muslims~\cite{salehi2023sustained}. The same platform affordances that are designed to empower users for ease of accessing the platforms, are weaponized against the minority social media users~\cite{salehi2023sustained}. Intersectional identities, such as race, gender, and other non-confirming identities, further intensify these harmful behaviors. In a similar vein, DeVito et al. conducted cognitive mapping exercises and an interview-based study to report on how LGBTQ+ communities have to take an extra burden to avoid stigma while performing their identities and getting social support~\cite{devito2018too}. They demonstrate how the communities maintain an ecosystem of social media platforms to strategize their identity performances while saving themselves from harassment. Andalibi et al. studied LGBTQ and other gender or sexual minorities who (or their intimate partners) had an experience of pregnancy loss~\cite{andalibi2022lgbtq}. Through an intersectional and categorical analysis of the communities’ online experiences during pregnancy loss, the authors discussed how various minority identities benefited or marginalized people online <expand>. Haimson et al. study the non-normative SNS users who go through identity changes and find that social media works both as a stressful and supportive platform for the users~\cite{haimson2015disclosure}. The authors find that various politics in categorization (such as gender) on the SNS’s interface could be a source of stress for the minority communities on socio-technical systems. Feuston et al. studies trans people with eating disorders and find that the minority trans community are more vulnerable to online harm than others with eating disorders, as the trans minority communities have to continuously validate their identity~\cite{feuston2022you}. The authors argue that the feminine contents and cis participants constitute the norms and standard on social media to discuss issues around eating disorders. The trans communities often challenge these norms and standards. These findings demonstrate how socio political influences of the dominant groups push the minorities on the periphery. Altogether, the literature documents various forms of marginalization, harassment, bias, and other negative experiences that minority communities often face on social media and other online spaces.

%the minority communities’ use of social media for identity performance, getting communal support, and coordinating grassroots activism, among others. Their findings indicate that the communities navigate additional stresses and bear the burden of undertaking cautious strategies and putting additional emotional energies to manage their identities on different platforms (Devito).



%Supporting minority communities through computational tools is also challenging for a number of reasons. The challenges primarily stem from the communities’ willingness to participate in designing and using computational tools that may make them vulnerable to increased exposure and scrutiny for the broader community~\cite{}. Saha et al., for example, note complexities of quantifying the data of the minority communities, that might limit the participation of the community in anticipation that their data are being quantified and silence their participation altogether~\cite{saha2019language}. The authors discuss methods, such as opting-in, to ensure that the minority communities are informed of any health intervention and supporting them in mitigating potential harms through such interventions. Cui et al. conduct an interview-based study with the sexual minority women in China in using dating apps and find that the SMWs use the dating app for careful identity disclosure and development~\cite{cui2022so}. The authors discussed how SMW communities are often afraid of unexpected disclosure of their identity, which, in turn, might threaten their online safety by non-LGBTQ communities. Because of these reasons, the CSCW literature must center their focus on adapting the the needs and vulnerabilities of minority communities. To this end, a nascent but growing body of literature in CSCW is increasingly focusing on restorative justice framework to better support the minority communities. As we will argue, these framework of restorative justice needs to expand in extending aftercare and adapting cultural process of shared meaning-making for the religious minorities in South Asia.

%Altogether, the literature on minority communities within the field of CSCW provides extensive documentation of various minority groups, but with a disproportionate emphasis in the Global North. These communities differ from South Asian minorities in terms of their identities, values, ethics, and context. In this paper, we particularly emphasize on how religious identities of minority groups shape their social media use experience, which is often an extension, albeit an amplified one, of their social life. We do so by centering fear into our analysis of minority experience of social media. The emphasis on fear is informed from a strong body of literature that shows how a stronger (compared to the Global North) form of ``religious nationalism'' often reify discrimination and fear against the religious minority communities in the South Asian regions~\cite{bhatia2021religious, bhatia2022hindu, mohan2015locating}. As opposed to most of the HCI studies primarily based in the West that presume that SNS will inspire a depoliticized and rational societies, the South Asian SNSs act as an ally in constituting religious subjects online and amplifying already existing social segregation along the line of religious identity~\cite{bhatia2021religious}. As opposed to the utopian vision of ``self-abstraction'' in the public spheres~\cite{cody2015populist} -- including the social media platforms -- the far-right religious nationalist in South Asia use the social media platforms to reify social fear, discrimination, and stereotypes against minority castes and religions~\cite{bhatia2021religious, mohan2015locating}. Some religious subjects are often perform different persona in online and offline. For example, people may not engage in harmful activities offline; but as a part of ``digital collectives'', the same person may engage in discriminatory behavior to the religious others through trolling, cyber-bullying, abusing, and in other ways online~\cite{bhatia2021religious}. As such, the politics of fear often are supported and normalized by political parties who benefit from the politics~\cite{bhatia2022hindu}. Various normative systems of ``online'' punishment from the far-right majoritarian religious forces, including mob violence against the religious minorities, intensify the minority communities' fear of social media engagement and discursive activities further in South Asian regions~\cite{bhatia2022hindu}. As such, the religious minority groups are presented as either the perpetrators and victims of violence~\cite{kirmani2008competing, bhatia2022revolution}. This is in this context, we emphasize how the existing insights about minority communities are insufficient for understanding the experiences of faith-based minority communities in their use of social media in this region. To address this gap, our research aims to comprehensively explore the experiences of religious minority communities using theoretical lenses drawn from anthropology and cultural studies. By doing so, we seek to contribute to the existing CSCW literature on online deliberation, participation, and online safety by providing a nuanced understanding of the experiences of religious minorities within the context of South Asia.



%While issues surrounding race, gender, and identity are pressing concerns in the modern West, faith, and religion play a significant role in delineating the boundary between majority and minority in South Asian regions~\cite{}. Given the dominant role of faith in shaping the values, ethics, and social fabric of life in South Asia~\cite{}, the existing insights about minority communities are insufficient for understanding the experiences of faith-based minority communities in their use of social media in this region. To address this gap, our research aims to comprehensively explore the experiences of religious minority communities using theoretical lenses drawn from anthropology and cultural studies. By doing so, we seek to contribute to the existing CSCW literature on online deliberation, participation, and online safety by providing a nuanced understanding of the experiences of religious minorities within the context of South Asia.

%*******


%Despite facing harassment, trauma, and fear, people in the global North enjoy greater freedom and courage to practice stronger agency and come up with safety and wellbeing plans~\cite{salehi2023sustained}. 

%We extend the existing work by centering fear into our analysis of minority experience of social media. The emphasis on fear is informed from a strong body of literature that shows how a stronger (compared to the Global North) form of ``religious nationalism'' often reify discrimination and fear against the religious minority communities in the South Asian regions~\cite{bhatia2021religious, bhatia2022hindu, mohan2015locating}.

%As opposed to most of the HCI studies primarily based in the West that presume that SNS will inspire a depoliticized and rational societies, the South Asian SNSs act as an ally in constituting religious subjects online and amplifying already existing social segregation along the line of religious identity~\cite{bhatia2021religious}. As opposed to the utopian vision of ``self-abstraction'' in the public spheres~\cite{cody2015populist} -- including the social media platforms -- the far-right religious nationalist in South Asia use the social media platforms to reify social fear, discrimination, and stereotypes against minority castes and religions~\cite{bhatia2021religious, mohan2015locating}. Some religious subjects are often perform different persona in online and offline. For example, people may not engage in harmful activities offline; but as a part of ``digital collectives'', the same person may engage in discriminatory behavior to the religious others through trolling, cyber-bullying, abusing, and in other ways online~\cite{bhatia2021religious}. As such, the politics of fear often are supported and normalized by political parties who benefit from the politics~\cite{bhatia2022hindu}. Various normative systems of ``online'' punishment from the far-right majoritarian religious forces, including mob violence against the religious minorities, intensify the minority communities' fear of social media engagement and discursive activities further in South Asian regions~\cite{bhatia2022hindu}. As such, the religious minority groups are presented as either the perpetrators and victims of violence~\cite{kirmani2008competing, bhatia2022revolution}. 


\subsection{Public Opinion, Online Polarization, and Marginalization of Minority Communities}
We connect our work to a second thread of literature within CSCW focusing on public opinion, online polarization, and CSCW’s design and policy solutions to address these issues. Nelimarkka et al. point out that as opposed to the social media’s ambition for deliberative and democratic discussion on social media, people tend to engage with ideologically like minded people resulting in political polarization~\cite{nelimarkka2018social}. The authors suggest prompting users with different viewpoints before they post something online might help to mitigate polarization. The authors further find that exposure to and deliberation with people having opposing views is often uncivil and antisocial. To address this issue, the authors suggest identifying weak ties having opposing views to a user and using them in creating a social environment to encourage an user to reflect on their viewpoints and revise them. Kim et al. presents the design and evaluation study of StarryThoughts, a socio-technical system for expressing and exploring diverse opinions on social issues online~\cite{kim2021starrythoughts}. The authors conducted a user study to see how people use the system to receive or reject others’ opinions on two pressing social issues in South Korea. Their evaluation study suggests that the demographic information of the author of a post helps others to put the content of a post more contextually, empathize with the users, and even be more receptive with the opinion that might contradict their own. As opposed to our findings, the authors find that the participants from the minority opinion were not necessarily conforming to the majorities and expressed their opinion freely. Wang et al. design affordances for the users of socio-technical systems to help users reflect on their understanding of opposing views online with the goal for bridging ideological divides~\cite{wang2022designing}. The authors use the Moral Foundation Theory to categorize and present posts and comments to the readers of news articles. This system made visible the confluences and differences of the moral framing of news articles and made users to be conscious of and literature about moral differences. Bail et al. found that exposing people to opposing political views to increase democratic and deliberative discussion could be both ineffective and counterproductive~\cite{bail2018exposure}. By indicating that intergroup communication has helped produce more effective deliberation in other contexts by promoting compromise and mutual understanding in intergroup ideologies and politics, the authors conclude that an intervention for intergroup communication needs to consider the contexts, tactics, and already existing social environment. <Summary and cite more works>


 In addition to the already existing challenges, religious minorities often encounter some additional risks of magnifying the already existing social polarization. In multicultural societies where people live alongside diverse religious “others”, people often use social media seeking for solidarity and like-minded people especially when the social climate is unfriendly towards religious others. Bhatia demonstrates how social media users extend their religious identities and engagement on social media~\cite{bhatia2019times}. This, in effect, amplifies religious prejudices and hostility among religious others, as people come together on social media spaces due to the intolerance experienced in offline spaces in the first place and they use the social media spaces to share their negative and unpleasant experiences~\cite{bhatia2019times}. The grand effect of micro-social behavior and its effect on pushing people to the online sphere to find solidarity reinforce and amplify religious divides in society~\cite{bhatia2019times}. Bhatia and Gajjala further discuss that intersectional identities often reinforce the marginality of the minority population~\cite{bhatia2020examining}. Muslim women, who constitute the minority community in a hypermasculine, characterized by dominant religious groups, and patriarchal society, often face additional barriers to appear in public spaces~\cite{bhatia2020examining}. To counter this marginality in terms of their public visibility, the minority Muslim women organized a grassroots activism on social media to develop support groups and raise their voices~\cite{bhatia2020examining}. Bahfen studies the minority Muslim communities in Australia and the USA to explore self expression and community building on social media~\cite{bahfen2018individual}. The author shows how the minority communities positively use social media for constantly validating their values and communal identities~\cite{}. In doing this, the community often counter members of their own Muslim community, who post borderline perception about their religious values. Moreover, the community also engages in public deliberation with non-minority members, who have powerful voices making public opinions online on religious issues. Following this, we argue CSCW literature on online public deliberation above is how identity -- especially religious identities and their intersection with other minority identities in the Global South -- might challenge or progress CSCW's overarching vision to address online polarization.
 
 
 
 <Summary>

The empirical exploration of opinion polarization and proposing design solutions to mitigate polarization build upon various assumptions about contexts and support infrastructures. Notable among them are related to democratic voices irrespective of faith-based identities, an increasingly unrestricted culture of practicing freedom of expression and identity, moral and legal support in unsafe situations, and an emphasis on the ``modern’’ and rational value systems. As far as faith is concerned in South Asia, <>. As a first step, we explore how ``fear’’ limits social media participation of religious minorities, especially in the global south where socio-political factors are strongly entangled with religious influences.  In effect, we draw on the cultural and peace studies to explore how such polarization operates and functions on various politics of fear. <expand a bit more>

\subsection{Fear and Group Coexistence}
Our study builds upon a substantial body of literature on conflict resolution and peacebuilding, focusing on the social and political psychological aspects of fear in the context of ethnic conflicts and peacebuilding efforts. This literature reveals that fear has been a significant factor contributing to conflicts between majority and minority groups, alongside intergroup differences and ``ancient hatred''~\cite{lake1996containing, lake1998international, melander2009geography, thiong2018politics}. Minority communities experience fear not only due to rational concerns such as safety and identity, but also as a result of political myths and various emotions, with fear being a primary emotion~\cite{lake1996containing, more}. Prominent among the scholars who have provided insights into the instrumental role of fear in lived experiences and existential questions is the theologian and philosopher Søren Kierkegaard. Kierkegaard explained how fear plays a role in helping individuals adapt to crises, while also addressing the irrational fear associated with embracing uncertainties and the unknown~\cite{kierkegaard2013fear}. In a similar line, the field of social psychology further explores the origin and role of fear in intergroup conflicts. Fear often arises from the lived experiences and past memories consciously or unconsciously held by individuals and groups. Jarymowicz and Bar-Tal discuss extensively how fear is a spontaneous and primary emotion that evolved as a response to violence and traumatic situations from the past~\cite{jarymowicz2006dominance}. Overcoming group-level fear proves to be challenging, as fear serves as an adaptive mechanism for individuals and groups to cope with adversity~\cite{jarymowicz2006dominance}. Group-level fear overrides hopes, fosters insecurity, generates mistrust, and hampers peaceful conflict resolution, as groups rely on past assumptions and threats~\cite{jarymowicz2006dominance}. 

Due to these psychological and political capacities, fear has been proved as detrimental to inter-group coexistence and build peace among groups. The detrimental impact of fear on peacebuilding is evident in Veena Das's analysis of the conflict between Hindu and Sikh communities, where fear stemming from violent memories and traumatic events hindered peaceful negotiation and conflict resolution ~\cite{das1998specificities}. Understanding these group dynamics of fear is crucial for making political decisions and fostering peace at both micro and macro levels. For instance, group coexistence necessitates compromise and support among the group members~\cite{worchel2008between, abu2001reconciliation}. While fear can sometimes inspire greater compromise, in other cases, it diminishes willingness to compromise as a group member~\cite{gayer2009overcoming, halperin2011emotional}. Besides, in peace negotiations between ethnic and religious groups, mutual risk-taking and tangible actions are vital. Halperin's empirical investigation demonstrates that fear acts as an obstacle in intergroup peace negotiations and hampers the adoption of concrete measures~\cite{halperin2011emotional}. Fear's influential impact often exacerbates conflicts by reinforcing belief in conspiracy theories~\cite{hebel2022vicious}. Overall, the aforementioned studies emphasize the importance of recognizing fear in intergroup relations and addressing its origins through psychological and political means to mitigate its effects. Drawing from this literature, our study delves into the modes, reasons, and political dimensions of fear within minority communities as manifested in their social media presence.

Similar works have also documented the fear experienced by minority communities in their social media engagement. The primary reasons behind this fear include social and political surveillance, false perceptions created by the media, and the fear of isolation and ridicule. One prominent example is the use of fear tactics to instill panic in minority communities, particularly through policing minority online activism~\cite{aziz2020fear}. Even in Western democratic nations, where individuals have more freedom and agency, minority communities, such as Muslims and Black communities, often self-censor their online expression due to the fear of increased scrutiny by law enforcement agencies~\cite{aziz2020fear}. The constant surveillance by these agencies leads minority communities to continuously monitor themselves, ensuring that their opinions align with the normative and legal frameworks, which are often set by majority voices~\cite{aziz2020fear}. News and social media also contribute to the creation of false perceptions about minority communities by disproportionately highlighting negative news about them, thereby subjecting them to extended surveillance and scrutiny. Consequently, these communities become hesitant to actively participate on social media platforms~\cite{hildreth2015fear}. In line with this, Fox and Warber explored how the fear of unintended identity exposure or social backlash limits the use of social media platforms by minority queer communities~\cite{fox2015queer}. Additionally, Leyn et al. studied ethno-religious minorities and revealed their perception of the social media "public sphere" as dominated by culturally and normatively defined majorities, leading to feelings of alienation, hostility, and distrust~\cite{de2022networked}. Consequently, they primarily connect with their networked peers to avoid conflict and potential backlash. Pew Research has also shown that individuals who perceive themselves as holding minority voices often refrain from freely expressing their opinions due to fear of ostracism and ridicule~\cite{hampton2014social}. These findings collectively demonstrate how fear marginalizes minority voices. In our study, we build upon these findings and provide an in-depth analysis of the social and political psychological insights into the fear experienced by religious minority communities on social media platforms in Bangladesh, along with their implication to CSCW.


%Older versions
%CSCW has documented various forms of harassment, harm, and violence faced by minority communities online. The dominant line of scholarship in this domain reports the harms faced by the minority communities in performing their identity on social media platforms. Cho conducts a cyberethnographic and interview-based research in queer Tumblr to explore the user experience of the US queer youth of color on social media platforms~\cite{cho2018default}. The author finds that social media adopts a ``default publicness'' -- a design orientation and belief encoded in the social media architecture -- that often privilege state-validated (which are often majoritarian) identity~\cite{cho2018default}. Because of the platforms' ignorance that all identities are not treated equally even in the US, the minority queer youth of color loss control in their social media activity and face drastic negative consequences as their posts are shared with an unexpected set of audiences~\cite{cho2018default}. Devito et al. in a similar vein find that much of the negative experiences and harms faced by the minority LGBTQ+ communities are due to the misalignment of the platforms' values and the values of minority communities~\cite{devito2021values}. A series of studies in CSCW builds on such findings of the minority community's struggle on social media platforms. For example, Scheuerman et al. conduct an interview-based study to explore the harms and risks of transgender individuals in the US~\cite{scheuerman2018safe}. The authors find that the same platforms and their affordances that gives the transgender individuals the opportunity to connect with others and build a safe space also are harmful and abusive towards them~\cite{scheuerman2018safe}. They explain how anti-trans social media users present transgender population ``enemies'' and harass them on the online sphere by making social media use a stigmatic experience~\cite{scheuerman2018safe}. DeVito et al. conducted cognitive mapping exercises and an interview-based study to report on how LGBTQ+ communities have to take an extra burden to avoid stigma while performing their identities and getting social support~\cite{devito2018too}. They demonstrate how the communities maintain an ecosystem of social media platforms to strategize their identity performances while saving themselves from harassment. CSCW has documented similar findings of harms and unsafe experience among the racial minority groups~\cite{ogbonnaya2020critical, smith2020s, cunningham2023grounds, adamu2023no}. To et al. conduct narrative episode interviews followed by semi-structured interviews to explore the support-seeking practices of racially marginalized population~\cite{to2020they}. The authors discussed how various direct and indirect experiences of racially discriminating activities resulted to emotional and physical feeling of discomfort, embarrassment, and a perceived feeling of lack of belongingness with the broader community~\cite{to2020they}. CSCW literature also shows that the minority communities often respond to harms by constituting counterpublics; however, their activism are also responded with extended harms and harassment. For example, Salehi et al. conduct an interview-based study to explore how visible Muslim American public personas use social media platforms to constitute counter narratives by challenging dominant social media narratives that demonize Muslims~\cite{salehi2023sustained}. The authors find that the same platform affordances that are designed to empower users for ease of accessing the platforms, are weaponized against the minority social media users to harass and abuse the minority communities over a sustained period of time~\cite{salehi2023sustained}. The above and other studies~\cite{buss2022transgender, southerton2021restricted, pym2021still, paceley2022sometimes, simpson2021you} in CSCW deepen our understanding of the forms of marginalization, harassment, bias, and other negative experiences that minority communities often face on social media and other online spaces.


%On top of the existing inequalities faced by the minority communities, various intersectional minority identities causes more harms for the minorities. Scheuerman et al. for example shows how the minority trans population, who are woman of color or sex workers, are further abused and marginalized~\cite{scheuerman2018safe}. Feuston et al. studies trans people with eating disorders and find that the minority eating disorder community, who are also trans individuals are more vulnerable to online harm than others with eating disorders, as the trans minority communities have to continuously validate their identity~\cite{feuston2022you}. The authors argue that the feminine contents and cis participants are dominant within the eating disorder community and constitute the norms and standard on social media to discuss issues around eating disorders, where trans communities often challenge these norms and standards~\cite{feuston2022you}. Andalibi et al. studied LGBTQ and other gender or sexual minorities who (or their intimate partners) had an experience of pregnancy loss~\cite{andalibi2022lgbtq}. Through an intersectional and categorical analysis of the communities’ online experiences during pregnancy loss, the authors discussed how the combined minority identities of LGBTQ and pregnancy loss intensify discrimination and exclusion on social media platforms~\cite{andalibi2022lgbtq}. Haimson et al. study the non-normative SNS users who go through identity changes and find that various politics in categorization (such as gender) on the SNS’s interface could be a source of stress for the minority communities on socio-technical systems~\cite{haimson2015disclosure}. Overall, the studies about intersectional minority communities confirm how these communities with intersecting minority identities along the axis of race, gender, sexuality, and more, encounter a range of compounding harmful experiences including harassment, marginalization, bias, and violence. The CSCW literature however has inadequate insights (save for a few) into the experience of religious minority experiences of social media.


==> sections/findings_disregard.tex <==
\section{Findings}
We draw on the theories from social-psychological and cultural studies of fear to report three patterns of marginalization of the minority communities’ social media use: (a) the fear of Isolation and the spiral of silence, (b) the politics of fear, and (c) coping up with fear and marginalization. The theories provide us with the analytical lenses to analyze our findings as well as set the groundwork to draw from the same set of theories to discuss how CSCW could benefit from taking fear as a critical and design resource to make the online spaces safer for the marginalized communities.

\rifat{The themes below are in random order. Will organize soon.}

\subsection{The Social Psychology of Fear}
<intro: The spiral of silence - Noelle Neumann>

\subsubsection{Quasi-Statistical Organ: The Frequency Distribution of Public Opinion and The Feeling of Harmony}

The willingness of our participants to speak up or remain silent is significantly influenced by their perception and assessment of the social climate surrounding them. This pattern of minority communities' engagement in social media activities aligns with the principle outlined in the spiral of silence theory described as the quasi-statistical organ~\cite{}. People create self-censoring mechanisms in their decision making processes when participating in public discourse. They continually assess the prevailing trends, the frequency of voices that align with their own convictions, and the perceived reasonableness of those voices~\cite{}. By carefully observing the social environment, the quasi-statistical organ provides individuals with cues for evaluating situations where expressing their views may disrupt social harmony, thereby instructing them to remain silent.


Our findings demonstrate several indicators through which the social media users from the minority communities develop their quasi-statistical organs. <Talk about them>

% general idea is mixed: support, oppose, and silence.

\begin{quote}
    I really appreciated that when the Hindu communities were victims of the violence of 2021, several of my friends and seniors messaged me to say sorry, out of nowhere. They were not responsible for the violence or involved in anyways with those, and I was not a direct victim of those incidents. Still, they said sorry on behalf of others. They called me over the phone to check in with me.--AP7
\end{quote}

\begin{quote}
    I try to observe what others' opinions are, if what I know or think is already said by someone else. Some people approach such disagreement with nice discussion-like manner, whereas some people are biased toward their own religion. Some people are stubborn and aggressive who try to keep these conflicts alive. I feel it distasteful to interact with these people and wonder among whom we live.\hfill--AP5
\end{quote}

\begin{quote}
    The minority community has become more cautious on social media which was not the case before. If you think about political wings--left and right, there's also a swing wing in the middle. That's gotten stronger. Not everyone believes in radicalism. There are many good people in the Muslim community. After the incident of 2021 or other issues on social media, a wing has emerged who opposes communal ideas strongly--on online, still not in real life. 
\end{quote}

AP8 said that he received social support from only a few friends from the Muslim community. Rather he saw some post justifying the violence. This is what he said,

\begin{quote}
    When it comes to religion, people often become radical. So, people from both the Muslim and Hindu communities became partisan on that topic. It makes sense that the Hindus were victims of the incident, so they were telling their side of the story. But the people from the Muslim community who justified that vandalization, in my opinion, are hypocrites and brain-washed individuals. I don’t believe that they can respect liberal thinking or values.\hfill--AP8
\end{quote}

% AP7 talked about avoiding interaction with those who blamed the victims of communal violence.




\begin{quote}
    [Supporting climate/Silent observation] After the Prottoy’s incident, I was closely following the social media groups. You know the Prottoy’s incident, someone who put on a “tip” and that incited some unrest. What I found is, there were a lot of people supporting Prottoy. It was hopeful. There are actually supportive people out there. 
\end{quote}

\begin{quote}
    I see the situation around me, if and where anybody supports others. When you see that you are outnumbered, when there are ten people arguing against you and you are just listening, you won’t like to stay in those arguments. On top of that, arguments do not end on Facebook. Someone may make me a target even after the argument is over on Facebook. Then why should I go into a conflict. I should be even more careful. That is why I don’t engage into an argument. 
\end{quote}

\begin{quote}
    [Helps to connect - solidarity - support] As I told you that I am a non-believer. When this journey started, I couldn't really ask people around me, because that was risky. Social media helped in that regard. I could at least connect to some people like me.
\end{quote}

\begin{quote}
    Many people speak for us. But most of them are renowned people, like celebrities. Mass population, normal people, supported the incidents, which is fearful for us as a nation.
\end{quote}

\begin{quote}
    [Public sensmaking from others' social media activities] In last year’s pride month, the chairman of ten minute school posted a pride flag and said something like, happy pride month. I gave a live reaction to that post. One of my friends saw them and asked me on the messenger whether or not I belong to the LGBTQ community. [Say mockingly] Then he gave me a lot of lessons. Said, you have a love reaction to the post, but remember, it is never going to be legal in Bangladesh. After that, for my own safety, I give a lot of thought before reacting to a post.
\end{quote}


\subsubsection{The Fear of Isolation: Seeking Societal Approval and Maintaining Reputation}
The spiral of silence theory presents a social-psychological concept of the public sphere, which the author characterizes as a ``social skin’’~\cite[]{}. Within this framework, people exist within a society where they are consistently subjected to the scrutiny and evaluation of what the authors refer to as the ``anonymous court’’~\cite[]{}. As people develop their quasi-statistical organs to assess their social environment, the fear of isolation, disrespect, and unpopularity among the dominant group serve as guiding forces, compelling them to conform to the established social norms embodied in the ``social skin’’ and actively seek social signals of reputation.

\begin{quote}
    I was talking to one of my friends and the conversation was going well. Suddenly we talked about religion and I said I am an atheist. Then he started to say how even is it possible. God is only one and we are the truth, etc… You should learn about Islam. If you read Quran you would [find] all the answers you are looking for. They would just forcefully tell me to read Quran to find all the answers whereas I was continuously telling them I do not want to read Quran. ... So, usually they got pissed off and stopped talking to me. Because they could not find any common ground to talk anymore. In this way, I have lost so many contacts. I ware not disrespecting them. I was just clearing my point of view and moral ground, which differed from theirs. They stop contacting me because I am not Muslim or do not believe in God.\hfill--AP1
\end{quote}

\begin{quote}
    I have some friends whose families are religious, I mean, practicing Hindus who observe the rituals–not for showing off but sincerely. But when they come to campus, because of being afraid, they try to prove themselves secular in front of [the Muslims] and do not participate in the religious programs on campus. To avoid being separated out or keep their connection with them [the majority community] safe and sound, they act secular. They will not present themselves as Hindus, which is problematic.\hfill--AP7
\end{quote}

\begin{quote}
    [Intersectional identity] I keep getting defaming message requests even from my own Hindu friends on my Facebook profile because of my gender identity. It used to make me feel really bad two to four years ago. On one or two occasions, I even had heated massages with people. I blocked people. Now, I have my support system around me. I can choose not to care.
\end{quote}

\begin{quote}
    [family and close relatives as a ``court''] My family does not know that I have social media profiles. There is a special reason for this. My family is conservative or semi-conservative. Now, when I run a social media profile, I want to be myself there, which my family might not like. I don’t let anyone stay on my profile who may hamper this [being thyself]. Now, my instagram is fully filtered. I don’t have anyone on my Instagram where someone will hear something from me, you know, my opinion, my reflection on something, and then will judge me. 
\end{quote}


\begin{quote}
    [Venting out to friends] When I see controversial posts, I don’t just react. As I mentioned before, the way I was brought up, there was always this impression that I cannot be identified as someone different in the community. You know, there was this time in Bangladesh when being Hindu was risky in Bangladesh. You know there was a lot of violence at some point. From then, we have learned that we cannot say anything out loud on social media. When I see a post, I get hurt, I feel the feeling in myself, and I just choose not to react. I just go to my friend’s inbox and create a conversation about it. 
\end{quote}


\begin{quote}
    Well, most of my friends are not Hindu. I have to get along with society. My [non-Muslim] friends are so close to me that we even share food from the same plate. I have received so much support from them, professionally and morally – I cannot ignore their contribution in my life. Just because there are some evil people out there, I can't or won’t make my relationship uncomfortable with my own friends. 
\end{quote}

\begin{quote}
    [lack of visible public solidarity further isolate people] Take the example of the religious debate of eating pork or beef. If you look around you in real life, you will obviously see people supporting you whatever you decide in terms of eating beef. But the same people would be silent on social media. It feels like I don’t know them. It [the silence] gives encouragement to those to spread hatred.
\end{quote}

\rifat{Fear or Isolation and seek for validation and reputation: Discuss our findings}

\subsubsection{Stereotypes and Unconsciousness of Perceiving the Social Climate and Reinforcement of Spiral of Silence}
The social psychological process of the spiral of silence is accelerated and intensified through social and mass media. The development and spread of both positive and negative stereotypes on social media can further contribute to silencing marginalized communities~\cite{}. Stereotypes have a natural characteristic of spreading quickly and at scale on social media platforms. However, stereotypes also tend to dissipate rapidly but leave an influence on shaping public opinion. The author describes such rapid appearance of stereotypes as ``storm clouds’’~\cite{}; people who directly do not experience the changes of the social environment due to stereotypes are unable to perceive and respond to the changes. Consequently, stereotypes create a more unstable interactive environment for religious minority communities.

\rifat{discuss our findings}
\begin{quote}
    In our everyday life, everything is social media based. It can manipulate us and bring good also. Sometime we get manipulated seeing posts in social media. For example, I have a believe and after seeing any post I started to think it makes more sense. So, this has effect in making the situation vulnerable. We can not calm them down as damage is done.\hfill--AP1
\end{quote}

\begin{quote}
    Actually, this [Ramu's incident in 2012] is a planned incident. Like, what was posted at the time of the Ramu incident was posted by a fake account. And the person who was accused of this had no idea about it either. The same kind of thing happened to you all [referring to Hindus in Cumilla, Rangpur in 2023] as well. 
\end{quote}

% Practices that are stigmatized, mocked: Idol-mediated worshipping** (mentioned by all so far), worshipping female deities, incorrect narratives around or interpretation of religious events from an outsiders angle, eating pork, not eating beef

\begin{quote}
    In our religion, we worship through idols. But in their religion, they think that it is just an idol. How much can it do for you? At the end of the day, what’s the point of talking to it, sharing your problem with it, or asking for anything from it? So it’s funny to them. One more thing is that taking pictures is not allowed in our pilgrims. But in recent times, I have seen some pictures that have been taken, even imitating the posture of the idols.\hfill--AP3
\end{quote}

\begin{quote}
    people from outside of the Hindu faith often talk about Hindu practices. Some people from the Muslim community often say vulgar things about our female deities, often in Waz mahfils, which creates discomfort in me. Let’s say there are 100-150 people at a waz who are coming out of that event, getting a negative impression about Hinduism, or are influenced to think of Hindus in a negative way.\hfill--AP8 % Similar to this, AP7 talked about hujurs in rural areas who spread radical views in khutba after Friday's prayers.
\end{quote}


\begin{quote}
    they generally have some curiosities. Like what is my lifestyle, what religion I follow, where my house is, what it looks like etc. 
\end{quote}


\begin{quote}
    There are a lot of misconceptions. I often see posts where people say that Hindu people don’t eat beef because they recognize cows as their mother. [laugh]. This is not like this. There is a long history behind this. It is just misrepresented [...] Another controversy is about the celebration of Pahela Baishakh. Many people take this as a Hindu festival. But if people were educated enough, they would have known that this is just a Bengali culture. 
\end{quote}

\begin{quote}
    [Aesthetics/looks/stereotypes] My beard has been problematic on some occasions. Some people keep telling me to be Muslims. Even some of my friends asked me to be Muslims in some occasions. 
\end{quote}

\begin{quote}
    [Family] My brother is a conservative and religious. He likes to follow religion and culture more strictly. If any conflict happens and you go ask him who he is going to save, he is probably going to tell you that he will prioritize his Hindu friends. What can we do? We have to be together in society, right? My mom is better though. When my Muslim friends come to our house to hangout, my mom happily cooks for them.
\end{quote}

\begin{quote}
    I have been on Facebook since 2010. In the beginning, I was very vocal. But it feels like nobody is willing to listen. I can give you an example. Someone read a book, I don’t know what book, that says that a Hindu can eat beef. Now they come to me and tell me, hey why don’t you eat beef? Now I can take a quote from Guita, and tell them why I cannot eat beef. But it feels like they won’t listen to that. Instead, they will be ready to bash me once I post this. When I understand this, it does not make any difference if I say anything, I stop saying anything. 
\end{quote}

\begin{quote}
    [Cultural stereotypes] A year ago, I posted something about wearing ornaments. I said that men can also put ornaments on their ears. Some of my friends from my hometown started saying negative things in the comment and also sent me texts. However, I did not have the mental situation to speak up. Surprisingly, some of my friends from the virtual community, who I didn't even ask, came forward and started defending me. I did not expect that.
\end{quote}

\begin{quote}
    There are also some people [Muslim religious leaders] try to assess what kind of things people prefer. If something is popular or triggering, even if it's incorrect, they will propagate those. [Religious preachers in Islam] all talk about how their religion is better than everyone else's. There are also some of them who discourage insulting other religions. They talk about differences but encourage harmony. ... However, they are very few in number, say one in a hundred. ... Different speakers preach different interpretations. ... Honestly, when it comes to religion, people are overly sensitive and often highlight the negative sides of others for social or political reasons.\hfill--AP5
\end{quote}

Another source of silencing stems from the unconsciousness of the influence of social media in public interaction~\cite[]{}. The author explains that, in their engagement with the social environment, people tend to simplify the complexity and subtlety inherent within it, constructing a simplified model of the social environment. In this process, individuals often rely on consuming indirect experiences and conflating them with their own perceptions in order to comprehend the social environment. Consequently, people reach a point where they are unable to differentiate their own perceptions from those of others~\cite[]{}. In other words, the influence of indirect sources of public opinion, such as mass and social media, becomes invisible to them to form public opinion.

\rifat{discuss our findings}



\subsection{Politics of Fear and Social Control}
<Politics of fear - Sara Ahmed>
The spiral of silence theory provides insights into the social psychological patterns through which religious minority communities subconsciously or unconsciously regulate their behavior on social media leading to marginalization. Our findings show that such fear is facilitated through a power relationship between the minority communities and South Asia's broader social, cultural, and state institutions. To examine this pattern of the political aspects of fear, we turn to Sara Ahmed's influential work, ``The Cultural Politics of Emotion~\cite{}.'' Ahmed's theoretical approach to explicate the intricate relationship between power and politics of fear gives insights into how fear is frequently employed by socially powerful entities as a means of control. This framing of the politics of fear allies with the spiral of silence, as Ahmed highlights the political dimensions of fear and its role in perpetuating social marginalization. Such a framing of fear emphasizes the political aspects of fear and its role in social marginalization. Drawing on the theory, we discuss <> below.

%Our findings demonstrate that these communities are also victims of external fears from religious and cultural institutions that exert political control over them. 

\subsubsection{Economies of Fear}
Drawing on the political theories of Machiavelli and Hobbes, Sara Ahmed discusses how fear has been used historically as an instrument for disciplining, punishing, and governing the less powerful by the people upper in the power hierarchies~\cite[p. ]{}. Civil societies also use fear as an instrument for protection as in the promises of freeing people from fear bring freedom. Beyond the forms of controls by states and power-hungry individuals and institutions, Ahmed also discusses fear as a ``symptom''  of modern life. Drawing on Furedi~\cite{furedi2006culture}, Ahmed explains how fear has made people hyper-conscious about the age-old values and traditions, where people anxiously and rapidly change their habits, norms, and behaviors to manage and live within a culture of fear to conform to the ``modern'' ways of being. On top, Sara Ahmed presents fear as a boundary-defining emotion between the ones that are threatening and the ones that are threatened~\cite[]{}. In other words, Ahmed describes how fear originating from power politics of the dominant and power-hungry people and institutions may marginalize a community by creating artificial insecurity, stigma, and stereotypes.


\begin{quote}
    I have already told you about an app called Rave. On that platform, I am friends with both Indians and Pakistanis. ... Hindu Muslim conflict was very usual on Rave. It is like a universal conflict. There Indians automatically thought that I was Muslim because I am Bangladeshi. Then they started to say bad things about Mohammad. ... Again, many Muslims say bad things about Hindus.\hfill--AP1
\end{quote}

\begin{quote}
    There was no violence in our district during Durga puja because security from government was strong--neither in villages nor town.\hfill--AP5
\end{quote}

\begin{quote}
    Division among Hindus and Muslims existed before partition of India and Pakistan. Has it brought anything good? If people continue those sentiment, if Muslims burn down Hindu houses and temples, in India where Muslims are minority, they will have to face troubles. It's not right what many Indian Hindus or Bangladeshi Muslims do to their minorities.\hfill--AP5
\end{quote}

%vulnerable and out of control

\begin{quote}
    \rifat{We can present it as a case} There are several Facebook and Instagram Bangladeshi Queer secret groups. At one point, I had a sexual interaction with someone, when he was 20-21 and he was 17 or 18. After a few years, they made an allegation that I forced myself into him, along with several other allegations. At one point, they started posting this from several groups. After two or three days, I realized that I have to clarify myself since this is a big allegation.” The participant then went on explaining how they wanted to clarify themselves with screenshots and other proof, but did not get support even though they had support from some of his close friends. Finally, when they told the people in the secret group that they are going to take “necessary [legal] steps”, the participant heard a counter threat because of their identity, “I can clearly remember what I heard – they said, spare yourself from the hassle of police. You being yourself as a homosexual person, you will get in trouble.” Now think, it is happening in a secret queer group. Who said this also is a renowned person. She also works with human rights and feminism and LGBTQ rights. Now think, when I am asking for my own justice, they are threatening me for being a gay. I kept a pdf of that post and my evidence. Sometimes people who I don’t even know keep asking me questions. Then I give them these documents. 

\end{quote}


\begin{quote}
    [Social media groups admins exercise power] When they [the secret group member] were spreading this news, they were saying that it is my verdict. My question is, how could you give a verdict and jeopardize my social life, when you are not a law enforcing agency? You just run a Facebook group! I could take a step. But if I did this, a lot of people would have suffered. 

    Now…these people harassed me on social media. They don’t just stop there. They also do the gatekeeping. Now, we are a minority, we are powerless in society. We want freedom, we want ourselves to be heard. We open these groups because of that. What happens after? People who become moderators, admin, you know the powerful faces, they make their own elite circle among us. They do it whatever the way they can. It could be gatekeeping, defaming, or whatever else. 
\end{quote}

\begin{quote}
    I remember the last time I went to the temple with my friends, I saw the news of temple attacks and attacks on the Hindu community spread out on Facebook. For a moment, I thought that it might not impact us. Then again, I realized that nobody is even gonna try to know what is in my mind – whether or not I am innocent. I will just get attacked. This is how I feel in incidents like this.
\end{quote}

\begin{quote}
    I did not receive any threats myself but my family members did. Once there was a big riot before we were born [was referring to the riot incited by Babri masjid demolition in India in 1992]. My cousin told me that the chacha [Muslim neighbor] who had a good relationship with us till two days before, they rushed to our house to beat my uncle. The good relationship they had changed for worse all of a sudden. My family faced such things, not me personally.\hfill--AP5
\end{quote}

\begin{quote}
    there was a story of Holey Artisan where they made people say Surah and killed them if they could not. ... There was an incident that also suffocated me. Do you remember in a mosque in Bangladesh, they burnt a man alive and killed him? It circulated on social media and nobody did anything. For just falling the Quran on a person's feet, people burnt him. After some time it was revealed that, he did not do that intentionally. Nobody deserves to die that way. So these made me feel sad.\hfill--AP1
\end{quote}

\begin{quote}
    Political leaders have to take a middle ground. So, they usually show sympathy to the victims of such violence. But administrative bureaucrats like DC and SP, do not need to do that. So, they show what's in their minds. In my district, some people did not give permission to observe the Durga puja, but others, many Muslims, convinced them and helped us organize the puja event.
\end{quote}

\rifat{discuss our findings}
\begin{quote}
    I think the reason behind the conflict [in 2021] was political. If you think about it, whoever belongs to the minority community in a country, usually tries to save themselves, be that Muslims in India or Hindus in Bangladesh. So, in Bangladesh, no Hindu person would not dare to agitate the Muslim community. So, I think it was done by political motivations of any fundamentalist Mullahs or someone like that. Otherwise, it could not happen. ... Recently, during Durga Puja in 2021, when they started vandalizing the idols, I felt like an inferior person and a constant fear was in my mind.--AP8
\end{quote}

% AP7 talked about VC's intervention to cancel the auditorium reservation for Mahalaya (a religiously influenced cultural program). However, he also mentioned support from other teachers, administrative stuffs, and DSW, from both faiths. The outcome of the negotiation was a closed-door program. A friend of his informed him about and showed a photo of a meeting that took place in a mess about interrupting the program. They later identified those individuals to be politically motivated outsiders. So, he had to take some measures for security around the critical entrances during the program, especially for the female students. When the program was completed, people were appreciative of the program, and Hindu students who present themselves as secular also thanked him for this effort.

\begin{quote}
    When I used to get posts ridiculing my religion, I used to comment and make my arguments. But later I realized that it is not good for me in the long run. It may instead grow anger towards me. Recently, you have seen many incidents [he was referring to temple attacks]. Now, we are even more careful. I am even careful in using public wifi. I always log out from Facebook and Instagram after I am done using them. 
\end{quote}

\begin{quote}
    [waz as a panopticon] Not only posts, I have seen many waz videos, where they tell even out loud that it is permissible to attack and rob from people having other religious affiliation. I have seen many such comments like this. The follower base of these preachers are so strong that you fear starting an argument, let alone convincing them that their hujur [preacher] said something wrong. 
\end{quote}

% AP2 and AP8 talked about how communal dynamics in neighboring countries affect the social psychology and fear of religious minorities in Bangladesh. AP8 talked about Muslims' marginalization by Hindu nationalists in India and AP2 talked about the Rohingya genocide by Buddhists in Myanmar. AP2 said, ``When the Rohinga refugees came, they mainly came from Myanmar. Myanmar is mainly a Buddhist country. So, we fear more now, thinking, if they want to take revenge of their oppression from us, the Buddhist community in Bangladesh." 

\begin{quote}
    We are basically facing it from very early age. We have been seeing this for so long! And I have realized it more clearly after the incident of 29th September [in 2012]. I basically have some distress also. ... Because those who do this, basically do it out of ignorance or unawareness. Those who are understanding, and properly educated, won't do this type of stuff. And it's not like no people support us. ... The things that have been destroyed, have been rebuilt very beautifully. Since I am from Ramu, I know well, those who had faced casualties, had been helped enough. But even after reestablishment, the fear never really fades away from the mind. ... On 29th September, when they were coming to set fire, they were giving some slogan, that I can't clearly remember. On that night, I along with all my other relatives, were sitting in the courtyard, all helpless, thinking about where we are living! That night is like the worst nightmare in my life! I don’t talk about it usually.\hfill--AP2
\end{quote}

\begin{quote}
    I have brought up in a place, which actually has harmony between communities. In every village of Ramu, they attacked. But they couldn't enter our village. Our chairman was very supportive of us every time. They even said things like, before harming us, the attackers had to harm them. Since I am seeing them from very early childhood, I respect them a lot.\hfill--AP2
\end{quote}

\subsubsection{The ``Uncertainty'' of Future and the Impression of Fear in the Present}

Ahmed describes that the ``object'' of fear does not necessarily have to be present ``here and now''~\cite[]{}. Rather, an anticipation of an uncertain future makes people fearful in the present.

\rifat{discuss our findings}

\begin{quote}
    There are several posts where you can see that people try to portray the superiority of their beliefs. Not only on just Facebook, you think about Waaz Mahfil. Whether you want to hear it or not, you have to hear it in Bangladesh because there are several speakers at every turn. Often, they talk about minorities and show how inferior are they. So ignoring these became a habit of minorities in Bangladesh. There is nothing to do and we are scared. If we try to say something, we will get threats and it happens. ... If anyone says a simple thing about Mohammad, people get so triggered. But they talk about Jesus Christ and why Christianity is bad. They talk about why celebrating puja is bad. How Hindus make no sense.\hfill--AP1
\end{quote}



\begin{quote}
    [Community leaders] try to solve. But that is not very effective most of the time. This is a reason, why people in our community are decreasing in numbers. … among them, those who are good at studies, think of going abroad. That is better than living here as a minority. Not like, everyone can go. Those who have that ability, are going.\hfill--AP3 %AP2 also said similar things about leaving the country for safety.
\end{quote}

\begin{quote}
    There has been a problematic change in the education sector. Curriculum in no class/level makes us conscious of this [the rising communal polarization]. They do not mention it, and even if they do, they avoid discussing the risks of it in detail. … They are also removing famous Hindu writers’ writings from textbooks. These impact and will impact the scenario. … General people like farmers and laborers are suggested to see themselves as Muslims only, not as Bengalis. Then the religious leaders will use those people for their self-benefit which will be the worst.\hfill--AP7 %same doubt about religious leaders' positive role in promoting harmony was echoed by AP2.
\end{quote}

\begin{quote}
    I did not see any religious leader to come forward and say this is bad and we need to stop this. The role of religious leader in our country is huge. In a waz mahfil, if a preacher say Ronaldo is bad then he is bad. No one will give a second thought. 80 out of 100 people would start to believe it without any question. In waz mafil, people get manipulated in wrong way. In Bangladesh one of a huge source is social media. ... If religious leaders start to tell people to be tolerant, then it would really help. Most of the people in our country look up to them and they are their ideal character. They follow them. We never saw any major religious leader to say to empathized or to forbid to do such things.\hfill--AP1
\end{quote}



\begin{quote}
    Why would I read about Mohammad mostly in Bengali books? I do not want to. I can read about Buddha. What if I want to read about Buddha, Jesus Crist or Krishna? If there is an article on Mohammad in our book, then there should be article about others. If I read about Mohammad in Class 6 then I should read about someone else in class 7. But almost every year there is atleast a chapter on Mohammad. How are we establishing secularism?\hfill--AP1
\end{quote}

\begin{quote}
    After the incidents of 2021, I saw many posts about it on social media, but very few of those were from the majority community. That’s why I fear that Bangladesh is gradually moving toward religious radicalism. The process has already started, Bangladesh is the next Pakistan.\hfill--AP8
\end{quote}

\begin{quote}
    When you first resist those stereotypes, that's the hardest part. Once it's broken or the reality is normalized to everyone, then the conversation becomes easier. ... However, there is a huge risk factor. That's why, I am motivated to keep a political background. Because, if I am non-political, no one will come to give me any backup.\hfill--AP7
\end{quote}

% AP2 and AP7 talked about the declining percentage of religious minorities. They mentioned religious conversion as a major concern.

\begin{quote}
    [The 'sign' of fear] I did not feel anything in Dhaka, but when I went to my village during the last Puja, it was a difficult time. People were getting together with safety measures to guard the temple. I liked that some Muslims also joined them. However, I could feel the fear. You know kirton, it is like waz for Hindus. People in the temple did not even use a mic, they were doing the kirton in a very low voice.
\end{quote}

\begin{quote}
    [Fear/numbers] You don’t see many things on the mainstream media, which you will know from friends or social media. For example, from the recent survey, you will know that the number of Hindus is declining. Why does it happen, you think? People are leaving. You don’t know about this information from the mainstream media, but you will know that from some social media posts. 

\end{quote}

\begin{quote}
    [Lack of visible action makes them more afraid] You could say I am a silent spectator now. I avoid sharing or posting something. It often happened that someone opened a fake ID pretended to be a Hindu person, posted something that led to violence targeted toward Hindu community, and nothing happened after that. The person who opened the fake ID is not identified or jailed. In such a situation, those who want to speak up are painted as someone who is trying to spread chaos. Which is why I try to be silent. 
\end{quote}

\begin{quote}
    Actually, I have rarely engaged in religious conflict on Facebook. I know the situation in Bangladesh for example death threats, rape threats, and hatred of some random human. Usually, I post and I have noticed how people threaten them if someone posts against a religious belief. They start to objurgate and demean. So, I kept myself away from these things.\hfill--AP1
\end{quote}

% AP7 and AP8 talked about their families' fear and how that drives their family conversation and guidelines for not getting involved in religion-related debates online. The fear is often driven by what happened in the neighborhood, in the country, the history of partition, and in the case of AP1 and AP7's case, death threats.


\begin{quote}
    I do it only on instagram. Because if I do it on facebook, my seniors, my classmates, all are observing me. They might come handy in future. They might be helpful for me, in my career. If I make them upset now just because I want to be myself, then I would get some backlashes in future.
\end{quote}

\begin{quote}
    
    [Caution from the family] My parents don’t use Facebook. Despite this, they keep alerting every now and then. Because they notice many incidents reported on TV or newspapers. From these, they also are fearful and alert me. They are especially worried because of my religion. There are also a lot of political issues. In these issues, about religion and politics, if you react or give your opinion on social media, you are actually getting into trouble.
\end{quote}



\subsection{Coping up with the Culture of Fear}
<The culture of fear and CAT>
Our participants exhibited various coping mechanisms in response to the social and psychological fears associated with isolation, uncertainty, and negative emotions. To illuminate this third pattern of findings, we draw upon the communication accommodation theory (CAT)~\cite{}. CAT has been a highly influential theory over the past several decades, offering valuable insights into interpersonal and intergroup communication dynamics~\cite{}. It provides a socio-psychological perspective on the significance and impact of power dynamics and micro-contextual factors in adjusting their behaviors in intergroup communication ~\cite{}.

According to CAT, people adjust their communication behaviors through convergence, divergence, and maintenance strategies. Convergence occurs when people seek approval or when the cost of conforming is low~\cite{}. Conversely, divergence is observed when individuals intentionally differentiate themselves from others in communication to highlight their identity differences~\cite{}. The motivation for communication accommodation includes the desire for social approval, the reinforcement of one's identity, and the aspiration to influence others to align with one's perspectives. These communication accommodations are influenced by micro-social factors such as the historical relations between groups, status, demography, and institutional support~\cite{}. Individuals often strike a balance between the 'desire to belong' and the 'desire to be unique' when adapting their communicative behaviors. Moreover, accommodation extends beyond linguistic behaviors and encompasses para-linguistic, discursive, and non-linguistic cues.

\begin{quote}
    [Social media as a learning tool to address homophobia] I was talking to a friend of mine, who is a medical student in Bangladesh. The other day I was talking to him about gender diversity. I told him how the gender could be many. He was like, no, our teachers teach us three genders, where do you get all this information about diversity in gender. Now, if a doctor, who is educated, holds this kind of belief, think about the mess population. I think social media could be helpful in this, to educate people. 
\end{quote}

\begin{quote}
    A few years ago, someone posted a meme that ridiculed one of our major festivals, maghi purnima. I posted a comment there indicating how much problems and ridicules we face from the bigger religious communities in Bangladesh. Following that comment, I received some threats on my inbox; someone told me that they are going to report my account, post my picture to secret religious groups, etc. Following that incident, I stopped posting anything that might trigger anger among other religious communities. My profile was public back then. I made it private after the incident. 
\end{quote}

\begin{quote}
    [minimizing/controlling damage] They try somewhat. But how much they could do. When it [the communal violence] happened, they privately called people they knew and told everyone to go home, or stay home if they were already home. They just tried to control damage as much as they could. At the end of the day, they don’t have the power to do much either.
\end{quote}

\begin{quote}
    [Fact-checking is ineffective – trying to flood social media with the “truth”] Trying to fact-check something to me is a fruitless effort. If you try to fact-check from social media posts, you will have to check who said what, how many people said, what sources they are using, etc. Instead of trying to do this, if people just came forward and try to flood social media with “truth” along with appropriate sources, that could have been more helpful.
\end{quote}

\begin{quote}
    [It’s a vicious cycle] It is a vicious cycle. Something is happening, and we are making our post private and discussing that less. People are not seeing them [the conflicting situation] anymore. Now, if people don’t see the conflict anymore, how come they are going to know about it! If people see the conflict, some progress will be made. Let’s say, 90\% of people will not change their viewpoint from a conflict, but 10\% will. If we are making our posts private, we are not letting them see our posts. We are not giving them the opportunity to change their opinion.
\end{quote}

\begin{quote}
    [Venting out to friends] When I see posts, obviously I take a position. But I don’t engage on social media. I learn the post and then take them up to my friends and close circle and discuss with them. Yes, the defaming posts bring anger and sadness. Definitely, if someone talks badly about my religion, it makes me sad. But generally, don’t do it on social media. No one knows who might see my comments.
\end{quote}
\subsubsection{Convergence}

\subsubsection{Divergence}

% Participants seemed to talk about their bad experiences in school life. They often debated with differing views then, however, they mentioned, such incidents do not happen as frequently as earlier at university level.
\begin{quote}
    [Divergence] I have had to experience similar issues before. In the beginning, I used to post publicly. But now I don’t do it anymore. I share posts only with my close friends. Let’s say if I posted a picture in front of my temple, I used to share that publicly. Pictures even like that used to get a lot of negative comments. Now, as I post them only to selected people, I don’t have any backlash anymore. 
\end{quote}

\begin{quote}
    I gave a status. The status was like this...Bangladeshi atheist people and their obsession with Hindu religion was an ultimate level of hypocrisy. This post brought me a lot of backlash. [...] Now, they are comparing Islam with Hindu religion. Even though they don’t participate in Hindu rituals, they join the Hindu festivals to support them. Now my perspective is [with a laugh], if you are an atheist, you should have a neutral stance about every religion. You should not have any soft corner for any other religion. Being atheist means you should not believe in any religion. So, I engaged into a lot of controversy from this argument. 
\end{quote}

\begin{quote}
    I have seen this tendency [of debating about religions] among my school friends. I tried to ignore those so it does not become something significant. They usually try to convince me through pressure and convert my religion. They will probably tell me that my religion is wrong. I could have said something in response, but I never opposed them completely. Because I know it won’t work because his brain is already set up to think in a certain way.\hfill--AP7  %AP1 also shared a story from his experience of being socially pressured for religious conversion.
\end{quote}

\begin{quote}
    several times few people told me that the basis of Christianity is false. Because, they believe in Jesus Christ in some another way which different from whole believe system of Christianity. They tried to say that they are the only true religion and we have answers to everything. All the other religion is not true. Once, when I was little probably at age 15, I was talking to a guy and he made me say a Surah which is [Kalima Tayyabah]. Then he said you became Muslim. They I asked him "How do I become Muslim?". He said that you just said. Then I said if it does not come from my heart, how can I be muslim? These are some stories which I remember.\hfill--AP1
\end{quote}

story from AP7: A social acquaintance from the Hindu community posted about the history of historic communal riots in Noakhali and Kolkata and how those marginalized Hindu communities. A Muslim friend blamed the Hindus for those riots. The participant and another friend rebutted that claim and discussed the history with references. After some exchanges, they stopped, and both parties eventually ignored that thread.


\begin{quote}
    I google it or check bible verse. There are 6-7 fathers and sisters in my family. If I get to meet them then I ask them. For example, there is a clash regarding holy trinity. Muslim do not understand this and there is a clash. Then I try to gather information and pass it. I do not take information from unreliable source.\hfill--AP1
\end{quote}

==> sections/introduction-n.tex <==
\section{Introduction}
\label{sec:introduction}
Despite the initial promise of social media platforms to foster the coexistence of diverse communities, ensure equality of voices in public deliberation, and provide a safe space for participation, these platforms have become unsafe spaces for minority communities -- the religious or ethnic groups that constitute a smaller proportion of the overall population within a particular society or region~\cite{jackson2005minority}. Over the past decade, as social media platforms gained popularity, the issue of inequality and online harms based on cultural, faith, and identity-related factors, including race~\cite{ogbonnaya2020critical, smith2020s}, caste~\cite{vaghela2021birds}, gender~\cite{bardzell2011towards, scheuerman2020we}, and religion~\cite{mizan2019silencing, rifat2020religion}, has received significant attention in academia and public discourse. Academia and the media have reported on how social media platforms have introduced and propagated new forms of online violence targeted at religious minority communities in the Global South~\cite{Human_Rights_Watch_2021, Hasan_Macdonald_Ooi_2022}. For example, over the past few years, a common pattern has emerged in which rumors defaming the holy books of Islam are spread from profiles pretending to be Hindu individuals, resulting in mob attacks on Hindu religious establishments and homes in Bangladesh~\cite{Hasan_Macdonald_Ooi_2022, Ethirajan_2021, VICE_2021}. During the COVID-19 pandemic, fake videos claiming that Muslims are deliberately spreading the virus went ``viral'' on social media platforms in India~\cite{bhatia2022discursive, Human_Rights_Watch_2021, Regan_Sur_Sud_2020, The_Washington_Post_2020}. These false videos led to physical abuses of Indian Muslims and hindered their businesses, as many people boycotted them~\cite{Human_Rights_Watch_2021}. In Bangladesh and other South Asian countries, organized misinformation tends to focus on religious sentiments, unlike in North American regions where misinformation is primarily targeted at politics and electoral systems~\cite{haque2020combating}. Rumors, fabricated images, and targeted memes are frequently posted from social media profiles impersonating members of minority communities, with the aim of inciting social violence South Asian countries~\cite{haque2020combating, kaur2018information, dash2022insights, minar2018violence}. Several incidents of social media-incited mob violence have resulted in the killings of individuals from minority communities~\cite{Hasan_Gooding_Dayant_Johnston_2017, roy2023sociological, al2021content}. In the extreme examples, social media has been found to be complicit in incidents of ethnic cleansing~\cite{Amnesty_International_2023, The_Guardian_2021}. These forms of online harms and violence, magnified through social media, have alarmingly escalated, making the lives of religious minority communities worldwide unsafe due to the instilled feelings of fear, intimidation, and anxiety.

%Despite the initial promise of social media platforms to foster the coexistence of diverse communities, ensure equality of voices in public deliberation, and provide a safe space for participation, for minority communities-- religious or ethnic groups that constitute a smaller proportion of the overall population within a particular society or region~\cite{jackson2005minority} -- these platforms have become unsafe spaces.


%In this paper, we particularly focus on the predominantly Muslim-majority (91.04\%) Bangladesh's religious minority communities, such as Hindu (7.95\%), Buddhist (0.61\%), and Christian (0.30\%)~\cite{bbs2022preliminary} and their experiences on social media platforms.

%around the world 




%Further, the ethical, political, and cultural aspects of faith are seldom considered in CSCW literature of faith-related online harms. 


While CSCW and related disciplines have made significant contributions to understanding and mitigating various forms of online harms for racial, linguistic, and other forms of minority communities, many of which are primarily based in the West~\cite{ogbonnaya2020critical, pyle2021lgbtq, erete2021can}, research in this domain is still limited by a lack of understanding of the contextual, social-psychological, and political aspects of social media use experienced by religious minorities in South Asian regions. We argue that studying the social media use and the unsafe experiences of religious minorities in South Asian countries separately from other forms of minority experiences, such as the well-documented CSCW literature concerning racial minorities in the West~\cite{ogbonnaya2020critical, rankin2021black, musgrave2022experiences}, is important for two primary reasons. First, whereas racial minorities' identities are primarily built on individuals' ancestral and genetical background~\cite{helms1994conceptualization, mcintyre1997making}, religious minorities' identities are based on their beliefs and social practices~\cite{fox2000religious}. Factors such as the perceived threat posed to the worldview of majority groups by the actions of minority groups, the use of religion in political legitimacy, and the influence of religion in ethnic conflicts strongly influence the experiences of ethno-religious minorities~\cite{fox2000religious}, which cannot be accurately characterized by discrimination faced by ethnic minorities alone. Second, unlike the race-based social justice concerns that are comparatively more prevalent in most of the West, social justice concerns in South Asia often revolve around faith-based issues~\cite{nandy1988politics, das2001remaking, rifat2020religion, mim2021gospels}. Religion has played an influential role not only in state politics in South Asian countries but also in socio-cultural politics in everyday life, due to its deep intertwining with the history and culture of the region~\cite{robinson2000islam, nandy1988politics}. These unique dynamics may not be fully captured when analyzing minority experiences where race, language, gender, or other factors have been the center of attention. 

%Due to the differences in identity, the experiences of religious minorities are strongly shaped by religious influences~\cite{fox2000religious}

Despite these differences, modern human rights frameworks tend to collapse all forms of minority rights under the single umbrella of minority protection rights~\cite{ghanea2012religious}. Moreover, when religious minorities face discrimination, their cases are often handled under the category of ``freedom of belief or religion'' instead of minority rights~\cite{ghanea2012religious}. CSCW literature shows a similar pattern, where religious aspects of minority experiences are often collapsed into other cultural and generalized minority categories, as evidenced by a substantial body of work where religion is considered in the periphery of analyzing online harms (see, for example~\cite{shahid2023decolonizing, mustafa2020patriarchy}). For these reasons above, we argue that the religious aspects of minority experiences are not merely a reflection of cultural, ethnic, and racial experiences but require distinct and separate attention to fully understand the safety and vulnerability of religious minority communities on social media.

%While societal power impacts racial identities, religious identities are more malleable due to the exposure of alternative beliefs, ideologies, and the scope of voluntary choices. The latter's susceptibility to societal power dynamics is evident through unique kinds of attacks and suppression of religious minorities' practices in different geocultural contexts.



To this end, we conducted an interview-based study involving three Bangladeshi religious minority communities to comprehensively understand their experiences of using social media platforms. Informed by our findings, we place ``fear'' at the center of our analysis when examining the experiences of religious minorities in their use of social media in Bangladesh. Our findings reveal three dominant patterns: first, the constant political and social psychological influence of fear within religious minority communities on social media platforms; second, the imposition of fear onto minorities by majority groups and social institutions; and third, the continuous adaptation of social media use by the communities based on their anticipation of future fearful consequences. The insights related to fear is also informed by the long history of the politics of fear concerning religious minority communities in South Asia. The strong religious influence on nationalist politics in the Indian subcontinent has utilized the politics of fear to justify anti-minority violence in the region~\cite{anand2016hindu}. The online harms incited by social media often align with hyper-nationalist majoritarian political ideologies in South Asian countries~\cite{dash2022insights}. For example, in India, Hindu nationalist politics known as Hindutva perceives religious minority groups as a threat to their identity, thus creating a stereotypical image of these minority groups as dangerous~\cite{anand2016hindu, shani2021towards}. Due to these perceived threats, the majority religious groups portray minority religious groups as ``anti-national'' \textit{Others}~\cite{dash2022insights, islam2007imagining, oommen1986insiders}. Similar strong intertwinings of religions and politics continue to fuel the politics of fear in other parts of South Asia as well~\cite{mohsin1984religion, riaz2016bangladesh, fair2012faith}. This politics of fear socially constructs hate against religious minority communities in South Asia, and justifies social surveillance, control, and policing against them~\cite{anand2016hindu}. As a result of the amplification of existing societal marginalization of minority communities, as well as the use of social media to incite violence against these communities, social media platforms evoke fear, anxiety, and other negative emotions among minority communities in South Asia~\cite{saha2021short}. Against this backdrop, there is a lack of insights within the field of CSCW and related disciplines regarding the negative experiences of religious minority communities with social media platforms and the support they require. While some aspects of CSCW work in privacy, sensitive disclosure, cyber security, and online harassment have alluded to fear, none are adequate to understand the fearful experiences of religious minorities as informed by our study. Such insights are crucial for understanding and designing strategies to mitigate harms for religious minority communities in the Global South. With this goal in mind, we make the following contributions to the CSCW community:

%\rifat{We can expand if we need to.}

\begin{itemize}
    \item We contribute to the CSCW literature on online safety by providing in-depth insights into the political and socio-psychological aspects of fear among religious minorities in Bangladesh who use social media. Drawing upon the theories of the spiral of silence, politics of emotion, and communication accommodation, we examine the sources and consequences of fear within these communities. Additionally, we discuss the social conditions that either empower or silence these minority communities through the use of the politics of fear. Finally, we explore how these communities address fear by reorienting their social and online connections and adjusting their participation strategies in public spheres.
    \item We contribute to the existing CSCW literature on polarization, restorative justice, and interfaith coexistence on social media by drawing on insights from religious studies, social justice, and interfaith communication. In our discussion, we explore the aftercare and cultural appropriation of restorative justice as means to enhance online safety for religious minority communities in South Asia. By analyzing our findings in relation to the existing literature on harms and violence in South Asia, we uncover the potential of incorporating considerations of history, memory, and postcolonial trauma in the design of solutions for addressing fear in the minority communities.

    %How to make them more specific and concrete. A bit vague now. Actually say those insights are. Spell out what are the sources and consequences
\end{itemize}

We believe our study will advance CSCW's broader vision of social justice and online safety. 


%When the majority religion dominates the political institutions (such as State), the religious minority Others live in an extended state of fearful situation in the South Asian regions~\cite{shani2021towards, lintner2004religious, datta2002post, misra2000hindu}, which is recently being execerbated on social media.



%These instances of social-media incited online harms often align with hyper-nationalist majoritarian political ideologies in South Asian countries~\cite{dash2022insights}. The experiences of religious minority communities are shaped within a cultural construct of the South Asian nations where minority religious groups are often portrayed as ``anti-national'' others~\cite{dash2022insights, islam2007imagining, oommen1986insiders}. As a result of the amplification of existing societal marginalization of minority communities, as well as the use of social media to incite violence against these communities, social media platforms evoke fear, anxiety, and other negative emotions among minority communities in South Asia\rifat{more citation}~\cite{saha2021short}. Against this backdrop, CSCW and related disciplines lack insights into the modes, factors, and consequences of how the fearful experiences of minority communities shape their online and offline experiences in the Global South. Such insights are crucial for our understanding and the design of strategies to mitigate polarization, misinformation, and other online harms in the Global South.



%We present this paper as a step to offer conceptual and design resources within the CSCW community to address online harms for minority communities in South Asia.


%CSCW literature shows a similar trend of sidelining the experiences of religious minority communities demonstrated by a negligible amount of works centering religion to analyze online harms, especially beyond the West when religion plays a dominant role in society. 











%While CSCW and related disciplines have made significant contributions to understanding and mitigating various forms of online harms for racial, linguistic, and other forms of minority communities~\cite{}, the research in this area is still limited by a lack of understanding of the contextual, social-psychological, and political aspects of social media use experienced by the religious minorities in the South Asian regions. Further, the ethical, political, and cultural aspects of faith are seldom considered in CSCW literature of faith-related online harms. We argue that studying the social media use and the unsafe experiences of religious minorities separately from other forms of minority experiences -- such as the considerable amount of HCI studies about racial minorities in the West~\cite{} -- are important for several reasons. Religious minorities represent a different set of aspects of a person's identity primarily based on their their belief and social practices~\cite{fox2000religious}, whereas racial identities build on an individuals' racial and ethnic backgrounds~\cite{}. Because of the differences in identity -- which could also be sometimes intersectional with other forms of minority identities -- the religious minority experiences are strongly shaped by religious influences~\cite{fox2000religious}. The perceived threat posed onto majority groups' worldview by the actions of minority groups, use of religions in political legitimacy, and the influence of religions in ethnic conflicts are consistently found that the harms of ethno-religious minorities are strongly influenced by religion~\cite{fox2000religious}, which could not be accurately characterized by discrimination faced by ethnic minorities, for example. Moreover, unlike the race-based socio-cultural concerns in most of the West, South Asian concerns for social justice often are dominated around faith-based issues. Because of the intertwinedness of religion with the South Asian history and culture~\cite{}, religion has played an influential role not only in state politics in South Asian countries, but also in socio-cultural politics in everyday life~\cite{}. These politics might not be captured from the minority experiences where race, language, or other axis has been the center of attention. Despite such differences, the modern human rights have collapsed all forms of minority rights into the bucket of minority protection rights~\cite{ghanea2012religious}. Further, when religious minorities face discrimination, their case are handled under the category of ``freedom of belief or religion'' instead of minority rights~\cite{ghanea2012religious}. CSCW literature shows a similar trend of sidelining the experiences of religious minority communities demonstrated by a negligible amount of works centering religion to analyze online harms, especially beyond the West when religion plays a dominant role in society. We argue that religious aspects of minority experiences are not merely a reflection of cultural, ethnic, and racial experiences and requires distinct and separate attention to holistically understand the religious minority communities safety and vulnerability on social media. We present this paper as a step to offer conceptual and design resources within the CSCW community to address online harms for minority communities in South Asia.



%The universal equal treatment, which has been celebrated by most democratic states and the peace organization such as the UN, had the underlying assumption that the universal rights for minorities will be panache against all discrimination~\cite{ghanea2012religious}. It took several decades to understand that the equal treatment are discriminatory to those that started lower. For example, if Brahmins and Dalits in India start getting equal treatment, then Dalits are more likely to be discriminated against. 




%These observations show that religious causes of harms and discrimination are not merely a reflection of cultural and ethnic causes of harms~\cite{fox2000religious}, rather demands distinct and separate attention. 


%<religious minorities are categorically different from other minorities> <religious minorities are categorically different in South Asia> <despite being categorically different, religious minority lost its appeal in the minority rights discourse even in insitutions like UN>


%Historically, the protection religious minorities precede the modern human-rights and protection for racial minorities~\cite{ghanea2012religious}. Religious minorities are covered under the general categories of minority rights in human rights protection~\cite{ghanea2012religious}. Although, normatively, religious minorities are designated almost equally alongside ethnic and linguistic minority, religious minority rights are protected only in passing~\cite{ghanea2012religious}. The universal equal treatment, which has been celebrated by most democratic states and the peace organization such as the UN, had the underlying assumption that the universal rights for minorities will be panache against all discrimination~\cite{ghanea2012religious}. It took several decades to understand that the equal treatment are discriminatory to those that started lower. For example, if Brahmins and Dalits in India start getting equal treatment, then Dalits are more likely to be discriminated against. 

%When religious minorities face discrimination, their case are handled under the category of ``freedom of belief or religion'' instead of minority rights~\cite{ghanea2012religious}.


%On top of this, religion as a separate axis of analysis in South Asia is particularly important because of the intertwinedness of religion with the South Asian history and culture. Religion has played the central role in the partition of Indian subcontinent into different states~\cite{}. As a result of this, religion has played an influential role not only in state politics in South Asian countries, but also in socio-cultural politics in everyday life~\cite{}. These politics might not be captured from the minority experiences where race, language, or other axis has been the center of attention.






%We situate our work within the context of Bangladesh, which shares religious-cultural characteristics with the neighboring South Asian countries, particularly regarding the prominent role of religions in society~\cite{}. This geographically, culturally, and historically unique site has drawn separate attention within the CSCW community due to its context largely shaped by colonial histories~\cite{}, limited access to digital technologies~\cite{}, and the influence of religious~\cite{} and spiritual~\cite{} forces. In this context, religious minorities have become victims of misinformation, disinformation, personal attacks, and ridicule~\cite{}. In Bangladesh and other South Asian countries, unlike the North American regions where misinformation is mainly targeted at politics and electoral systems, organized misinformation often targets religious sentiments~\cite{haque2020combating}. Rumors, fabricated images, and targeted memes are often posted from social media profiles impersonating members of minority communities, with the aim of inciting social violence, a common occurrence in South Asian countries~\cite{haque2020combating, kaur2018information, dash2022insights, minar2018violence}. Such harmful online acts frequently lead to organized attacks on places of worship, homes, businesses, and religious festivals~\cite{}. In more extreme cases, social media-incited mob violence results in the killing of individuals from minority communities~\cite{Hasan_Gooding_Dayant_Johnston_2017, roy2023sociological, al2021content}. In several extreme examples, social media has been found to be complicit in incidents of ethnic cleansing~\cite{}. 




%To this end, we conducted an interview-based study involving <n> Bangladeshi religious minority communities, including <Hindu>, to comprehensively understand the social, psychological, and political aspects of using social media platforms. Our findings reveal three dominant patterns: first, the gradual social-psychological influence of fear within the religious minority communities on social media; second, the imposition of fear onto minorities by social or state apparatuses; and third, the continuous adaptation of social media use by the communities based on their anticipation of future fearful consequences. Based on these patterns, our study makes the following contributions to the CSCW community:

%\begin{itemize}
%    \item We contribute significantly to the CSCW literature on online safety by providing in-depth insights into the psychological, political, and cultural dimensions of fear among religious minorities in Bangladesh who use social media. Drawing upon the theories of the spiral of silence, politics of emotion, and communication accommodation, we examine the sources and consequences of fear within these communities. We also highlight how their intersectional minority identities (such as women and LGBTQ individuals) intensify their experiences. Additionally, we discuss the social conditions that either empower or silence these minority communities, as well as their strategies for managing discomfort and fear on social media usage by reorienting their social and online connections and adjusting their participation strategies in public spheres.
%    \item We contribute to the existing CSCW literature on polarization, restorative justice, and online peacebuilding. Drawing on religious studies, indigenous justice, and interfaith communication, we discuss aftercare and cultural appropriation of restorative justice to enhance online safety for religious minority communities in South Asia. By analyzing our findings in relation to the literature on harms and violence in South Asia, we uncover the potential of considering history, memory, and postcolonial trauma in designing solutions for the online safety of these minorities.

    %How to make them more specific and concrete. A bit vague now. Actually say those insights are. Spell out what are the sources and consequences
%\end{itemize}

%We believe our study will advance CSCW's broader vision of social justice and online safety.


%fear is a structural product of history.
%Not as an essential characteristics of religious people
%Misinformation: religious communities is not particularly gullible
%A common way whereby marginalize communities experience fear

%More general 1st para, where does this paper go rather than what are the gaps, what is really interesting in three (what faith based lense offers in this conversation)



%Firstly, drawing upon theories such as the spiral of silence, politics of emotion, and communication accommodation, we provide in-depth insights into the psychological, political, and cultural dimensions of fear experienced by religious minorities in Bangladesh. We examine the sources and consequences of fear within these communities, particularly considering how their other intersectional minority identities exacerbate their experiences. Additionally, we discuss the social conditions that either enable or silence the minority communities, as well as their strategies for accommodating the discomforting aspects of social media use by reorienting their social and online connections, and reorganizing their participation strategies in public spheres. Secondly, building upon our findings and engaging with the existing literature on fear, we contribute to enriching the CSCW literature on online harms by providing policy and design implications for a range of CSCW design resources aimed at mitigating these harms. These implications include the detection of hateful speech, content moderation, and the promotion of contestability. In a broader sense, we discuss how our findings shed light on the barriers faced by minority communities in engaging in public deliberation and democratic participation on social media platforms.


%*****
%Despite the founding promise of social media platforms to foster the coexistence of diverse communities, ensure equality of voices in public deliberation, and provide a safe space for participation, these platforms have instead become unsafe sites for minority communities around the world. In the past decade, as social media platforms gained popularity, the issue of inequality and online harms based on culture and identity related factors including race~\cite{ogbonnaya2020critical, smith2020s}, caste~\cite{vaghela2021birds}, gender~\cite{bardzell2011towards, scheuerman2020we}, and faith~\cite{rifat2020religion} has drawn significant attention in academia and public politics. Academia and the media have reported how social media platforms have introduced and spread new forms of online violence targeted towards religious minority communities in the Global South~\cite{Human_Rights_Watch_2021, Hasan_Macdonald_Ooi_2022}. For example, over the past years, a common pattern of rumor of defaming the holy books in Islam by the minority Hindu individuals spread on social media resulted in mob attacks on Hindu religious establishments and homes in Bangladesh~\cite{Hasan_Macdonald_Ooi_2022, Ethirajan_2021, VICE_2021}. During the COVID-19 pandemic, fake videos claiming that Muslims are deliberately spreading the virus went viral on social media in India~\cite{Human_Rights_Watch_2021, Regan_Sur_Sud_2020, The_Washington_Post_2020}. The fake videos resulted in physical abuses of the Indian Muslims and hampering the business as many people boycott them~\cite{Human_Rights_Watch_2021}. In Bangladesh and other South Asian countries, unlike the North American regions where misinformation is mainly targeted at politics and electoral systems, organized misinformation often targets religious sentiments~\cite{haque2020combating}. Rumors, fabricated images, and targeted memes are often posted from social media profiles impersonating members of minority communities, with the aim of inciting social violence, a common occurrence in South Asian countries~\cite{haque2020combating, kaur2018information, dash2022insights, minar2018violence}. Several social media-incited mob violence resulted in the killing of individuals from minority communities~\cite{Hasan_Gooding_Dayant_Johnston_2017, roy2023sociological, al2021content}. In several extreme examples, social media has been found to be complicit in incidents of ethnic cleansing~\cite{Amnesty_International_2023, The_Guardian_2021}. This forms of online harms and violence amplified through social media have been alarmingly increasing and making the lives of religious minority communities unsafe around the world.

%While CSCW and related disciplines have made significant contributions to understanding and mitigating various forms of online harms for racial, linguistic, and other forms of minority communities, many of which are primarily based in the West~\cite{}, the research in this area is still limited by a lack of understanding of the contextual, social-psychological, and political aspects of social media use experienced by the religious minorities in the South Asian regions. We argue that studying the social media use and the unsafe experiences of religious minorities in South Asian countries separately from other forms of minority experiences -- such as the well-documented CSCW literature concerning racial minorities in the West~\cite{} -- is important for two primary reasons. First, religious minorities represent a different set of aspects of a person's identity primarily based on their their belief and social practices~\cite{fox2000religious}, whereas racial identities build on an individuals' racial and ethnic backgrounds~\cite{}. Because of the differences in identity, the religious minority experiences are strongly shaped by religious influences~\cite{fox2000religious}. The perceived threat posed onto majority groups' worldview by the actions of minority groups, the use of religions in political legitimacy, and the influence of religions in ethnic conflicts are a few of the strong reasons why ethno-religious minorities are strongly influenced by religion~\cite{fox2000religious}, which could not be accurately characterized by discrimination faced by ethnic minorities, for example. Second, unlike the race-based social justice concerns in most of the West, South Asian concerns for social justice often are dominated around faith-based issues~\cite{}. Because of the intertwinedness of religion with the South Asian history and culture~\cite{}, religion has played an influential role not only in state politics in South Asian countries, but also in socio-cultural politics in everyday life~\cite{}. These politics might not be captured from the minority experiences where race, language, or other axis has been the center of attention. Despite such differences, the modern human rights have collapsed all forms of minority rights into the bucket of minority protection rights~\cite{ghanea2012religious}. Further, when religious minorities face discrimination, their case are handled under the category of ``freedom of belief or religion'' instead of minority rights~\cite{ghanea2012religious}. We observe a similar trend in CSCW literature, when religion is collapsed into other cultural and minority categories, which is evident in a sizable CSCW literature where religion is put into a periphery of analyzing online harms (see, for example~\cite{shahid2023decolonizing, mustafa2020patriarchy}). We argue that religious aspects of minority experiences are not merely a reflection of cultural, ethnic, and racial experiences and requires distinct and separate attention to holistically understand the religious minority communities safety and vulnerability on social media.

%To this end, we conducted an interview-based study involving three Bangladeshi religious minority communities to comprehensively understand their experience of using social media platforms. Informed from our findings, we put fear into the center of analysing the religious minority experiences of social media use in Bangladesh. Our findings reveal three dominant patterns: first, the gradual social-psychological influence of fear within the religious minority communities on social media; second, the imposition of fear onto minorities by social or state apparatuses; and third, the continuous adaptation of social media use by the communities based on their anticipation of future fearful consequences. Our attention to fear is also informed from a long history of the politics of fear concerning the religious minority communities in South Asia. A strong religious influence on the nationalist politics in the Indian subcontinent has used the politics of fear in justifying anti-minority violence in the region~\cite{anand2016hindu}. The social-media incited online harms often align with hyper-nationalist majoritarian political ideologies in South Asian countries~\cite{dash2022insights}. For example, the the Hindu national politics in India, Hindutva, feels the insecurity that the religious minority Others are a threat to their identity, and thus create a stereotype image of the minority Others as a danger to them~\cite{anand2016hindu, shani2021towards}. In doing so, the majority religious groups portray minority religious groups as ``anti-national'' Others~\cite{dash2022insights, islam2007imagining, oommen1986insiders}. Similar strong intertwindness of religions and politics continue to create the politics of fear in other parts of South Asia, too~\cite{mohsin1984religion, riaz2016bangladesh, fair2012faith}. Such a politics of fear socially construct hate against the religious minority Others in South Asia and justify social surveillance, control, and policing against them~\cite{anand2016hindu}. As a result of the amplification of existing societal marginalization of the minority communities, as well as the use of social media to incite violence against these communities, social media platforms evoke fear, anxiety, and other negative emotions among minority communities in South Asia\rifat{more citation}~\cite{saha2021short}. Against this backdrop, CSCW and related disciplines lack insights into how the fearful experiences of minority communities shape their online and offline experiences in the Global South. While a body of CSCW of work in privacy, sensitive disclosure, cyber security, and online harassment has alluded to fear, none are adequate to understand the religious minorities' fearful experiences informed from our study. Such insights are crucial for our understanding and the design of strategies to mitigate polarization, misinformation, and other online harms for the religious minority communities in the Global South. With this goal, we make the following contributions to the CSCW community:

==> sections/litreview-rewrite.tex <==
\section{Literature Review}
We draw from three lines of scholarship to inform and frame our work: firstly, we explore the social and political psychological aspects of fear relating to group coexistence, ethnic conflicts, and peacebuilding. We then extend our discussion to two related lines of CSCW literature and demonstrate how the literature might benefit from addressing fear in the use of social media by religious minority communities. These two areas include the fear-based marginalization of religious minorities in public spheres, particularly social media, and addressing fear in supporting religious minority communities, with a specific focus on restorative justice.



%We draw from three lines of scholarship to inform and frame our work: we open the discussion by drawing from the social and political psychological aspects of fear in the context of group coexistence, ethnic conflicts, and peacebuilding. We then extend our discussion to two related lines of CSCW literature and demonstrate how the literature might benefit from addressing fear in religious minority communities' use of social media and mitigating harms: first, fear-based marginalization of religious minorities in public spheres in general and social media in particular, and second, addressing fear in supporting religious minority communities, particularly focusing on restorative justice.



\subsection{Fear and Group Coexistence: Social and Political Psychological Aspects of Fear}
\label{fearandgroup}

We build upon a substantial body of literature on fear, focusing on the social, political, and psychological aspects of fear. The literature defines fear as an apprehension of harm to the well-being of a group~\cite{robin2004fear, furedi2006culture, jarymowicz2006dominance}. These apprehensions can range from panic due to crimes to everyday acts of intimidation between different groups~\cite{robin2004fear}. Various tensions within the civic sphere can invoke fear, leading to repercussions on various societal groups and institutions~\cite[ch~.1]{robin2004fear}. To demonstrate the significance of fear, theologian and philosopher S{\o}ren Kierkegaard, for example, explained the role of fear in creating as well as dealing with political crises and uncertainties in everyday life~\cite{kierkegaard2013fear}. As a result, fear sometimes emerges as a spontaneous response to civic crises at the group level, serving as an adaptive mechanism for individuals and groups to cope with adversity~\cite{jarymowicz2006dominance}. This body of literature warns that fear acts as an enemy of freedom and liberty, perpetuating conflicts at the group level by hindering the use of political tools to mitigate them.




%We build upon a substantial body of literature on fear, focusing on the social and political psychological aspects of fear. The literature defines fear as an apprehension of harms to the well being of a group~\cite{robin2004fear, furedi2006culture, jarymowicz2006dominance}. Such kinds of apprehension may range from the panic from crimes to everyday intimidation by one group to the others~\cite{robin2004fear}. Various tensions within the civic sphere invoke fear with repercussions on various societal groups and institutions~\cite[ch~.1]{robin2004fear}. To demonstrate the significance of fear, theologian and philosopher, Kierkegaard, for example, explained the role of fear in creating as well as dealing with political crises and uncertainties in everyday life~\cite{kierkegaard2013fear}. Because of this, fear is sometimes a spontaneous response to civic crises in the group level, as fear serves as an adaptive mechanism for individuals and groups to cope with adversity~\cite{jarymowicz2006dominance}. This body of literature about political and social psychological aspects of fear warns that fear is an enemy of freedom and liberty, that perpetuates group-level conflicts by blindsiding the political tools to mitigate the conflicts.

%A significant body of literature has built on such political aspects of fear to provide insights into the instrumental role of fear in group-level conflicts. 


Due to these social and political psychological capacities -- alongside intergroup differences and ``ancient hatred'' -- fear has been proven to be detrimental to inter-group coexistence~\cite{lake1996containing, lake1998international, melander2009geography, thiong2018politics}. Fear among groups overrides hopes, fosters insecurity, generates mistrust, and hampers peaceful conflict resolution, as groups rely on past assumptions and threats~\cite{jarymowicz2006dominance, neocosmos2008politics}. Minority communities experience fear not only due to rational concerns such as safety and identity but also as a result of political myths and various other emotions, with fear being a primary emotion~\cite{lake1996containing}. These detrimental impact of fear on group coexistence and peacebuilding is evident in celebrated South Asian scholar Veena Das's analysis of the conflict between Hindu and Sikh communities, where fear stemming from violent memories and traumatic events hindered peaceful negotiation and conflict resolution between the two religious groups~\cite{das1998specificities}. Understanding these group dynamics shaped by fear is crucial for making political decisions and fostering peace at both micro and macro societal levels. For instance, group coexistence necessitates compromise and support among the group members~\cite{worchel2008between, abu2001reconciliation}. While fear can sometimes inspire greater compromise, in other cases, it diminishes willingness to compromise as a group member~\cite{gayer2009overcoming, halperin2011emotional}. Besides, in peace negotiations between ethnic and religious groups, mutual risk-taking and concrete actions are vital. Fear acts as an obstacle in intergroup peace negotiations and hampers the adoption of concrete measures~\cite{halperin2011emotional}. Fear's influential impact often exacerbates conflicts by reinforcing belief in conspiracy theories~\cite{hebel2022vicious}. Overall, the aforementioned studies emphasize the importance of recognizing fear in intergroup relations and addressing its origins through psychological and political means to mitigate its effects. To acknowledge the prominence of fear in the coexistence of minority and majority religious groups, a factor that is currently not adequately recognized in CSCW, we build upon the existing political and socio-psychological literature on fear to make two primary contributions to CSCW: first, we explicate fear-based marginalization of religious minority voices on social media, and second, we discuss how fear may advance restorative justice for religious minority voices.



\subsection{Fear-based Marginalization of Minority Voices in Public Spheres}
To examine the impact of fear on social media, we begin by tracing the concept of the public sphere, its foundational principles of freedom of expression and participation, and the challenges it faces in ensuring equal participation due to fear. Subsequently, we delve into the literature of CSCW focused on public deliberation, illustrating how fear can contribute to critical discourses and the design of socio-technical systems aimed at addressing fear within religious minority communities in South Asia.

\subsubsection{Fear's Influence on Public Spheres}
One influential work that has shaped the discourse on free speech, equal public participation, and deliberation is Jürgen Habermas's concept of the public sphere. According to Habermas, the public sphere refers to a social space where public opinion is formed through rational-critical debates and discussions among free and equal citizens~\cite{habermas1996public}. Habermas and his colleagues extend, ``citizens behave as a public body when they confer in an unrestricted fashion -- that is, with the guarantee of freedom of assembly and association and the freedom to express and publish their opinions-about matters of general interest~\cite{habermas1974public}.'' Based on these arguments, Habermas and subsequent literature envision a public sphere that emphasizes equality and inclusivity, enabling individuals to express their opinions regardless of their social status and power. As social media gained popularity, scholars started exploring whether these platforms could provide a space akin to the public sphere, potentially enhancing freedom and equality~\cite{kruse2018social, shirky2011political, bruns2015habermas}. With features such as free and unlimited access to information, unrestrained participation, and the ability to facilitate collective action, social media platforms align closely with the core characteristics of the Habermasian public sphere~\cite{shirky2011political}. Consequently, social media platforms function as digitally-mediated public spheres that operate alongside the physical world public sphere~\cite{ccela2015social}. Overall, there was hope among entrepreneurs and academics that social media platforms would promote equality and inclusivity by amplifying diverse voices.

Critics have challenged the assumptions of the public sphere and expressed skepticism regarding social media platforms' ability to facilitate equal political participation and public deliberation~\cite{kruse2018social, polan1990public, kellner2000habermas, dahlberg2005habermasian, susen2011critical}. Two main lines of criticism argue that power is separated from the public sphere by masking exclusion and domination, and minority voices are suppressed when they differ from the majority~\cite{dahlberg2005habermasian}. Subsequent literature reveals how fear suppresses minority voices in social media platforms, influenced by social and political surveillance, media-driven misperceptions, and the fear of isolation and ridicule~\cite{hampton2014social}. For instance, minority communities, like Muslims and Black communities, often self-censor their online expression due to increased scrutiny by law enforcement agencies, even in Western democratic nations where individuals enjoy more freedom and agency~\cite{aziz2020fear}. This continuous surveillance leads to self-monitoring of opinions to align with normative frameworks set by majority voices~\cite{aziz2020fear}. Disproportionate negative news coverage of minority communities by the news and social media platforms further perpetuates false perceptions, fostering feelings of alienation, hostility, and distrust, inhibiting active participation on social media~\cite{hildreth2015fear, fox2015queer}. Empirical studies by Pew Research confirm these findings by presenting their insights that individuals perceiving themselves as holding minority identities refrain from freely expressing opinions due to fear of ostracism and ridicule~\cite{hampton2014social}. These findings highlight how fear marginalizes minority voices on social media. Next, we discuss relevant CSCW studies on public deliberation and polarization on social media, emphasizing the significance of recognizing fear to address the marginalization of religious minority voices in South Asian regions.

%However, a powerful thread of criticisms challenged the founding assumptions of the public sphere and showed their skepticism of social media platforms' capabilities of equal political participation and public deliberation~\cite{kruse2018social, polan1990public, kellner2000habermas, dahlberg2005habermasian, susen2011critical}. Two dominant threads in these criticism argue that power has been separated from the public sphere by masking of exclusion and domination and minority voices have been suppressed in the cases where minorities might not agree with the majority voices~\cite{dahlberg2005habermasian}. A dominant line of subsequent literature demonstrates how fear plays an instrumental role in suppressing minority voices from social media and other public spheres due to social and political surveillance, false perceptions created by the media, and the fear of isolation and ridicule. One prominent example is the use of fear tactics to instill panic in minority communities, particularly through policing minority online activism~\cite{aziz2020fear}. Even in Western democratic nations, where individuals have more freedom and agency, minority communities, such as Muslims and Black communities, often self-censor their online expression due to the fear of increased scrutiny by law enforcement agencies~\cite{aziz2020fear}. The constant surveillance by these agencies leads minority communities to continuously monitor themselves, ensuring that their opinions align with the normative and legal frameworks, which are often set by majority voices~\cite{aziz2020fear}. News and social media also contribute to the creation of false perceptions about minority communities by disproportionately highlighting negative news about them, thereby subjecting them to extended surveillance and scrutiny. Consequently, these communities become fearful to actively participate on social media platforms due to their feelings of alienation, hostility, and distrust~\cite{hildreth2015fear, fox2015queer}. An empirical study conducted by Pew Research has also confirm that individuals who perceive themselves as holding minority voices often refrain from freely expressing their opinions due to fear of ostracism and ridicule~\cite{hampton2014social}. These findings collectively demonstrate how fear marginalizes minority voices from social media. Building upon these findings, we discuss CSCW studies about public deliberation and polarization on social media and extend that to show how acknowledging fear can enrich CSCW literature to account for the marginalization of religious minority voices in South Asian regions.

%In line with this, Fox and Warber explored how the fear of unintended identity exposure or social backlash limits the use of social media platforms by minority queer communities~\cite{fox2015queer}. Additionally, Leyn et al. studied ethno-religious minorities and revealed their perception of the social media "public sphere" as dominated by culturally and normatively defined majorities, leading to feelings of alienation, hostility, and distrust~\cite{de2022networked}. Consequently, they primarily connect with their networked peers to avoid conflict and potential backlash.

 %are the masking of exclusion and domination by assuming that power could be separated from the public sphere and promoting consensus by suppressing minority voices who might not agree with the majority voices~\cite{dahlberg2005habermasian}. Fear relates to these threads of criticism where it creates power differential between majority and minority groups. The works have documented the fear experienced by minority communities in their social media engagement.


\subsubsection{Public Deliberation and Marginalization of Minority Voices in CSCW}
%Following our discussion on the social and political psychological influence of fear in public spheres, we now shift our focus to a specific CSCW literature that centers on public opinion, online polarization, and design and policy solutions to tackle these issues. Subsequently, we address the absence of fear as a missing thread within this literature, particularly concerning religious minorities in the Global South.


CSCW has a substantial body of literature that provides insights into online polarization on social media platforms and discusses solutions for mitigating it. Nelimarkka et al. emphasize that, contrary to social media's goal of deliberative and democratic discussion, individuals tend to engage with like-minded people, resulting in political polarization~\cite{nelimarkka2018social}. They suggest that prompting users with different viewpoints before posting online could help mitigate polarization. Kim et al. present the design and evaluation study of StarryThoughts, a socio-technical system for expressing and exploring diverse opinions on social issues online~\cite{kim2021starrythoughts}. Their evaluation study reveals that the demographic information of a post's author helps contextualize the content, fosters empathy, and promotes openness to conflicting opinions. Wang et al. utilize the Moral Foundation Theory to categorically present posts and comments to readers of news articles, aiming to bridge ideological divides~\cite{wang2022designing}. The authors find that this system highlights both the commonalities and differences in the moral framing of news articles, enabling users to become conscious of and learn about moral distinctions. Bail et al. discover that intergroup communication promotes more effective deliberation by encouraging compromise and mutual understanding in intergroup ideologies and politics~\cite{bail2018exposure}. In summary, the aforementioned and other works~\cite{semaan2014social, terren2021echo, baughan2021someone, das2021jol} within CSCW explore design and policy suggestions, ranging from exposing users to diverse political perspectives to utilizing compromise and mutual understanding as design resources. These insights are based on assumptions about the contexts and support infrastructures in public deliberation, including democratic voices irrespective of faith-based identities, an increasingly unrestricted culture of freedom of expression and identity, moral and legal support in unsafe situations, and an emphasis on modern and rational value systems.

Contrary to these insights and their underlying assumptions, a line of scholarly studies about South Asian religious minorities shows how the already existing divides between religious majorities and minorities are magnified on social media, resulting in fear and anxiety within the religious minority communities~\cite{bahfen2018individual, bhatia2020examining, bhatia2019times}. As the societal divides among religious groups in South Asia are stronger, people often use online platforms seeking solidarity and like-minded individuals~\cite{bhatia2019times}. However, as people start performing their religious identities on social media and sharing their negative and unpleasant experiences on the platforms, the already existing social divides along religious lines are further amplified, causing religious minority communities to lose their voices on the platforms~\cite{bhatia2019times}. Intersectional identities -- encompassing multiple social identities that intersect and interact with each other, shaping people's experiences and societal positions~\cite{cho2013toward} -- often reinforce the marginalization of the minority population in South Asian societies~\cite{bhatia2020examining}. For example, Muslim women, who constitute the minority community in a hypermasculine, dominant religious groups, and patriarchal society, often face additional barriers to appear in public spaces~\cite{bhatia2020examining}. Religious marginalization happens even within the same religious groups. For example, Muslims who express borderline perceptions about their religious values often face opposition from members of their own Muslim community~\cite{bahfen2018individual}. These studies suggest that CSCW needs to recognize and address the marginalization based on religious identities in order to empower religious minority voices in online and societal public spheres.

Combining the two threads of literature above—the CSCW literature on public deliberation and polarization, and the South Asian studies on the marginalization of religious minorities—we conclude that fear is a crucial missing piece in studying the social media participation of religious minorities, particularly in the Global South where socio-political factors are closely intertwined with religious influences. We aim to address this gap in our study.

%As opposed to these insights and their underlying assumptions, a line of scholarships about South Asian religious minorities show how already existing divides between religious majorities and minorities are magnified on social media resulting in fear and anxiety of the religious minority communities~\cite{bahfen2018individual, bhatia2020examining, bhatia2019times}. As the divides among religious groups in South Asian are stronger, people often use social media seeking for solidarity and like-minded people~\cite{bhatia2019times}. However, as people start performing their religious identities on social media and sharing their negative and unpleasant experiences on the platforms~\cite{bhatia2019times}. As a grand effect, the already existing social divides along the line of religions amplify and religious minority communities loose their voices on the platform~\cite{bhatia2019times}. Intersectional identities -- multiple social identities that intersect and interact with each other, shaping people experiences and societal positions~\cite{cho2013toward} -- often reinforce the marginality of the minority population in South Asian societies~\cite{bhatia2020examining}. For example, Muslim women, who constitute the minority community in a hypermasculine, characterized by dominant religious groups, and patriarchal society, often face additional barriers to appear in public spaces~\cite{bhatia2020examining}. Religious marginalization happen even within the same religious groups. For example, study shows that Muslims who post borderline perception about their religious values, often counter members of their own Muslim community~\cite{bahfen2018individual}. These studies suggest that CSCW needs to recognize and address marginalization based on religious identities for empowering religious minority voices in online and societal public spheres.

\subsection{Design Justice for Minority Communities: The Case of Restorative Justice}
The political and social psychological aspects of fear, as discussed in section \ref{fearandgroup}, together with our findings, indicate the influential role of fear in shaping the pursuit of justice and the sustainability of justice practices for minority communities. Recognizing this pivotal role, our contribution aligns with a separate strand of literature in CSCW that utilizes restorative justice to support victims from minority communities. To contextualize our contribution within this literature, we initially explore the negative experiences encountered by minority communities, followed by an examination of coping mechanisms and available support mechanisms for addressing these negative experiences. Finally, we focus on the CSCW literature concerning restorative justice and discuss the necessity of addressing the fear experienced by religious minority communities in South Asia.


\subsubsection{Negative Experiences of Minority Communities on Social Media}
CSCW has extensively documented the various forms of negative experiences and challenges that minority communities face online. The ``default publicness,''  an inherent design orientation that prioritizes state-validated identities and favor majoritarian views~\cite{cho2018default}, creates disparities between the platform values and the values of the minority communities~\cite{devito2021values}. Because of such disparities, as CSCW literature has examined, members of LGBTQ+ communities face incidents of unexpected exposure of their posts to unintended audiences~\cite{cho2018default}, abuse~\cite{scheuerman2018safe}, and stigma~\cite{scheuerman2018safe}. CSCW research has similarly documented emotional and physical discomfort, embarrassment, lack of belongingness, harassment, and demonization, among other harms and unsafe experiences among racial minority groups~\cite{ogbonnaya2020critical, smith2020s, cunningham2023grounds, adamu2023no, salehi2023sustained}. The intersectionality of multiple minority identities further exacerbates the harm experienced by these communities. For example, CSCW has documented how the dual minority identities of transgender women~\cite{scheuerman2018safe}, trans individuals with eating disorders~\cite{feuston2022you}, LGBTQ young individuals~\cite{10.1145/3173574.3173683}, and gender or sexual minorities experienced pregnancy loss~\cite{andalibi2022lgbtq}, among other intersectional identities experienced intensified abuse and marginalization. Collectively, the studies on minority communities confirm that individuals with minority identities along axes of race, gender, sexuality, and more encounter a range of compounding harmful experiences, including harassment, marginalization, bias, and violence. However, the CSCW literature currently lacks comprehensive insights (with a few exceptions) into the experiences of religious minority communities in the Global South.











%These studies reveal that minority communities have to take an extra burden to strategically utilize social media ecosystems in mitigating harassment and maintaining a sense of safety.

%Scholars in this field have shed light on the challenges minority communities encounter when expressing their identity on social media platforms. One notable study by Cho explores the experiences of US queer youth of color on social media, specifically within the queer Tumblr community~\cite{cho2018default}. The research highlights the concept of ``default publicness,'' an inherent design orientation that prioritizes state-validated identities, often favoring majoritarian views~\cite{cho2018default}. As a result, minority queer youth of color often lose control over their social media activity and face severe negative consequences as their posts are unexpectedly shared with unintended audiences~\cite{cho2018default}. Building on these findings, Devito et al. investigate the misalignment between platform values and the values held by minority LGBTQ+ communities, revealing the negative experiences and harms that arise from this disconnect~\cite{devito2021values}. The CSCW community has further expanded on the struggles faced by minority communities on social media platforms. For instance, Scheuerman et al. conduct interviews to examine the risks and harms experienced by transgender individuals in the US~\cite{scheuerman2018safe}. Their research uncovers how the same platforms that offer opportunities for connection and safe spaces can also be harmful and abusive towards transgender individuals~\cite{scheuerman2018safe}. Anti-trans social media users are shown to target and harass transgender populations, making their online experiences stigmatizing~\cite{scheuerman2018safe}. In similar vein, DeVito et al. employ cognitive mapping exercises and interviews to illustrate how LGBTQ+ communities navigate stigma while performing their identities and seeking social support on social media platforms~\cite{devito2018too}. These studies reveal that minority communities have to take an extra burden to strategically utilize social media ecosystems in mitigating harassment and maintaining a sense of safety. CSCW research has similarly documented harms and unsafe experiences among racial minority groups~\cite{ogbonnaya2020critical, smith2020s, cunningham2023grounds, adamu2023no}. To et al. utilize narrative episode interviews and semi-structured interviews to explore support-seeking practices among racially marginalized populations~\cite{to2020they}. Their findings illustrate the emotional and physical discomfort, embarrassment, and lack of belongingness experienced by individuals due to direct and indirect racially discriminating activities~\cite{to2020they}. Additionally, CSCW literature highlights how minority communities often form counterpublics in response to harms; however, their activism is met with further harassment and harm. For instance, Salehi et al. investigate how visible Muslim American public figures utilize social media platforms to challenge dominant narratives demonizing Muslims and construct counter narratives~\cite{salehi2023sustained}. The demonstrate, the same platform affordances designed to empower users are weaponized against minority social media users, resulting in sustained harassment and abuse of these communities~\cite{salehi2023sustained}. These studies, alongside others in the CSCW and HCI~\cite{buss2022transgender, southerton2021restricted, pym2021still, paceley2022sometimes, simpson2021you}, provide a broad and nuanced understanding of the marginalization, harassment, bias, and other negative experiences encountered by minority communities on social media and other online spaces.


%In addition to the existing inequalities faced by minority communities, the intersectionality of multiple minority identities further exacerbates the harms experienced by these communities. Scheuerman et al., for instance, shed light on the intensified abuse and marginalization faced by minority transgender populations, who are also women of color or sex workers~\cite{scheuerman2018safe}. Further exploring the intersectionality of identities, Feuston et al. examine trans individuals with eating disorders and find that the trans minority community within the eating disorder community is more vulnerable to online harm due to the continuous need to validate their identity~\cite{feuston2022you}. The authors argue that dominant norms and standards around eating disorders, often perpetuated by cisgender individuals, create challenges for trans communities who challenge these norms~\cite{feuston2022you}. Similarly, Andalibi et al. focus on LGBTQ individuals and other gender or sexual minorities who have experienced pregnancy loss or have partners who have experienced it~\cite{andalibi2022lgbtq}. Through an intersectional analysis of online experiences during pregnancy loss, the authors demonstrate how the combination of LGBTQ identity and pregnancy loss intensifies discrimination and exclusion on social media platforms~\cite{andalibi2022lgbtq}. Haimson et al. examine non-normative users of social networking sites (SNS) who undergo identity changes and find that the politics of categorization, such as gender, on SNS interfaces can contribute to stress for minority communities within socio-technical systems~\cite{haimson2015disclosure}. Collectively, studies on intersectional minority communities confirm that individuals with intersecting minority identities along axes of race, gender, sexuality, and more, encounter a range of compounding harmful experiences, including harassment, marginalization, bias, and violence. However, the CSCW literature currently lacks comprehensive insights (with a few exceptions) into the experiences of religious minority communities on social media.

\subsubsection{Coping Up with Negative Experiences and Seeking Justice}

To cope with the negative experiences and navigate other online safety-related issues, minority communities often find social media platform policies misaligned and sometimes hostile towards them. For example, minority communities are often forced to conform to universal platform policies, leading to further marginalization~\cite{shahid2023decolonizing, feuston2020conformity}. Due to the social media platforms' universal content moderation policies, minority communities lose personal content more frequently than majority groups, even when the content follows community guidelines~\cite{feuston2020conformity, haimson2021disproportionate}. The platforms lack resources to filter out content that is made for ridiculing and bullying minority communities~\cite{medina2020dancing}, and individuals in the community bear an extra burden in seeking support in these situations~\cite{feuston2020conformity}. Furthermore, the social media platforms lack policies to be inclusive of minority communities by increasing their participation~\cite{saha2019language}. Moreover, moderation policies and support for minority communities are weaker in the Global South, as moderation policies often overlook the context and culture of the population in the Global South~\cite{shahid2023decolonizing}. These findings suggest that social media policies are barely adapted to non-dominant identities, norms, and ways of being. To address these limitations and better support minority communities, CSCW is increasingly drawing on various justice frameworks to integrate them into CSCW design~\cite{xiao2023addressing, erete2021applying}. In this paper, we specifically draw on the framework of restorative justice~\cite{xiao2023addressing} due to its capability to support religious minority communities in addressing fear.




%Drawing on a two years long digital ethnography, Feuston et al. shows how an already marginalized group, people with eating disorders, are pressured to conform to the dominant groups in the content moderation policies~\cite{feuston2020conformity}. The authors show how the eating disorder community loses personal contents and community support due to a moderation that is more aligned with the dominant online user groups. This, in turn, loads the community with an added task of restoring their lost contents. In a similar vein, Haimson et al. study the frequency of content removals for the political conservatives, transgender, and black people through moderation is higher than other communities~\cite{haimson2021disproportionate}. The authors further show that trasnpeoples’ contents are often removed with the allegation of being adult, insulting for the dominant groups, and violent, even though these contents follow the community guidelines. Shahid and Vashistha find how content moderation policies are often oblivious of the context and culture of the global south population~\cite{shahid2023decolonizing}. The risks and vulnerability of the minority communities can also be exacerbated by the increasing move from text-based interactive platforms to video-based interactive platforms. For example, while platforms such as Facebook and Twitter are mostly friends and/or follower based that can emphasize in-group interaction, the video sharing platform such as TikTok cross-partisan dialogues, with the contents being created with aggressive goals to be viral~\cite{medina2020dancing}. The contents are created with humor and sarcasm with the goal of making them viral and run into the risk of ridiculing and bullying minority communities in the form of entertainment, which may not be filtered in the existing moderation technologies. Supporting minority communities through computational tools is also challenging for a number of reasons. The challenges primarily stem from the communities’ willingness to participate in designing and using computational tools that may make them vulnerable to increased exposure and scrutiny for the broader community. Saha et al., for example, note complexities of quantifying the data of the minority communities, that might limit the participation of the community in anticipation that their data are being quantified and silence their participation altogether~\cite{saha2019language}. Cui et al. conduct an interview-based study with the sexual minority women in China in using dating apps and find that the SMWs use the dating app for careful identity disclosure and development~\cite{cui2022so}. The authors discussed how SMW communities are often afraid of unexpected disclosure of their identity, which, in turn, might threaten their online safety by non-LGBTQ communities. These findings suggest that social media policies are barely adaptive to non-dominant identities, norms, and their ways of being.


\subsubsection{Restorative Justice for Minority Communities}

A nascent body of literature is focusing on restorative justice to mitigate harm for minority communities~\cite{xiao2023addressing, xiao2022sensemaking, chatlani2023teen, rabaan2023survivor, sultana2018design}. Social media companies often address online harm following a justice model primarily centered on ``isolation and punishment''\cite{myers2018censored, vaccaro2020end}. While social media platforms offer users the ability to customize, report, delete, and block content as well as contest moderation decisions, these features effectively place the burden on users, especially those with minority identities, while the platforms hold the power in their hands. In contrast, proponents of restorative justice within CSCW argue for turning the attention from platforms to the vulnerable and affected communities and supporting them\cite{salehi2023sustained, xiao2023addressing}. Restorative justice prioritizes the victims of online harms by restoring communal bonds and relationships~\cite{xiao2023addressing}. Alongside modern values of freedom, equality, accountability, and deliberation, concepts like healing, apology, social harmony, and other human virtues are receiving attention in addressing online harms through restorative justice~\cite{xiao2023addressing}. While these directions offer hope for supporting the victims, as we will argue below, the literature needs to contextualize restorative justice to account for the social-psychological and political aspects of fear in South Asia.

Religious sensitivities, which are more prevalent in South Asian everyday life and national politics, reinforce discrimination and fear against religious minority communities~\cite{bhatia2021religious, bhatia2022hindu, mohan2015locating}. Far-right religious nationalists in South Asia employ social media to perpetuate social fear, discrimination, and stereotypes against minority castes and religions~\cite{vaghela2021birds, bhatia2021religious, mohan2015locating}. Even people who are friendly in society, exhibit hostile and discriminatory behavior online through trolling, cyber-bullying, and other means towards religious minority communities~\cite{bhatia2021religious}. The politics of fear is often supported and normalized by political parties that benefit from such narratives~\cite{bhatia2022hindu}. Overall, religious minority groups are depicted as both perpetrators and victims of online violence~\cite{kirmani2008competing, bhatia2022revolution}. In this context, we emphasize that fear adds an extra layer of challenge in supporting victims through restorative justice. To address this gap, we draw from our findings to provide design and policy implications to address fear and better support religious minority communities in the Global South.







%existing CSCW insights about minority communities are inadequate for understanding the experiences of religious minority communities. To address this gap, our research aims to comprehensively explore the experiences of religious minority communities particularly emphasizing fear-related aspect of their experience using theoretical lenses drawn from anthropology and cultural studies. 



%Social media companies often address online harm following a justice model primarily centered on ``isolation and punishment’’~\cite{myers2018censored, vaccaro2020end}. While social media platforms offer users the ability to customize posts, report, delete, block content, and contest moderation decisions, these features effectively place the burden on users while holding the power in their hands. These affordances support the platform's governance, moderation, and regulation within the framework of isolation and punishment. Consequently, ethical and political aspects of societies, local modes of justice, and the essence of life of users are disregarded as social media platforms’ policies to tackle online harms are often isolated from local histories, communal practices, and culture~\cite{shahid2023decolonizing}. In contrast, CSCW advocates for prioritizing the victims of online harms and restoring communal bonds and relationships~\cite{xiao2023addressing}. Alongside modern values of freedom, equality, accountability, and deliberation, concepts like healing, apology, social harmony, and other human virtues~\cite{xiao2023addressing} are receiving attention in addressing online harms through restorative justice. While these directions offer hope for supporting the victims, we argue that the literature needs an extension to contextualize restorative justice—as we have discussed in this paper—to better account for the social-psychological and political aspects of fear in South Asia. These aspects in South Asia are often laden with colonial trauma and religious sensitivity, particularly for religious minority communities.

%The primary reason why we argue for an extension of the literature about religious minority communities, along with the justice frameworks to support them in South Asia, stems from the differences among minority communities in terms of their identities, values, ethics, and contexts. In this paper, we specifically emphasize how faith based politics shape the social media use experiences of religious minority groups, which often serve as an extension, albeit an amplified one, of their social lives. Our analysis centers around fear as a key aspect of the minority experience on social media. This emphasis on fear is informed by a robust body of literature demonstrating how ``religious nationalism,'' which is more prevalent in South Asian regions compared to the Global North and reinforces discrimination and fear against religious minority communities~\cite{bhatia2021religious, bhatia2022hindu, mohan2015locating}. As opposed to modern and secular presumption that social networking sites (SNS) inspire depoliticized and rational societies, SNS platforms in South Asia contribute to the constitution of religious subjects online and amplify existing social segregation along religious identity lines~\cite{bhatia2021religious}. Contrary to the utopian notion of ``self-abstraction'' in public spheres, including social media platforms~\cite{cody2015populist}, far-right religious nationalists in South Asia employ social media to perpetuate social fear, discrimination, and stereotypes against minority castes and religions~\cite{vaghela2021birds, bhatia2021religious, mohan2015locating}. Some individuals may adopt different personas online compared to offline interactions. For instance, they may refrain from engaging in harmful activities offline, but as part of ``digital collectives,'' the same individuals exhibit discriminatory behavior towards religious others through trolling, cyber-bullying, and other online means in South Asian online sphere~\cite{bhatia2021religious}. The politics of fear are often supported and normalized by political parties that benefit from such narratives~\cite{bhatia2022hindu}. The far-right majoritarian religio-political forces enforce various normative systems of ``online'' punishment, including mob violence against religious minorities, further intensifying the fear of engagement with social media and discursive activities among minority communities in South Asia~\cite{bhatia2022hindu}. Altogether, religious minority groups are depicted as both perpetrators and victims of online violence~\cite{kirmani2008competing, bhatia2022revolution}. This is in this context we emphasize that the existing CSCW insights about minority communities are inadequate for understanding the experiences of religious minority communities. To address this gap, our research aims to comprehensively explore the experiences of religious minority communities particularly emphasizing fear-related aspect of their experience using theoretical lenses drawn from anthropology and cultural studies. 

%In our study, we build upon these findings and provide an in-depth analysis of the social and political psychological insights into the fear experienced by religious minority communities on social media platforms in Bangladesh, along with their implication to CSCW.








%Such social and political psychological characteristics of fear has been a significant factor contributing to conflicts between majority and minority groups, alongside intergroup differences and ``ancient hatred''~\cite{lake1996containing, lake1998international, melander2009geography, thiong2018politics}.


%Minority communities experience fear not only due to rational concerns such as safety and identity, but also as a result of political myths and various other emotions, with fear being a primary emotion~\cite{lake1996containing}.  In a similar line, the field of social psychology further explores the origin and role of fear in intergroup conflicts. Fear often arises from the lived experiences and past memories consciously or unconsciously held by individuals and groups. Jarymowicz and Bar-Tal discuss extensively how fear is a spontaneous and primary emotion that evolved as a response to violence and traumatic situations from the past~\cite{jarymowicz2006dominance}. Overcoming group-level fear proves to be challenging, as fear serves as an adaptive mechanism for individuals and groups to cope with adversity~\cite{jarymowicz2006dominance}. Group-level fear overrides hopes, fosters insecurity, generates mistrust, and hampers peaceful conflict resolution, as groups rely on past assumptions and threats~\cite{jarymowicz2006dominance}.


%In this paper, we particularly focus on the social and political psychological aspects of fear especially as they pertain to group coexistence.  Prominent among the scholars who have provided insights into the instrumental role of fear in lived experiences and existential questions is the theologian and philosopher Søren Kierkegaard. Kierkegaard explained how fear plays a role in helping individuals adapt to crises, while also addressing the irrational fear associated with embracing uncertainties and the unknown~\cite{kierkegaard2013fear}.

% in the context of ethnic conflicts and peacebuilding efforts


%###########

%extend our discussion to frame and situate our work within two lines of scholarship within CSCW: first, the marginalization of religious minorities in public spheres in general and social media in particular, and second, addressing fear in the design for religious minority voices in CSCW. Finally, in the Findings section, we draw from the theories of the spiral of silence, politics of emotion, and communication accommodation to frame and discuss our findings from the study.


%CSCW has a sizable body of literature that gives insights into online polarization on social media platforms and discuss solutions for mitigating them. Nelimarkka et al. point out that as opposed to the social media’s ambition for deliberative and democratic discussion on social media, people tend to engage with ideologically like minded people resulting in political polarization~\cite{nelimarkka2018social}. The authors suggest prompting users with different viewpoints before they post something online might help to mitigate polarization. Kim et al. presents the design and evaluation study of StarryThoughts, a socio-technical system for expressing and exploring diverse opinions on social issues online~\cite{kim2021starrythoughts}. Their evaluation study suggests that the demographic information of the author of a post helps others to put the content of a post more contextually, empathize with the users, and even be more receptive with the opinion that might contradict their own. Wang et al. use the Moral Foundation Theory to categorically present posts and comments to the readers of news articles with the goal for bridging ideological divides~\cite{wang2022designing}. The authors find that this system made visible the confluences and differences of the moral framing of news articles and made users to be conscious of and learn about moral differences. Bail et al. found that intergroup communication has helped produce more effective deliberation in other contexts by promoting compromise and mutual understanding in intergroup ideologies and politics~\cite{bail2018exposure}. In summary, the above and other works~\cite{semaan2014social, terren2021echo, baughan2021someone} within CSCW explore design and policy suggestions starting from exposing users to various political perspectives to use compromise and mutual understanding as design resources. These insights build upon various assumptions about the contexts and support infrastructures in public deliberation, including democratic voices irrespective of faith-based identities, an increasingly unrestricted culture of practicing freedom of expression and identity, moral and legal support in unsafe situations, and an emphasis on the ``modern’’ and rational value systems.


%To cope with the negative experience and navigating other online safety related issues, the minority communities often find the social media platform policies misaligned and sometimes hostile to them. For example, minority communities are often forced to conform to the universal platform politics and marginalized further~\cite{shahid2023decolonizing, feuston2020conformity}. Because of the social media platforms' universal content moderation policies, minority communities loose personal contents more frequently than majority groups even when the contents follow community guidelines~\cite{feuston2020conformity, haimson2021disproportionate}; the platforms have lack of resources to filter out contents that are made for ridiculing and bullying minority communities~\cite{medina2020dancing}; individuals in the community go through extra burden to seek support~\cite{feuston2020conformity}; and the social media platforms have lack of policies to be inclusive of minority communities in increasing minority participation~\cite{saha2019language}. Moreover, the moderation policies and support for minority communities are weaker in the Global South, as moderation policies are often oblivious of the context and culture of the global south population~\cite{shahid2023decolonizing}. These findings suggest that social media policies are barely adaptive to non-dominant identities, norms, and their ways of being. To address these limitation and better support minority communities, CSCW is increasingly drawing on various justice framework to integrate into CSCW design~\cite{xiao2023addressing, erete2021applying}. We particularly draw on one of these frameworks in this paper, namely restorative justice~\cite{xiao2023addressing}, particularly because of its capability to support religious minority communities to address fear.

%One nascent body of literature is focusing on restorative justice to mitigate harm for the minority communities~\cite{xiao2023addressing, xiao2022sensemaking, chatlani2023teen, rabaan2023survivor}. Social media companies often address online harm following a justice model primarily centered on ``isolation and punishment’’~\cite{myers2018censored, vaccaro2020end}. While social media platforms offer users the ability to customize posts, report, delete, block content, and contest moderation decisions, these features effectively place the burden on users, especially the ones with minority identities, while holding the power in their hands. These actions support the platform's governance, moderation, and regulation within the framework of isolation and punishment. In contrast, the proponent of restorative justice within CSCW are arguing for turning the attention from platforms to the vulnerable and affected communities and supporting them~\cite{salehi2023sustained, xiao2023addressing}. Restorative justice prioritizes the victims of online harms by restoring communal bonds and relationships~\cite{xiao2023addressing}. Alongside modern values of freedom, equality, accountability, and deliberation, concepts like healing, apology, social harmony, and other human virtues~\cite{xiao2023addressing} are receiving attention in addressing online harms through restorative justice. While these directions offer hope for supporting the victims, as we will argue bellow, the literature needs to contextualize restorative justice to account for the social-psychological and political aspects of fear in South Asia.

%Religious sensitivities, which is more prevalent in South Asian everyday life and national politics, reinforces discrimination and fear against religious minority communities~\cite{bhatia2021religious, bhatia2022hindu, mohan2015locating}. Far-right religious nationalists in South Asia employ social media to perpetuate social fear, discrimination, and stereotypes against minority castes and religions~\cite{vaghela2021birds, bhatia2021religious, mohan2015locating}. Even people who are friendly in society, exhibit hostile and discriminatory behavior through trolling, cyber-bullying, and other online means towards religious minority communities~\cite{bhatia2021religious}. The politics of fear are often supported and normalized by political parties that benefit from such narratives~\cite{bhatia2022hindu}. Altogether, religious minority groups are depicted as both perpetrators and victims of online violence~\cite{kirmani2008competing, bhatia2022revolution}. This is in this context we emphasize that fear add an extra layer of challenge in supporting victims through restorative Justice. To address this gap, we draw from our findings to povide design and policy implication to address fear and better support religious minority communities in the Global South.


==> sections/method.tex <==
\section{Methods}
To gain a deeper understanding of how the diverse social and political psychological impacts of fear exacerbate the marginalization of religious minority communities in Bangladesh, we conducted a detailed qualitative study, which is presented in this paper. This section discusses our recruitment for semi-structured interviews and the data analysis method. Finally, we discuss and reflect on our positionality in relation to this study.

\subsection{Data Collection}
We used semi-structured interviews for data collection in our study. To recruit participants, we primarily used purposive sampling~\cite{suri2011purposeful}. The recruitment criteria for someone to be eligible to participate in our study were that they have to identify as a member of the Bangladeshi Hindu, Buddhist, Christian, Indigenous, or atheist communities and have used social media for at least a year. We only considered individuals of 18 years or over for our study. We circulated our call for participants on online social networks (e.g., Facebook). We also benefited from word-of-mouth advertisements about our study. After interviewing the first few participants, we started running a snowball sampling~\cite{goodman1961snowball} to recruit more participants until theoretical saturation was met. We summarize the demographic information of our participants (n=20) in Table~\ref{tab:participants}.

Due to the sensitivity of the topic of this study, establishing a sense of trust between the interviewer and interviewees was vital. Therefore, the author, who knew someone personally or had the closest social affinity with them, interviewed that particular participant. We interviewed the participants in person or through audio calls using their preferred mediums (e.g., Zoom, phone calls). Before starting the interviews, we briefly explained key points about participation, data management, and its intended use for scholarly writing. Then, we shared the informed consent document with them and asked permission from them to record the audio of the interviews. Once they read and verbally agreed with the terms in the document, we started the interviews. Participation in the interviews was voluntary, and no compensation was offered.

\begin{table}[!ht]
    \centering
    \caption{Demographic information of the participants.}
    \label{tab:participants}
    \begin{tabular}{p{1.5cm}p{1cm}p{1.3cm}p{2.5cm}p{2cm}p{3.5cm}}
    \toprule
    \textbf{Identifier} & \textbf{Age} & \textbf{Gender} & \textbf{Education} & \textbf{Occupation} & \textbf{Religious background} \\
    \midrule
        P1 & 25-30 & Female & Bachelor's & Unemployed & Christianity\\
        P2 & 25-30 & Female & Bachelor's & Unemployed & Buddhism and\newline Indigenous\\
        P3 & 20-25 & Female & Higher secondary & Student & Buddhism\\
        P4 & 20-25 & Male & Higher secondary & Student & Hinduism\\
        P5 & 25-30 & Male & Bachelor's & Research assistant & Hinduism\\
        P6 & 25-30 & Male & Master's & Unemployed & Hinduism\\
        P7 & 20-25 & Male & Higher secondary & Student & Hinduism\\
        P8 & 25-30 & Male & Higher secondary & Student & Hinduism\\
        P9 & 20-25 & Female & Higher secondary & Student & Hinduism\\
        P10 & 20-25 & Male & Higher secondary & Student & Hinduism\\
        P11 & 25-30 & Female & Bachelor's & Unemployed & Hinduism\\
        P12 & 25-30 & Male & Bachelor's & Unemployed & Hinduism\\
        P13 & 20-25 & Female & Higher secondary & Student & Hinduism\\
        P14 & 25-30 & Non-heteronormative & Bachelor's & Job holder & Hinduism\\
        P15 & 20-25 & Male & Higher secondary & Student & Buddhism\\
        P16 & 25-30 & Male & Bachelor's & Unemployed & Hinduism\\
        P17 & 20-25 & Female & Master's & Job holder & Hinduism\\
        P18 & 30-35 & Male & Master's & Job holder & Buddhism\\
        P19 & 20-25 & Male & Master's & Student & Hinduism\\
        P20 & 25-30 & Male & Bachelor's & Unemployed & Hinduism\\
    \bottomrule
    \end{tabular}
\end{table}

The interviews began with demographic questions and asking about their general experience and use of social media. Then, in our discussions with our participants, we encouraged them to reflect on and share their recent experiences on social media, especially those of conflict, unease, and discomfort. We sought to understand whether and how often such experiences are entangled with religious identities. Later in the conversation, we asked about their views on whether and how those interactions on online platforms translate to real-life marginalization of religious minority communities. We further asked them follow up questions to reflect and share their perception about the roles of different institutions, religious leaders, misinformation, and intersectional identities in the marginalization of religious minorities and how technology influences their online and offline experiences.

During the interviews, we took detailed notes about their non-verbal cues. We did not gather any personally identifiable information. All interviews were conducted in Bengali; each session typically lasted an hour. We transcribed and translated the interviews into English and deleted the audio recordings. To further de-identify the data, we removed all identifiers from the transcripts so that those cannot be linked to any individual.

\subsection{Data Analysis}
We combined inductive coding with theoretically guided interpretation for our data analysis. Such combinatory approaches are commonly used in HCI and CSCW research~\cite{das2022collaborative, semaan2016transition, kumar2018uber, rifat2019breaking}. We used MAXQDA, a qualitative data analysis tool, to inductively analyze the data. Four authors collaboratively engaged in the iterative inductive coding of the transcripts at weekly online meetings. In this phase, we identified abstract representations of objects, events, and interactions which repeatedly appeared in the transcripts. We also juxtaposed the notes we had taken during the interviews with the transcripts to complement our data analysis. Some examples of open codes in our analysis were \textit{``monitoring social media users' reaction and comment to recent events of communal tension''}, \textit{``observation of participants' interactions on social media by religious majority users''}, \textit{``paying attention to social media influencers' role during events of communal tension''}, and `\textit{``remembering both online and offline interaction with individuals from the religious majority community''}. Since interview data are contextual, following McDonald and colleagues' recommendations~\cite{mcdonald2019reliability}, we did not report an inter-coder reliability score. Upon generating the open codes, we noticed their close relationship and frequent mentions of concepts like fear, surveillance and the role of social media, and communication strategies in tense discussions.

Following the conclusion of our inductive analysis stage, we proceeded to peruse related literature to gain a deeper and theoretically guided understanding of the codes generated based on our participants' insights during the interviews. This exploration led us to Elisabeth Noelle-Neumann's ``spiral of silence''~\cite{noelle1974spiral, noelle1993spiral}, Sara Ahmed's concept of ``cultural politics of emotion''~\cite{ahmed2014cultural}, and Howard Giles' ``communication accommodation theory''~\cite{giles2016communication}. Neumann's theory explaining how and when individuals tend to remain silent or conform to majority opinions when they perceive their own views to be in the minority due to a fear of isolation or social backlash~\cite{noelle1974spiral, noelle1993spiral} was comprehensive to understanding Bangladeshi religious minority communities' experience in social media and how their voices are silenced. Ahmed's work helped us interpret our participants' views and situate those within broader South Asian socio-psychological and institutional power relationships, as she explains how emotions are not only personal experiences but are also shaped and influenced by cultural norms, power structures, and social expectations~\cite{ahmed2014cultural}. Finally, Giles' theory~\cite{giles2016communication}, which suggests that individuals adjust their communication patterns to either converge or diverge with others, depending on their motivations to either emphasize similarity or difference in social interactions, was useful in understanding the Bangladeshi religious minorities' interaction strategies on social media and offline. Thus, these three theories feed each other in a way that helps us understand our participants' perspectives in relation to the politics of fear in Bangladeshi religious minority communities and how it is mediated through social media platforms. 

\subsection{Positionality and Reflexivity}
Prior research in HCI has highlighted emerging tensions around exploitation, membership, disclosure, and allyship in studying marginalized communities~\cite{liang2021embracing}. Therefore, it becomes immensely important to account for these tensions while moving forward with this study. In understanding the marginalized communities' experiences, the authors’ race and ethnicity reflexively bring certain affinities into perspective~\cite{schlesinger2017intersectional}. All but two (who are Americans) authors of the paper were born and brought up in Bangladesh. Two of them belong to the Bangladeshi religious minority Hindu community, while three authors were born in the Bangladeshi religious majority Muslim community. Six authors of this paper identify as cis-gender men, and one as a cis-gender woman. The paper's authors have research experience in postsecular, decolonial, and postcolonial computing, the relationship between faith and technology, and various marginalized identities in the context of the Global South, especially in Bangladeshi communities. The authors' lived experience and research background motivated them to study how the Bangladeshi religious minority communities' experiences are mediated by technology and put them in the capacity to prioritize the agency of local marginalized communities in computing research.

%\subsection{Limitations}
%One primary limitation of our study is the limited age diversity of our participants. While the diversity of religious backgrounds is also limited, it is commensurate with these communities' population distribution in the country~\cite{bbs2022preliminary}. In this study, we have focused on broadly defined religious minority communities in Bangladesh. However, there are various nuances within religious communities in Bangladesh (e.g., Matuas--a Hindu sect primarily comprising of underprivileged castes like the \textit{namasudras}~\cite{lorea2020religion} and Ahmadiyyas--a minority Islamic sect~\cite{uca2023bangladesh}) that also face marginalization in the country in myriad ways due to their intersectional faith-based identity. The present study is part of a larger project to understand the experiences of various marginalized communities in the Global South, and our future works will focus on how the users of intersectional faith-based identities face marginalization on social media. This paper presents a semi-structured interviews-based study. While interview data are useful for understanding individuals' experiences, future work should also use qualitative and quantitative content analysis-based approaches to understand the dynamics of the interaction of religious minority communities around times of national sociopolitical important events. Moreover, our study is based on perspectives shared by a set of participants with somewhat homogeneous demographics. In the case of this paper, similar to the nature of qualitative research~\cite{leung2015validity}, our objective is not to produce generalizability but rather to study a specific process in a defined context.

==> sections/results.tex <==
\section{Findings}
We draw on the theories from social-psychological and cultural studies of fear to report three patterns of marginalization of the minority communities’ social media use: (a) the fear of isolation and the spiral of silence, (b) the politics of fear, and (c) coping with fear and marginalization. The theories provide us with the analytical lenses to analyze our findings that contribute to ongoing discussions in CSCW on identity, faith, and polarization with broader implications of making online spaces safer for marginalized communities.

\subsection{Social Psychology of Fear: The Spiral of Silencing of Minority Perspectives}
People feel increasing pressure to suppress their views when they perceive themselves as being in the minority, as they fear social isolation and exclusion. Based on this idea, Noelle Neumann theorizes the ``spiral of silence''~\cite{noelle1974spiral} that explains the growth and spread of public opinion. According to her, people closely observe their social environment to decide whether their opinion conforms with normative views. People tend to remain silent about opinions if they are likely to face social disapproval, while more likely to voice popular or dominant opinions. This fear of isolation stems from the belief that minority opinions would be seen as deviant and face negative consequences. Over time, mass and social media lead to a spiral effect where the minority opinion is further marginalized~\cite{gearhart2015something}.

\subsubsection{Quasi-Statistical Organ: The Frequency Distribution of Public Opinion and The Feeling of Harmony}\label{quasi-statistical-organ}

The willingness of our participants to speak up or remain silent is significantly influenced by their perception and assessment of the social climate surrounding them. This pattern of minority communities' engagement in social media activities aligns with the principle outlined in the spiral of silence theory described as the quasi-statistical organ~\cite{noelle1974spiral}. People self-censor themselves by continually assessing the prevailing trends, the frequency of voices that align with their own convictions, and the perceived reasonableness of those voices~\cite{noelle1974spiral}. Thus, by carefully observing the social environment, the quasi-statistical organ helps individuals evaluate situations where expressing their views may disrupt social harmony, thereby instructing them to remain silent.

% general idea is mixed: support, opposition, and silence.
Our findings demonstrate several indicators through which social media users from minority communities develop their quasi-statistical organs. These indications come from observing others' use of various reaction emoticons and the number of comments expressing support or opposition. They assess how the discussants in a social media post approach a topic, particularly when it relates to their rights associated with faith. They usually feel comfortable expressing their opinion in a moderated civil discourse, whereas identifying stubborn or aggressive users among the discussants discourages them from speaking up. Participant P7 described his strategy for deciding whether his views align with the majority opinions and explained his rationale behind remaining silent in case of holding a minority view in an argument:

\begin{quote}
    I see the situation around me. When you see that you are outnumbered, you will be just listening, you won't like to stay in those arguments. On top of that, arguments do not end on Facebook. Someone may make me a target even after the argument is over on Facebook. Then why should I go into a conflict? I should be even more careful. That is why I don't engage in an argument. [P7, Male, Hinduism]
\end{quote}

While individuals from minority communities monitor social media posts and discussions to gauge the amount of support, their social media activities are also subject to public surveillance, especially from the majority religious groups. A few of our participants described their experience or knowledge of such cases where unrest was incited by a tip-off from those who were in opposition to minority views. In other cases, surveillance of minorities' is followed by condescending lectures or mass reporting of minorities' posts that aim to reinforce a dominant perspective. Examples of these included justifying vandalization and violence and alleging the victims of religious minority communities as responsible for such incidents. These experiences motivate our participants to stop interacting with certain individuals. One of our participants, who also identifies with a non-heteronormative sexual orientation, described how their intersectional identity was being surveilled:

\begin{quote}
    In last year’s pride month, the chairman of 10 Minute School\footnote{An online educational platform in Bangladesh} posted a pride flag and said something like Happy pride month. I gave a \emoji{heart} reaction to that post. One of my friends saw that, and then he gave me a lot of lessons. He said, you have a love reaction to the post, but remember, [LGBTQ identity] is never going to be legal in Bangladesh. After that, for my own safety, I think a lot before reacting to a post. [P14, Non-heteronormative, Hinduism]
\end{quote}

Contrary to these stories of suppressing minorities' voices on social media, some participants also shared stories of how they received social support in times of such crises and marginalization. Social media helped them to find and connect with others of similar identities and perspectives. Whereas they were concerned that many mass social media users in the past supported the violence or remained silent, they found hope in the emerging support for religious minorities from renowned people whom they described as ``celebrities'' on social media. They are also appreciative of the growing solidarity and strong opposition from the majority Muslim community against radicalism. Participant P4, to describe the social support he received from his friends and acquaintances from the Muslim community, said:

\begin{quote}
    I really appreciated that when the Hindu communities were victims of the violence of 2021, several of my Muslim friends and seniors messaged me to say sorry out of nowhere. They were not responsible for the violence or involved in anyways with those, and I was not a direct victim of those incidents. Still, they said sorry on behalf of others. They called me over the phone to check in with me. [P4, Male, Hinduism]
\end{quote}

Beyond concrete incidents of communal violence, our participants described how the social media landscape has affected traditional inter-faith cultural practices. Several of our participants explained this phenomenon with the example of social media debate during their biggest religious festival, Durga Puja. Despite the longstanding tradition of Muslims and Hindus exchanging foods and Muslims visiting Hindu temples, some Islamic clerics preached against this practice, labeling it as a prohibited (\textit{haram}) act. Followers of these preachers inundate social media platforms during Puja, cautioning their Muslim peers to abstain from such cultural practices. Our participants thus were doubtful about inviting their Muslim friends during Puja, fearing that their sense of intimacy with their Muslim friends would be hampered. Some participants even reported instances of personal attacks on their Muslim friends who visited them during Puja. There was a counter-trend, too. Many Muslims on social media amplified such interpretations by emphasizing that visiting a Hindu temple and accepting halal food have no bearing on their own faith. Instead, they argue that these traditions foster tolerance and empathy among religious groups, virtues upheld in all religions. However, as our participants explained, the comparatively liberal voices constitute a minority on social media and are often rudely dismissed by the majority.

The above findings, along with others, illustrate how religious minority communities choose to remain silent or speak out based on the frequency distribution of public opinion. The stronger voices of the majority invoke fear and intimidation, influencing the religious minority communities' decisions regarding participation on social media.

\subsubsection{The Fear of Isolation: Seeking Societal Approval and Maintaining Reputation}
The spiral of silence theory presents a social-psychological concept of the public sphere~\cite[p. 61]{noelle1993spiral}. Within this framework, people exist within a society where they are consistently subjected to the scrutiny and evaluation of what she referred to as the ``anonymous court''~\cite[p. 62]{noelle1993spiral}. As people develop their quasi-statistical organs to assess their social environment, the fear of isolation, disrespect, and unpopularity among the dominant group serve as guiding forces, compelling them to conform to the established social norms and actively seek social signals of reputation.

Participants shared their experiences of discussing religion on social media platforms and how it changed later online interactions. In the cases of resisting the social pressure of constantly being preached about orthodoxy, communal hierarchy, and superiority and proposals for religious conversion, many users from the majority faith got disappointed and stopped talking with them. Upon losing many social contacts due to differences in opinion, some participants made conscious changes in how they represented themselves to their online and offline social peers. Participant P7 talked about how some of their friends from religious minority communities presented themselves to avoid social isolation:

\begin{quote}
    I have some friends whose families are religious--practicing Hindus who observe the rituals sincerely. But when they come to campus, because of being afraid, they try to prove themselves secular in front of [Muslims] and do not participate in the religious programs on campus. They act secular to avoid being singled out or to keep their connection with them [the majority community] safe and sound. [P7, Male, Hinduism]
\end{quote}

In addition to the rationale of maintaining good social relations and reputation, given the history and contemporary instances of religious marginalization in various ways, several participants were advised by their families not to present themselves differently for the sake of getting along with religious others better. Participants' families sometimes object to their presence on social media altogether. Therefore, some maintain secret social media profiles and find support through covert social media activities like passive browsing of various posts and venting out to close friends in direct messages. Participant P17 explained how family guidelines affected her response and strategies to find support on social media,

\begin{quote}
    The way I was brought up, there was always this impression that I could not be identified as someone different. You know, there was this time in Bangladesh when being Hindu was risky. There was a lot of violence at some point. From then, we have learned that we cannot say anything out loud on social media. When I see a post, I get hurt, keep that feeling to myself, and just choose not to react. I just go to my friend's inbox and start a conversation about it. [P17, Female, Hinduism]
\end{quote}

To safely and freely express themselves and their concerns, our participants highlighted the importance of their allies from other religious communities. Most participants' social circles expectedly included many people from other religious communities. Similar to the discussion earlier in~\ref{quasi-statistical-organ}, our participants were thankful for various moral and professional support of their friends and acquaintances from the majority Muslim community. They did not dismiss the contributions of their compassionate compatriots because of the bad actors. However, they emphasized how belonging to a majority community brings certain power to speak up on social media that many users from religious minority communities cannot afford. For example, participant P20 expressed his expectation for visible public solidarity and societal approval by saying,

\begin{quote}
    Take the example of the religious debate about eating pork or beef. If you look around you in real life, you will obviously see people supporting you, whatever you decide. But the same people would be silent on social media. It feels like I don’t know them. [Silence] gives encouragement to those who spread hatred. [P20, Male, Hinduism]
\end{quote}

In addition to highlighting the importance of social support and allies from different religious communities, our participants emphasized the detrimental impact of stereotypes propagated through social and mass media. These patterned narratives contribute to the silencing of marginalized communities and the conflation of perceptions. Furthermore, rituals and identity are often misunderstood and stigmatized, reinforcing the othering of religious minority communities that we elaborate on next.

\subsubsection{Stereotypes and Unconsciousness of Perceiving the Social Climate and Reinforcement of Spiral of Silence}
The development and spread of both positive and negative stereotypes -- preconceived notions or generalizations about a particular group of people based on their characteristics, traits, or social identities that are accelerated and intensified through social and mass media -- can further contribute to silencing marginalized communities~\cite{gearhart2015something}. People tend to simplify social complexity and subtlety, constructing a simplified social environment model. In this process, individuals often rely on consuming indirect experiences and conflating them with their own perceptions. While minorities are particularly sensitive to what Neumann called the ``climate of opinion''~\cite[p. 161]{noelle1993spiral} or ``silent majority''~\cite[p. 93]{noelle1993spiral}, stereotypes about certain groups may lead them to assume that the majority opinion aligns with those stereotypes. For example, in the absence of all voters' participation in social media discussion and people's tendency to construct simplified social environmental models, people often conflate others' political opinions using stereotypes, such as in the US political landscape, where certain ideas are mentally associated with democratic or republican parties even though the landscape of political opinions is much more nuanced and complex~\cite{wilson2020polarization}. At this point, they become unconscious of the influence of mass and social media in public opinion and interaction~\cite{noelle1974spiral} and unable to differentiate their own perceptions from those of others~\cite{noelle1993spiral}. Consequently, the perceived negative climate of opinion creates a more unstable environment for religious minority communities, influencing their willingness to express their views openly, suppressing divergent opinions, and reinforcing the dominance of the prevailing viewpoint.

Our participants mentioned how rituals, dietary practices, and materiality of identity become important points in forming cultural stereotypes, stigmatization, and alienation of religious minority communities. There exist people who are genuinely curious about the lifestyles of religious minorities and indigenous communities -- how their houses or places of worship look. However, participants emphasized the negative experiences of being stigmatized based on stereotypes about them. For example, most of our Hindu and Buddhist participants discussed how people often ridiculed and undermined their rituals as worshipping idols without understanding the idea or philosophy behind such practices. Our participants, on several occasions, debated with people from Muslim communities about their religious dietary choices (e.g., Hindus not eating beef or Buddhists and Christians eating pork), where their peers and, on some occasions, strangers from the majority community often tried to convince them otherwise. A few participants also shared how their appearance was often judged from the majority religious perspectives instead of their own. For example, one participant received pressure to convert to Islam due to their beards, while some received negative comments and messages after expressing their opinion on wearing ornaments. These stereotypes and material notions of identity expression often contribute to the othering of religious minority communities. The conversation also mentioned the influence of \textit{hujurs} and religious leaders in spreading negative stereotypes. As participant P8 said,

\begin{quote}
    People from outside of the Hindu faith often talk about Hindu practices. Some people from the Muslim community often say vulgar things about our female deities, often in waz mahfils, which creates discomfort in me. Let's say there are 100-150 people at a waz who are coming out of that event, getting a negative impression about Hinduism, or are influenced to think of Hindus in a negative way. [P8, Male, Hinduism]
\end{quote}

These stereotypes being embedded within the social perception make religious minorities (e.g., Hindus, Buddhists, Christians, and Indigenous) and the religious majority Muslim communities see each other as intrinsically different, leading to communal distrust. As discussed in section~\ref{research_site}, many recent incidents of communal violence in Bangladesh were incited by rumors of disrespect to religion. Because of communal distrust and stereotypes, in case of incidents like Quran desecration, Muslim communities are influenced to believe that someone from another religion is behind the act without critically considering the possibility of other kinds of politics and the self-interests of someone from their own community. Such hasty speculation about other religions, especially the minorities, marginalize those communities unfairly and disproportionately. Participant P19 described his perspective, saying,

\begin{quote}
    I think the reason behind the conflict [in 2021] was political. If you think about it, whoever belongs to a minority community in a country, usually tries to save themselves, whether Muslims in India or Hindus in Bangladesh. So, in Bangladesh, no Hindu person would dare to agitate the Muslim community. So, I think any politically motivated fundamentalist or someone like that did it. When they started vandalizing the idols, I felt like an inferior person, and a constant fear was in my mind. [P19, Male, Hinduism]
\end{quote}

Our participants expressed their expectation of a more positive role from Muslim religious leaders. Like social media microcelebrities' role in shaping sociopolitical discourse in Bangladesh~\cite{das2022understanding, rifat2022situating}, they believe that religious influencers -- the preachers who are widely popular on social media for their Waz~\cite{rifat2022putting} -- have greater social responsibilities in these cases. Especially given the different possible interpretations of religious texts, according to our participants, some preachers try to asses whichever interpretation attracts mass people. While participants appreciated some preachers who highlighted religious harmony through their interpretations, they also expressed concerns about some preachers propagating triggering interpretations for popularity. Participant P5 described his view as follows:


\begin{quote}
    Some [religious preachers in Islam] talk about how their religion is better than everyone else's. There are also some of them who discourage insulting other religions. They talk about differences but encourage harmony [among all religions]. ... However, they are very few in number, say one in a hundred. ... Different speakers preach different interpretations. ... Honestly, when it comes to religion, people are overly sensitive and often highlight the negative sides of others. [P5, Male, Hinduism]
\end{quote}

Using Neumann's theory, we understood how individuals in the religious minority community observe their social environment, often feel pressured to suppress their views due to the fear of social isolation and exclusion, and how social media mediate their experiences. These individual experiences are also entangled with the South Asian context that we discuss later in this paper.

\subsection{Politics of Fear and Social Control}
The spiral of silence theory provides insights into the social psychological patterns through which religious minority communities subconsciously or unconsciously regulate their behavior on social media leading to marginalization. Our findings show that such fear is facilitated through a power relationship between the minority communities and South Asia's broader social, cultural, and state institutions. To examine this pattern of the political aspects of fear, we turn to Sara Ahmed's influential work, ``The Cultural Politics of Emotion''~\cite{ahmed2014cultural}. Ahmed's theoretical approach to explicating the intricate relationship between power and the politics of fear gives insights into how socially powerful entities frequently employ fear as a means of control. This framing of the politics of fear allies with the spiral of silence, as Ahmed highlights the political dimensions of fear and its role in perpetuating social marginalization. Drawing on her theory, we discuss how religious minority communities also become victims of external fears from religious and cultural institutions that exert political control over them.

\subsubsection{Economies of Fear}
Drawing on the political theories of Machiavelli and Hobbes, Sara Ahmed discusses how fear has been historically used as an instrument for disciplining, punishing, protecting, and governing the less powerful by civil societies and the people upper in the power hierarchies~\cite{ahmed2014cultural}. Beyond the forms of controls by states and power-hungry individuals and institutions, Ahmed also discusses fear as a ``symptom''  of modern life. Ahmed explains how fear has made people hyper-conscious about the age-old values and traditions, where people anxiously change their habits, norms, and behaviors to manage and live within a culture of fear to conform to the ``modern'' ways of being. On top, she presents fear as a boundary-defining emotion between the ones that are threatening and the ones that are threatened~\cite{ahmed2014cultural}. In other words, Ahmed describes how fear originating from power politics and institutions may marginalize a community by creating artificial insecurity, stigma, and stereotypes.

%Because of the history of colonial divide-and-rule in the region and the subsequent partition of Bengal based on religion, national identities like Bangladeshi and Indian are often conflated with religious Muslim and Hindu identities, respectively~\cite{chatterji2002bengal, das2021jol}. 
Our participants discussed how majoritarian violence against minorities operates in a transnational context and creates a politics of power in which fear is utilized as an instrument to establish and perpetuate power dynamics. For example, Hindu minorities' sufferings in Bangladesh can be used by communal politicians in India to justify their discrimination against Indian Muslims. Similarly, the marginalization of Indian Muslims or Rohingya Muslims is often used as an excuse by many Bangladeshi Muslims to dismiss the marginalization of Bangladeshi Hindus or Bangladeshi Buddhists. As a result, the transnational politics of justifying minority oppression instills fear within the minority communities, making them hesitant to speak up, especially given the ease with which majority voices can superficially find "evidence" to target and attack these minority communities. Participant P5 shared what his family experienced as a Bangladeshi Hindu minority in the aftermath of a major communal riot in India:

\begin{quote}
    I did not receive any threats myself, but my family members did. Once there was a big riot before we were born [was referring to the riot incited by the Babri masjid demolition in India in 1992]. My cousin told me that the chacha [Muslim neighbor], who had a good relationship with us till two days before, rushed to our house to beat my uncle. The good relationship they had worsened all of a sudden. [P5, Male, Hinduism]
\end{quote}

Our participants also shared incidents where institutions successfully intervened to diffuse tension and the possibility of violence against minority communities. They described amidst the instability and communal sentiment in many districts across the country during such a crisis, local governments and law enforcement authorities in some localities were proactive in ensuring their security and mitigating fear. Our participants discussed both the sincerity and shortcomings of state institutions and how they felt and thought during contemporary major incidents like attacks on Buddhist temples in Ramu in 2012, the attack in Holey Artisan in 2016, and the vandalization of Hindu temples and houses in many districts in 2021. However, beyond these major incidents, our participants shared stories of their everyday marginalization, both online and offline, for example, being called a \textbengali{''ভারতের দালাল''} (\textit{``Bharoter dalal''}: Indian agent) for being a Hindu in Bangladesh. Such everyday experiences, recent major incidents, and past occurrences altogether install a sense of constant fear, inferiority, insecurity, and alienation in the religious minority communities' memories. Like the history of late colonial British India~\cite{pal2021partition}, our participants described the women from minority communities as being particularly targeted for harassment. Participant P2 shared her memory, saying,

\begin{quote}
    We basically face it from a very early age. I have realized it more clearly after the incident of 29th September [in 2012]. ... It's not like that nobody supports us. ... The things that have been destroyed have been rebuilt very beautifully. Since I am from Ramu, I know well those who had faced casualties had been helped enough. But even after reestablishment, the fear never really fades away from the mind. ... When they were coming to set fire, they were giving some slogan that I can clearly remember. That night, we were sitting in the courtyard, all helpless, thinking about where we were living! That night is like the worst nightmare in my life! I don’t talk about it usually. [P2, Female, Buddhism, and Indigenous]
\end{quote}

Our participants discussed how social media exacerbates their marginalization. Our participants agreed that fundamentalist voices from the majority communities are often louder and more active than the supportive voices on social media. They believe the former actively tries to make religious minorities feel inferior and fuels communal violence for political motivations. They mentioned some stories covered by mainstream media in the past years where fake social media accounts with Hindu or Buddhist names were used to post religiously insensitive content and agitate Muslim communities as examples. The perpetrators of these fake social media posts often remained unidentified and unpenalized. Participants described their disappointment about the lack of judiciary actions against such malicious social media identity frauds and, consequently, their fear about being visible on social media through malicious fake accounts. As one participant said:

%~\cite{tribune2017justice, rezwan2016phony, chowdhury2021man}

\begin{quote}
    I avoid sharing or posting anything. It often happened that someone opened a fake ID, pretended to be a Hindu person, and posted things that led to violence against the Hindu community, and nothing happened after that. The person who opened the fake ID is not identified or jailed. In such a situation, those who want to speak up are painted as someone trying to spread chaos, which is why I try to be silent. [P17, Female, Hinduism]
\end{quote}

Due to the fear instilled by social and often State institutions, resulting in the internalization of their fear of openly expressing their views on social media, Bangladeshi religious minorities facing discrimination (such as Hinduphobia and Atheophobia) often seek out confined and hidden spaces on these platforms to find communities and social support. However, our participants demonstrated their frustration with those groups and held the moderators responsible for not allowing everyone to speak up in those spaces. Describing those moderators using metaphors like ``elite circle'', ``judge'', and ``law enforcing agency'', the participants discussed how those group admins' and moderators' gate-keeping based on caste, sect, and sexuality obstructed their freedom of expressing identity and opinions and instilling fear even within those confined groups.

%like other marginalized communities (e.g., LGBTQ+ communities facing trans and homophobia~\cite{walker2020more}, Muslims facing Islamophobia~\cite{das2021jol}), 


\subsubsection{The ``Uncertainty'' of Future and the Impression of Fear in the Present}

Sara Ahmed describes that the ``object'' of fear does not necessarily have to be present ``here and now''~\cite[p. 65]{ahmed2014cultural}. Rather, anticipating an uncertain future makes people fearful in the present. We discussed earlier our participants' fear of being represented on social media in a way that can be exploited for inciting violence by fundamentalists who use religion for political gains. With the fear of constantly being surveilled, our participants talked about their practices to remain mindful of their social media activities and their accounts' security and access. In Participant P18's words,

\begin{quote}
    When I used to see posts ridiculing my religion, I commented and made my arguments. But later, I realized it was not good for me in the long run. It may instead grow anger towards me. Recently, you have seen many incidents [referring to the persecution of atheist bloggers]. Now, we are even more careful. I am even careful in using public Wi-fi. I always log out from Facebook and Instagram after using them. [P18, Male, Buddhism]
\end{quote}

Our participants' observation on social media of others being objurgated, humiliated, and threatened with death, rape, etc., in case of posting religiously controversial content condition them to rarely engage in discussions on social media that hint toward religious tension. They are often afraid to be themselves at the cost of being isolated and not receiving help from their social circles. Some participants talked about their strategy of separating platforms among different social circles, for example, using Instagram for more candid identity expression and Facebook as their impression management site. In the cases of several participants, though their parents are not on social media, various incidents reported by mainstream media where communal violence had been incited using Facebook and direct observations in the neighborhoods shape those participants' family guidelines forbidding them from discussing religion and politics on social media. Such fear about self-representation scale up from individual to family to neighborhood and often upward. Participant P16 observed differences in people's perceptions of fear in urban and rural areas. They described the self-suppression and cautionary measures taken by the minority communities and also the support from some individuals from the Muslim community in their village:

\begin{quote}
    I did not feel anything in Dhaka\footnote{Capital city of Bangladesh.}, but it was a difficult time when I went to my village during the last Puja. People were getting together with safety measures to guard the temple. I liked that some Muslims also joined them. However, I could feel the fear. You know Kirtan\footnote{A popular Hindu practice of praising and glorifying a form of divinity, with its origins rooted in a Sanskrit word that signifies narrating, reciting, telling, and describing~\cite{lal2009theatres}.}? It is like Waz for Hindus. People in the temple did not even use a mic. They were doing the Kirtan in a very low voice. [P13, Female, Hinduism]
\end{quote}

Some participants discussed how the present impression of fear and uncertainty about the future as a member of religious minority communities in Bangladesh motivates them to make certain life decisions. For example, one participant mentioned his hope of gaining political support during communal violence as his motivation for joining student politics. A few participants were concerned about the declining\footnote{While the raw number of the Hindu population has increased in the last few decades (from 12.3 million in 2011 to 13.1 million in 2022), the percentage of their population is declining (from 8.54\% in 2011 to 7.95\% in 2022)~\cite{bbs2022preliminary}. Different stakeholders have often used this information to construct different kinds of narratives.} percentage of Hindu minorities in the country. They identified different reasons for this decrease in percentage, such as many from the minority communities being afraid of increasing religious intolerance and leaving the country. Participant P8 said,

\begin{quote}
    After the incidents of 2021, I saw many posts about it on social media, but very few of those were from the majority community. That’s why I fear that Bangladesh is gradually moving toward religious radicalism. The process has already started. Bangladesh is going to be the next Pakistan. [P8, Male, Hinduism]
\end{quote} %waz, education

Our participants underscored the importance of institutional support and state intervention in addressing religious minority communities' fear. Similar to international human rights organizations~\cite{riaz2021how, hrw2018bangladesh}, a few of them felt that some recent digital legislation (e.g., the ICT Act) falls short in ensuring religious minorities' freedom of expression online and disproportionately penalizes them than violators from the majority community. In addition to the disparity of representation of different religious communities in the national curriculum, some of them specifically described the erasure of Bengali Hindu writers' works from textbooks as concerning. Hence, they recommended a more pluriversal approach to curriculum design that promotes similarities and interconnectedness of different religious values. They believe that under the circumstances of increasing polarization and religious intolerance, the education system should make students conscious of the risks of such sentiment and encourage communal harmony.

\subsection{Coping up with the Culture of Fear}
Our participants exhibited various coping mechanisms in response to the social and political psychological aspects of fear associated with isolation, uncertainty, and negative emotions. We draw upon the communication accommodation theory (CAT)~\cite{giles2016communication} to illuminate these coping mechanisms. CAT has been a highly influential theory over the past years, offering valuable insights into interpersonal and intergroup communication dynamics~\cite{giles2016communication}. It provides a socio-psychological perspective on the significance and impact of power dynamics and micro-contextual factors in adjusting their behaviors in intergroup communication ~\cite{giles2016communication}.

According to CAT, people adjust their communication behaviors through convergence, divergence, and maintenance strategies. The motivation for communication accommodation includes the desire for social approval, the reinforcement of one's identity, and the aspiration to influence others to align with one's perspectives. People often try to negotiate their extent of belonging using their in-group and out-group positionalities to express one's identity. These communication accommodations are influenced by micro-social factors such as the historical relations between groups, faith, status, demography, and institutional support~\cite{giles2016communication}. Individuals often balance the ``desire to belong'' and the ``desire to be unique'' when adapting their communicative behaviors. Moreover, the accommodation extends beyond linguistic behaviors and encompasses para-linguistic, discursive, and non-linguistic cues. When individuals intentionally differentiate themselves from others in communication to highlight their identity differences, CAT terms this strategy as ``divergence''~\cite{giles2016communication}.

\subsubsection{Divergence}
As we discussed earlier, many of our participants shared experiences of being socially pressured to change their religions. In the face of these social pressures, where their religious beliefs are undermined as false or wrong by a large number of people of another religion, participants often accommodate their communication through divergence. Instead of submitting to the majoritarian views, religious minorities try to distinguish and reaffirm their religious identities. Participant P1 describing his experience, said,

\begin{quote}
    Several times a few people told me that the basis of Christianity is false. Because they believe in Jesus Christ in another way which is different from the whole belief system of Christianity. They tried to say theirs was the only true religion and had answers to everything. All other religions are wrong. Once, when I was little, probably at age 15, I was talking to a guy, and he made me say a Surah\footnote{The equivalent of ``chapter'' in the Quran, which is the sacred scripture of Islam.} [mentions the Surah]. ... Then he said you became Muslim. I asked him, ``How have I become Muslim?''. He said that you just said the Surah. Then I said, how can I be Muslim if it does not come from my heart? [P1, Female, Christianity]
\end{quote}

These divergence attempts need the participants to know about their religions more deeply. Our participants often look into their religious texts, search for references using the internet, ask questions to their family members, or reach out to religious leaders (e.g., fathers at local churches). While most of them emphasized the importance of reliable sources in discussions comparing religions and their belief systems, they also mentioned people's strong attachment to their beliefs and communities. For example, a social acquaintance of participant P7 posted about the history of historic communal riots and how those marginalized Bengali Hindu communities. One of his Muslim friends blamed the Hindus for those riots. Like several of our participants, he also described fact-checking as a ``fruitless'' effort and such divergence-based communication as a ``vicious cycle'' in such cases because of people's cognitive biases. Nonetheless, our participants highlighted the importance of distinguishing and reaffirming their religious identities and perspectives, hoping to make small changes in collective perceptions of them within the majority community. However, these efforts from minority communities often face challenges online. Participant P15 describes his experience as follows:

\begin{quote}
    A few years ago, someone posted a meme that ridiculed one of our major festivals, Maghi Purnima\footnote{One of the largest festivals observed by Bangladeshi Buddhists: \url{https://en.banglapedia.org/index.php/Maghi_Purnima}}. I posted a comment there indicating how much problems and ridicule we face from the bigger religious communities in Bangladesh. Following that comment, I received some threats in my inbox; someone told me they would report my account, post my picture to secret religious groups, etc. Following that incident, I stopped posting anything that might trigger anger among other religious communities. My profile was public back then. I made it private after the incident. [P15, Male, Buddhism]
\end{quote}

The participant described their effort to protest someone bullying their community during a religious festival. However, in their effort to reaffirm their religious identity, they were threatened with being silenced using various social media mechanisms. Several other participants shared similar stories of limiting their social media presence, activities (e.g., post, share, comment, react), and privacy settings because of fear induced by such threats and negative comments. Especially a couple of our participants who identify with intersectional LGBTQ identities shared experiences of further marginalization on social media.

\subsubsection{Convergence}
With adversarial attitudes of many social media users challenging their desire to differentiate themselves by expressing their religious identity safely and freely, many of our participants use convergence--seeking approval or when the cost of conforming is low~\cite{giles2016communication}, to cope with the culture of fear. While our participants from minority communities mostly discussed their approaches to convergence, they also highlighted the role of individuals from the majority community. They mention that certain individuals or a group of people, often religious preachers tried to take some action to address the situation, but their efforts were often limited by their locality or reach on social media. These individuals privately reached out to people they knew and either advised them to stay home or urged them to go home from sites of violence. The intention behind these calls was to control the damage caused by the violence as much as possible. However, participants also acknowledged that these individuals or groups didn't have significant power or authority to impact the situation substantially. They often distance themselves from discussions on religious differentiation to assimilate themselves with others. In such cases, they search for social support more privately. Participant P17 described her strategy for convergence, saying,

\begin{quote}
    I obviously take a position when I see these kinds of posts. But I don't engage on social media. I learn the post and then take them up to my friends and close circle and discuss with them. Yes, the defaming posts bring anger and sadness. Definitely, if someone talks badly about my religion, it makes me sad. But generally, I don't express it on social media. No one knows who might see my comments. [P17, Female, Hinduism]
\end{quote}

Several participants described experiencing such fear since their middle school days in the forms of pressures for religious conversion, ridicule, and their religious beliefs being undermined. They expressed a kind of fatigue and fear that accumulated over time, for which they eventually decided not to express and surface their religious identity in most cases openly and rarely participate in religion-related discussions online. In contrast to avoidance as a strategy, some participants deemed discussions an important strategy for convergence. However, as we discussed previously, such discussions from religious minorities often face backlash. Hence, our participants emphasized that popular religious preachers can use their social positions to shape a culture of interfaith tolerance and respect. Participant P1 expressed his expectation, saying:

\begin{quote}
    The role of religious leaders in our country is huge. One of the major sources [of influence] is social media. If religious leaders start telling people to be tolerant, it would really help. Most people in our country look up to them, and [religious speakers] are their ideal figures. [Muslim communities] follow [religious speakers]. We rarely saw any major religious leader say to empathize or forbid doing such things. [P1, Female, Christianity]
\end{quote}

As mentioned in~\ref{quasi-statistical-organ}, our participants sometimes receive support from social acquaintances from the religious majority Muslim community. They discussed with us how those conversations strive to achieve harmony and where those attempts for convergence fall short. Given the contemporary status of the communal violence against Hindu minorities in 2021, commonly referred to as \textbengali{রক্তাক্ত শারদ} (\textit{roktakto sharod}: Sanguinary Fall) by the Hindus, most of our participants mentioned that incident in their discussions. They applauded some from the majority Muslim community for condemning the violence based on the facts. However, they were also disappointed that instead of recognizing the Hindus as victims of the violence, many people were invested in impression management as a community through lengthy social media posts that often served no purpose as they tended to provide separate statements rather than engaging in meaningful discussions for supporting the victims and holding the perpetrators of that violence responsible. Participant P13 expressed her disappointment, saying,

\begin{quote}
    Rarely do people from the majority community come forward on social media and simply admit that what is happening is an injustice. They take very complex stands. For example, they described their religion's teachings and tried to prove that the person who put the Quran in the temple was not following those teachings and, thus, was not an ``real Muslim.'' They were trying to avoid responsibility as a community by disowning that person. Some were trying to paint that guy as mentally unstable. [P13, Female, Hinduism]
\end{quote}

The majority Muslim community attempted to disown Iqbal Hossain (context described in section~\ref{research_site}) through complex justifications, which can be described as an example of a community attempting to evade collective responsibility for an individual's behavior. However, our participants emphasized that to address the Bangladeshi religious minorities' marginalization, such problematic patterns should not be overlooked. While the apparent cost of ignoring these incidents to achieve convergence might be small for the religious majority communities, the consequences are more expensive for religious minority communities.

==> sections/revisedintro.tex <==
\section{Introduction}
\label{sec:introduction}
Despite the initial promise of social media platforms to foster the coexistence of diverse communities, ensure equality of voices in public deliberation, and provide a safe space for participation, these platforms have become unsafe spaces for minority communities -- the religious or ethnic groups that constitute a smaller proportion of the overall population within a particular society or region~\cite{jackson2005minority}. Over the past decade, as social media platforms gained popularity, the issue of inequality and online harms based on cultural, faith, and identity-related factors, including race~\cite{ogbonnaya2020critical, smith2020s}, caste~\cite{vaghela2021birds}, gender~\cite{bardzell2011towards, scheuerman2020we}, and religion~\cite{mizan2019silencing, rifat2020religion}, has received significant attention in academia and public discourse. Academia and the media have reported on how social media platforms have introduced and propagated new forms of online violence targeted at religious minority communities in the Global South~\cite{Human_Rights_Watch_2021, Hasan_Macdonald_Ooi_2022}. For example, over the past few years, a common pattern has emerged in which rumors defaming the holy books of Islam are spread from profiles pretending to be Hindu individuals, resulting in mob attacks on Hindu religious establishments and homes in Bangladesh~\cite{Hasan_Macdonald_Ooi_2022, Ethirajan_2021, VICE_2021}. During the COVID-19 pandemic, fake videos claiming that Muslims are deliberately spreading the virus went ``viral'' on social media platforms in India~\cite{bhatia2022discursive, Human_Rights_Watch_2021, Regan_Sur_Sud_2020, The_Washington_Post_2020}. These false videos led to physical abuses of Indian Muslims and hindered their businesses, as many people boycotted them~\cite{Human_Rights_Watch_2021}. In Bangladesh and other South Asian countries, organized misinformation tends to focus on religious sentiments, unlike in North American regions where misinformation is primarily targeted at politics and electoral systems~\cite{haque2020combating}. Rumors, fabricated images, and targeted memes are frequently posted from social media profiles impersonating members of minority communities, with the aim of inciting social violence South Asian countries~\cite{haque2020combating, kaur2018information, dash2022insights, minar2018violence}. Several incidents of social media-incited mob violence have resulted in the killings of individuals from minority communities~\cite{Hasan_Gooding_Dayant_Johnston_2017, roy2023sociological, al2021content}. In the extreme examples, social media has been found to be complicit in incidents of ethnic cleansing~\cite{Amnesty_International_2023, The_Guardian_2021}. These forms of online harms and violence, magnified through social media, have alarmingly escalated, making the lives of religious minority communities worldwide unsafe due to the instilled feelings of fear, intimidation, and anxiety.

%Despite the initial promise of social media platforms to foster the coexistence of diverse communities, ensure equality of voices in public deliberation, and provide a safe space for participation, for minority communities-- religious or ethnic groups that constitute a smaller proportion of the overall population within a particular society or region~\cite{jackson2005minority} -- these platforms have become unsafe spaces.


%In this paper, we particularly focus on the predominantly Muslim-majority (91.04\%) Bangladesh's religious minority communities, such as Hindu (7.95\%), Buddhist (0.61\%), and Christian (0.30\%)~\cite{bbs2022preliminary} and their experiences on social media platforms.

%around the world 




%Further, the ethical, political, and cultural aspects of faith are seldom considered in CSCW literature of faith-related online harms. 


While CSCW and related disciplines have made significant contributions to understanding and mitigating various forms of online harms for racial, linguistic, and other forms of minority communities, many of which are primarily based in the West~\cite{ogbonnaya2020critical, pyle2021lgbtq, erete2021can}, research in this domain is still limited by a lack of understanding of the contextual, social-psychological, and political aspects of social media use experienced by religious minorities in South Asian regions. We argue that studying the social media use and the unsafe experiences of religious minorities in South Asian countries separately from other forms of minority experiences, such as the well-documented CSCW literature concerning racial minorities in the West~\cite{ogbonnaya2020critical, rankin2021black, musgrave2022experiences}, is important for two primary reasons. First, whereas racial minorities' identities are primarily built on individuals' ancestral and genetical background~\cite{helms1994conceptualization, mcintyre1997making}, religious minorities' identities are based on their beliefs and social practices~\cite{fox2000religious}. Factors such as the perceived threat posed to the worldview of majority groups by the actions of minority groups, the use of religion in political legitimacy, and the influence of religion in ethnic conflicts strongly influence the experiences of ethno-religious minorities~\cite{fox2000religious}, which cannot be accurately characterized by discrimination faced by ethnic minorities alone. Second, unlike the race-based social justice concerns that are comparatively more prevalent in most of the West, social justice concerns in South Asia often revolve around faith-based issues~\cite{nandy1988politics, das2001remaking, rifat2020religion, mim2021gospels}. Religion has played an influential role not only in state politics in South Asian countries but also in socio-cultural politics in everyday life, due to its deep intertwining with the history and culture of the region~\cite{robinson2000islam, nandy1988politics}. These unique dynamics may not be fully captured when analyzing minority experiences where race, language, gender, or other factors have been the center of attention. 

%Due to the differences in identity, the experiences of religious minorities are strongly shaped by religious influences~\cite{fox2000religious}

Despite these differences, modern human rights frameworks tend to collapse all forms of minority rights under the single umbrella of minority protection rights~\cite{ghanea2012religious}. Moreover, when religious minorities face discrimination, their cases are often handled under the category of ``freedom of belief or religion'' instead of minority rights~\cite{ghanea2012religious}. CSCW literature shows a similar pattern, where religious aspects of minority experiences are often collapsed into other cultural and generalized minority categories, as evidenced by a substantial body of work where religion is considered in the periphery of analyzing online harms (see, for example~\cite{shahid2023decolonizing, mustafa2020patriarchy}). For these reasons above, we argue that the religious aspects of minority experiences are not merely a reflection of cultural, ethnic, and racial experiences but require distinct and separate attention to fully understand the safety and vulnerability of religious minority communities on social media.

%While societal power impacts racial identities, religious identities are more malleable due to the exposure of alternative beliefs, ideologies, and the scope of voluntary choices. The latter's susceptibility to societal power dynamics is evident through unique kinds of attacks and suppression of religious minorities' practices in different geocultural contexts.



To this end, we conducted an interview-based study involving three Bangladeshi religious minority communities to comprehensively understand their experiences of using social media platforms. Informed by our findings, we place ``fear'' at the center of our analysis when examining the experiences of religious minorities in their use of social media in Bangladesh. Our findings reveal three dominant patterns: first, the constant political and social psychological influence of fear within religious minority communities on social media platforms; second, the imposition of fear onto minorities by majority groups and social institutions; and third, the continuous adaptation of social media use by the communities based on their anticipation of future fearful consequences. \DIFdelbegin \DIFdel{Our focus on }\DIFdelend \DIFaddbegin \DIFadd{The insights related to }\DIFaddend fear is also informed by the long history of the politics of fear concerning religious minority communities in South Asia. The strong religious influence on nationalist politics in the Indian subcontinent has utilized the politics of fear to justify anti-minority violence in the region~\cite{anand2016hindu}. The online harms incited by social media often align with hyper-nationalist majoritarian political ideologies in South Asian countries~\cite{dash2022insights}. For example, in India, Hindu nationalist politics known as Hindutva perceives religious minority groups as a threat to their identity, thus creating a stereotypical image of these minority groups as dangerous~\cite{anand2016hindu, shani2021towards}. Due to these perceived threats, the majority religious groups portray minority religious groups as ``anti-national'' \textit{Others}~\cite{dash2022insights, islam2007imagining, oommen1986insiders}. Similar strong \DIFdelbegin \DIFdel{intertwining }\DIFdelend \DIFaddbegin \DIFadd{intertwinings }\DIFaddend of religions and politics continue to fuel the politics of fear in other parts of South Asia as well~\cite{mohsin1984religion, riaz2016bangladesh, fair2012faith}. This politics of fear socially constructs hate against religious minority communities in South Asia, and justifies social surveillance, control, and policing against them~\cite{anand2016hindu}. As a result of the amplification of existing societal marginalization of minority communities, as well as the use of social media to incite violence against these communities, social media platforms evoke fear, anxiety, and other negative emotions among minority communities in South Asia~\cite{saha2021short}. Against this backdrop, there is a lack of insights within the field of CSCW and related disciplines regarding the negative experiences of religious minority communities with social media platforms and the support they require. While some aspects of CSCW work in privacy, sensitive disclosure, cyber security, and online harassment have alluded to fear, none are adequate to understand the fearful experiences of religious minorities as informed by our study. Such insights are crucial for understanding and designing strategies to mitigate harms for religious minority communities in the Global South. With this goal in mind, we make the following contributions to the CSCW community:

%\rifat{We can expand if we need to.}

\begin{itemize}
    \item We contribute to the CSCW literature on online safety by providing in-depth insights into the political and socio-psychological aspects of fear among religious minorities in Bangladesh who use social media. Drawing upon the theories of the spiral of silence, politics of emotion, and communication accommodation, we examine the sources and consequences of fear within these communities. Additionally, we discuss the social conditions that either empower or silence these minority communities through the use of the politics of fear. Finally, we explore how these communities address fear by reorienting their social and online connections and adjusting their participation strategies in public spheres.
    \item We contribute to the existing CSCW literature on polarization, restorative justice, and interfaith coexistence on social media by drawing on insights from religious studies, social justice, and interfaith communication. In our discussion, we explore the aftercare and cultural appropriation of restorative justice as means to enhance online safety for religious minority communities in South Asia. By analyzing our findings in relation to the existing literature on harms and violence in South Asia, we uncover the potential of incorporating considerations of history, memory, and postcolonial trauma in the design of solutions for addressing fear in the minority communities.

    %How to make them more specific and concrete. A bit vague now. Actually say those insights are. Spell out what are the sources and consequences
\end{itemize}

We believe our study will advance CSCW's broader vision of social justice and online safety. 


%When the majority religion dominates the political institutions (such as State), the religious minority Others live in an extended state of fearful situation in the South Asian regions~\cite{shani2021towards, lintner2004religious, datta2002post, misra2000hindu}, which is recently being execerbated on social media.



%These instances of social-media incited online harms often align with hyper-nationalist majoritarian political ideologies in South Asian countries~\cite{dash2022insights}. The experiences of religious minority communities are shaped within a cultural construct of the South Asian nations where minority religious groups are often portrayed as ``anti-national'' others~\cite{dash2022insights, islam2007imagining, oommen1986insiders}. As a result of the amplification of existing societal marginalization of minority communities, as well as the use of social media to incite violence against these communities, social media platforms evoke fear, anxiety, and other negative emotions among minority communities in South Asia\rifat{more citation}~\cite{saha2021short}. Against this backdrop, CSCW and related disciplines lack insights into the modes, factors, and consequences of how the fearful experiences of minority communities shape their online and offline experiences in the Global South. Such insights are crucial for our understanding and the design of strategies to mitigate polarization, misinformation, and other online harms in the Global South.



%We present this paper as a step to offer conceptual and design resources within the CSCW community to address online harms for minority communities in South Asia.


%CSCW literature shows a similar trend of sidelining the experiences of religious minority communities demonstrated by a negligible amount of works centering religion to analyze online harms, especially beyond the West when religion plays a dominant role in society. 











%While CSCW and related disciplines have made significant contributions to understanding and mitigating various forms of online harms for racial, linguistic, and other forms of minority communities~\cite{}, the research in this area is still limited by a lack of understanding of the contextual, social-psychological, and political aspects of social media use experienced by the religious minorities in the South Asian regions. Further, the ethical, political, and cultural aspects of faith are seldom considered in CSCW literature of faith-related online harms. We argue that studying the social media use and the unsafe experiences of religious minorities separately from other forms of minority experiences -- such as the considerable amount of HCI studies about racial minorities in the West~\cite{} -- are important for several reasons. Religious minorities represent a different set of aspects of a person's identity primarily based on their their belief and social practices~\cite{fox2000religious}, whereas racial identities build on an individuals' racial and ethnic backgrounds~\cite{}. Because of the differences in identity -- which could also be sometimes intersectional with other forms of minority identities -- the religious minority experiences are strongly shaped by religious influences~\cite{fox2000religious}. The perceived threat posed onto majority groups' worldview by the actions of minority groups, use of religions in political legitimacy, and the influence of religions in ethnic conflicts are consistently found that the harms of ethno-religious minorities are strongly influenced by religion~\cite{fox2000religious}, which could not be accurately characterized by discrimination faced by ethnic minorities, for example. Moreover, unlike the race-based socio-cultural concerns in most of the West, South Asian concerns for social justice often are dominated around faith-based issues. Because of the intertwinedness of religion with the South Asian history and culture~\cite{}, religion has played an influential role not only in state politics in South Asian countries, but also in socio-cultural politics in everyday life~\cite{}. These politics might not be captured from the minority experiences where race, language, or other axis has been the center of attention. Despite such differences, the modern human rights have collapsed all forms of minority rights into the bucket of minority protection rights~\cite{ghanea2012religious}. Further, when religious minorities face discrimination, their case are handled under the category of ``freedom of belief or religion'' instead of minority rights~\cite{ghanea2012religious}. CSCW literature shows a similar trend of sidelining the experiences of religious minority communities demonstrated by a negligible amount of works centering religion to analyze online harms, especially beyond the West when religion plays a dominant role in society. We argue that religious aspects of minority experiences are not merely a reflection of cultural, ethnic, and racial experiences and requires distinct and separate attention to holistically understand the religious minority communities safety and vulnerability on social media. We present this paper as a step to offer conceptual and design resources within the CSCW community to address online harms for minority communities in South Asia.



%The universal equal treatment, which has been celebrated by most democratic states and the peace organization such as the UN, had the underlying assumption that the universal rights for minorities will be panache against all discrimination~\cite{ghanea2012religious}. It took several decades to understand that the equal treatment are discriminatory to those that started lower. For example, if Brahmins and Dalits in India start getting equal treatment, then Dalits are more likely to be discriminated against. 




%These observations show that religious causes of harms and discrimination are not merely a reflection of cultural and ethnic causes of harms~\cite{fox2000religious}, rather demands distinct and separate attention. 


%<religious minorities are categorically different from other minorities> <religious minorities are categorically different in South Asia> <despite being categorically different, religious minority lost its appeal in the minority rights discourse even in insitutions like UN>


%Historically, the protection religious minorities precede the modern human-rights and protection for racial minorities~\cite{ghanea2012religious}. Religious minorities are covered under the general categories of minority rights in human rights protection~\cite{ghanea2012religious}. Although, normatively, religious minorities are designated almost equally alongside ethnic and linguistic minority, religious minority rights are protected only in passing~\cite{ghanea2012religious}. The universal equal treatment, which has been celebrated by most democratic states and the peace organization such as the UN, had the underlying assumption that the universal rights for minorities will be panache against all discrimination~\cite{ghanea2012religious}. It took several decades to understand that the equal treatment are discriminatory to those that started lower. For example, if Brahmins and Dalits in India start getting equal treatment, then Dalits are more likely to be discriminated against. 

%When religious minorities face discrimination, their case are handled under the category of ``freedom of belief or religion'' instead of minority rights~\cite{ghanea2012religious}.


%On top of this, religion as a separate axis of analysis in South Asia is particularly important because of the intertwinedness of religion with the South Asian history and culture. Religion has played the central role in the partition of Indian subcontinent into different states~\cite{}. As a result of this, religion has played an influential role not only in state politics in South Asian countries, but also in socio-cultural politics in everyday life~\cite{}. These politics might not be captured from the minority experiences where race, language, or other axis has been the center of attention.






%We situate our work within the context of Bangladesh, which shares religious-cultural characteristics with the neighboring South Asian countries, particularly regarding the prominent role of religions in society~\cite{}. This geographically, culturally, and historically unique site has drawn separate attention within the CSCW community due to its context largely shaped by colonial histories~\cite{}, limited access to digital technologies~\cite{}, and the influence of religious~\cite{} and spiritual~\cite{} forces. In this context, religious minorities have become victims of misinformation, disinformation, personal attacks, and ridicule~\cite{}. In Bangladesh and other South Asian countries, unlike the North American regions where misinformation is mainly targeted at politics and electoral systems, organized misinformation often targets religious sentiments~\cite{haque2020combating}. Rumors, fabricated images, and targeted memes are often posted from social media profiles impersonating members of minority communities, with the aim of inciting social violence, a common occurrence in South Asian countries~\cite{haque2020combating, kaur2018information, dash2022insights, minar2018violence}. Such harmful online acts frequently lead to organized attacks on places of worship, homes, businesses, and religious festivals~\cite{}. In more extreme cases, social media-incited mob violence results in the killing of individuals from minority communities~\cite{Hasan_Gooding_Dayant_Johnston_2017, roy2023sociological, al2021content}. In several extreme examples, social media has been found to be complicit in incidents of ethnic cleansing~\cite{}. 




%To this end, we conducted an interview-based study involving <n> Bangladeshi religious minority communities, including <Hindu>, to comprehensively understand the social, psychological, and political aspects of using social media platforms. Our findings reveal three dominant patterns: first, the gradual social-psychological influence of fear within the religious minority communities on social media; second, the imposition of fear onto minorities by social or state apparatuses; and third, the continuous adaptation of social media use by the communities based on their anticipation of future fearful consequences. Based on these patterns, our study makes the following contributions to the CSCW community:

%\begin{itemize}
%    \item We contribute significantly to the CSCW literature on online safety by providing in-depth insights into the psychological, political, and cultural dimensions of fear among religious minorities in Bangladesh who use social media. Drawing upon the theories of the spiral of silence, politics of emotion, and communication accommodation, we examine the sources and consequences of fear within these communities. We also highlight how their intersectional minority identities (such as women and LGBTQ individuals) intensify their experiences. Additionally, we discuss the social conditions that either empower or silence these minority communities, as well as their strategies for managing discomfort and fear on social media usage by reorienting their social and online connections and adjusting their participation strategies in public spheres.
%    \item We contribute to the existing CSCW literature on polarization, restorative justice, and online peacebuilding. Drawing on religious studies, indigenous justice, and interfaith communication, we discuss aftercare and cultural appropriation of restorative justice to enhance online safety for religious minority communities in South Asia. By analyzing our findings in relation to the literature on harms and violence in South Asia, we uncover the potential of considering history, memory, and postcolonial trauma in designing solutions for the online safety of these minorities.

    %How to make them more specific and concrete. A bit vague now. Actually say those insights are. Spell out what are the sources and consequences
%\end{itemize}

%We believe our study will advance CSCW's broader vision of social justice and online safety.


%fear is a structural product of history.
%Not as an essential characteristics of religious people
%Misinformation: religious communities is not particularly gullible
%A common way whereby marginalize communities experience fear

%More general 1st para, where does this paper go rather than what are the gaps, what is really interesting in three (what faith based lense offers in this conversation)



%Firstly, drawing upon theories such as the spiral of silence, politics of emotion, and communication accommodation, we provide in-depth insights into the psychological, political, and cultural dimensions of fear experienced by religious minorities in Bangladesh. We examine the sources and consequences of fear within these communities, particularly considering how their other intersectional minority identities exacerbate their experiences. Additionally, we discuss the social conditions that either enable or silence the minority communities, as well as their strategies for accommodating the discomforting aspects of social media use by reorienting their social and online connections, and reorganizing their participation strategies in public spheres. Secondly, building upon our findings and engaging with the existing literature on fear, we contribute to enriching the CSCW literature on online harms by providing policy and design implications for a range of CSCW design resources aimed at mitigating these harms. These implications include the detection of hateful speech, content moderation, and the promotion of contestability. In a broader sense, we discuss how our findings shed light on the barriers faced by minority communities in engaging in public deliberation and democratic participation on social media platforms.


%*****
%Despite the founding promise of social media platforms to foster the coexistence of diverse communities, ensure equality of voices in public deliberation, and provide a safe space for participation, these platforms have instead become unsafe sites for minority communities around the world. In the past decade, as social media platforms gained popularity, the issue of inequality and online harms based on culture and identity related factors including race~\cite{ogbonnaya2020critical, smith2020s}, caste~\cite{vaghela2021birds}, gender~\cite{bardzell2011towards, scheuerman2020we}, and faith~\cite{rifat2020religion} has drawn significant attention in academia and public politics. Academia and the media have reported how social media platforms have introduced and spread new forms of online violence targeted towards religious minority communities in the Global South~\cite{Human_Rights_Watch_2021, Hasan_Macdonald_Ooi_2022}. For example, over the past years, a common pattern of rumor of defaming the holy books in Islam by the minority Hindu individuals spread on social media resulted in mob attacks on Hindu religious establishments and homes in Bangladesh~\cite{Hasan_Macdonald_Ooi_2022, Ethirajan_2021, VICE_2021}. During the COVID-19 pandemic, fake videos claiming that Muslims are deliberately spreading the virus went viral on social media in India~\cite{Human_Rights_Watch_2021, Regan_Sur_Sud_2020, The_Washington_Post_2020}. The fake videos resulted in physical abuses of the Indian Muslims and hampering the business as many people boycott them~\cite{Human_Rights_Watch_2021}. In Bangladesh and other South Asian countries, unlike the North American regions where misinformation is mainly targeted at politics and electoral systems, organized misinformation often targets religious sentiments~\cite{haque2020combating}. Rumors, fabricated images, and targeted memes are often posted from social media profiles impersonating members of minority communities, with the aim of inciting social violence, a common occurrence in South Asian countries~\cite{haque2020combating, kaur2018information, dash2022insights, minar2018violence}. Several social media-incited mob violence resulted in the killing of individuals from minority communities~\cite{Hasan_Gooding_Dayant_Johnston_2017, roy2023sociological, al2021content}. In several extreme examples, social media has been found to be complicit in incidents of ethnic cleansing~\cite{Amnesty_International_2023, The_Guardian_2021}. This forms of online harms and violence amplified through social media have been alarmingly increasing and making the lives of religious minority communities unsafe around the world.

%While CSCW and related disciplines have made significant contributions to understanding and mitigating various forms of online harms for racial, linguistic, and other forms of minority communities, many of which are primarily based in the West~\cite{}, the research in this area is still limited by a lack of understanding of the contextual, social-psychological, and political aspects of social media use experienced by the religious minorities in the South Asian regions. We argue that studying the social media use and the unsafe experiences of religious minorities in South Asian countries separately from other forms of minority experiences -- such as the well-documented CSCW literature concerning racial minorities in the West~\cite{} -- is important for two primary reasons. First, religious minorities represent a different set of aspects of a person's identity primarily based on their their belief and social practices~\cite{fox2000religious}, whereas racial identities build on an individuals' racial and ethnic backgrounds~\cite{}. Because of the differences in identity, the religious minority experiences are strongly shaped by religious influences~\cite{fox2000religious}. The perceived threat posed onto majority groups' worldview by the actions of minority groups, the use of religions in political legitimacy, and the influence of religions in ethnic conflicts are a few of the strong reasons why ethno-religious minorities are strongly influenced by religion~\cite{fox2000religious}, which could not be accurately characterized by discrimination faced by ethnic minorities, for example. Second, unlike the race-based social justice concerns in most of the West, South Asian concerns for social justice often are dominated around faith-based issues~\cite{}. Because of the intertwinedness of religion with the South Asian history and culture~\cite{}, religion has played an influential role not only in state politics in South Asian countries, but also in socio-cultural politics in everyday life~\cite{}. These politics might not be captured from the minority experiences where race, language, or other axis has been the center of attention. Despite such differences, the modern human rights have collapsed all forms of minority rights into the bucket of minority protection rights~\cite{ghanea2012religious}. Further, when religious minorities face discrimination, their case are handled under the category of ``freedom of belief or religion'' instead of minority rights~\cite{ghanea2012religious}. We observe a similar trend in CSCW literature, when religion is collapsed into other cultural and minority categories, which is evident in a sizable CSCW literature where religion is put into a periphery of analyzing online harms (see, for example~\cite{shahid2023decolonizing, mustafa2020patriarchy}). We argue that religious aspects of minority experiences are not merely a reflection of cultural, ethnic, and racial experiences and requires distinct and separate attention to holistically understand the religious minority communities safety and vulnerability on social media.

%To this end, we conducted an interview-based study involving three Bangladeshi religious minority communities to comprehensively understand their experience of using social media platforms. Informed from our findings, we put fear into the center of analysing the religious minority experiences of social media use in Bangladesh. Our findings reveal three dominant patterns: first, the gradual social-psychological influence of fear within the religious minority communities on social media; second, the imposition of fear onto minorities by social or state apparatuses; and third, the continuous adaptation of social media use by the communities based on their anticipation of future fearful consequences. Our attention to fear is also informed from a long history of the politics of fear concerning the religious minority communities in South Asia. A strong religious influence on the nationalist politics in the Indian subcontinent has used the politics of fear in justifying anti-minority violence in the region~\cite{anand2016hindu}. The social-media incited online harms often align with hyper-nationalist majoritarian political ideologies in South Asian countries~\cite{dash2022insights}. For example, the the Hindu national politics in India, Hindutva, feels the insecurity that the religious minority Others are a threat to their identity, and thus create a stereotype image of the minority Others as a danger to them~\cite{anand2016hindu, shani2021towards}. In doing so, the majority religious groups portray minority religious groups as ``anti-national'' Others~\cite{dash2022insights, islam2007imagining, oommen1986insiders}. Similar strong intertwindness of religions and politics continue to create the politics of fear in other parts of South Asia, too~\cite{mohsin1984religion, riaz2016bangladesh, fair2012faith}. Such a politics of fear socially construct hate against the religious minority Others in South Asia and justify social surveillance, control, and policing against them~\cite{anand2016hindu}. As a result of the amplification of existing societal marginalization of the minority communities, as well as the use of social media to incite violence against these communities, social media platforms evoke fear, anxiety, and other negative emotions among minority communities in South Asia\rifat{more citation}~\cite{saha2021short}. Against this backdrop, CSCW and related disciplines lack insights into how the fearful experiences of minority communities shape their online and offline experiences in the Global South. While a body of CSCW of work in privacy, sensitive disclosure, cyber security, and online harassment has alluded to fear, none are adequate to understand the religious minorities' fearful experiences informed from our study. Such insights are crucial for our understanding and the design of strategies to mitigate polarization, misinformation, and other online harms for the religious minority communities in the Global South. With this goal, we make the following contributions to the CSCW community:
